The resource cost of large scale quantum computing

This thesis deals with the problematics of the scalability of fault-tolerant quantum computing. This question is studied under the angle of estimating the resources needed to set up such computers. What we call a resource is, in principle, very general; it could be the power, the energy, the total bandwidth allocated to the different qubits... However, we mainly focus on the energetic cost of quantum computing. In particular, we develop an inter-disciplinary approach that allows to minimize the resources required to implement algorithms on quantum computers. By asking to find the minimum amount of resources required to perform a computation under the constraint that the algorithm provides a correct answer with a targeted accuracy, it is possible to optimize the whole computer in order to minimize the resources spent, while being sure to have a correct answer with a high probability. We apply this approach to a complete model fault-tolerant quantum computer based on superconducting qubits. Our results indicate that for algorithms implemented on thousands of logical qubits, our method makes it possible to reduce the energetic cost by orders of magnitudes in regimes where, without optimizing, the power consumption could be close to the gigawatt. This work illustrates that the energetic cost of quantum computing should be a criterion in itself, allowing to evaluate the scaling potential of a given quantum computer technology. It also illustrates that optimizing the architecture of a quantum computer, via inter-disciplinary methods, including algorithms, error correction, qubit physics, engineering aspects, such as the ones that we propose, can prove to be a powerful tool, clearly improving the scaling potential of quantum computers. Finally, we provide general hints about how to make fault-tolerant quantum computers energy efficient.

==> chapter4/chapter4_old.tex <==
\chapter{The energetic cost of quantum computing: formulation of the question}
\section{Introduction}
In this chapter, we are going to design the general method behind energetic estimation of quantum computing. This method can in principle be applied both in NISQ algorithm (with some restrictions that we will explain) and in fault tolerance. This chapter will however be dedicated to explain the general principle of the method and to provide simple examples where it can be applied. The estimations we will do behind those examples shouldn't however be taken too seriously because of the many simplified assumption we are going to do. They are just here to allow to grasp the concept in a concrete manner. We will also see what are the differences between energetic estimation for algorithm implemented with or without quantum error correction: in the end of this chapter we will adapt the approach to fault tolerance. The following chapter will consist in using this method in order to make a more realistic energetic estimation of implementing an algorithm on a fault tolerant quantum computer.
\section{Formulating the question}

\subsection{The principle}
The general purpose of an algorithm is to provide an answer to some computational task. What we care about is obviously to have the good answer to this task, there is no point in having a bad one. However, because of noise, there will always have a probability that the answer we find is not the good one. On the other hand, the probability to find a successful answer will be related to how much some resource an experimentalist is ready to invest in the calculation. Indeed, implementing successfully an algorithm (in the sense that it provides an answer having a high probability of success) has a cost. We saw examples in the previous chapter with the energy that we allowed to spend in order to create the pulses driving the qubits. When we restricted too much this energy, the algorithm had a poor success probability. Without loss of generality, we will now assume that the resource we are interested in is the \textit{power} required to implement an algorithm. We understand that there must exist a \textit{minimum} power required to implement successfully an algorithm. And we can phrase the exact question we should address in order to find it. We basically ask: "what is the minimum power I have to spend under the constraint that the algorithm I am implementing provides the good answer to the task with a probability higher or equal to some target I want.". The answer to this somewhat lengthy question is the only thing that really matters in order to be power efficient. We can phrase it in a mathematical manner as the following problem of optimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | p_{\text{success}}(\bm{\delta}) \geq p_{\text{target}}},
\label{eq:ideal_solve}
\end{align}
where $P$ is the power, $p_{\text{target}}$ is the success probability we aim for, and $p_{\text{success}}$ is the actual probability of success of the algorithm. We see that we introduced the family of parameters $\bm{\delta}$ (the fact it is a family is represented by the bold notation associated to vectors). They represent the \textit{tunable} parameters that the experimentalist can vary in order to reach the minimum. A typical example would be the qubit temperature $T_{\text{Q}}$: changing it would at the same time modify the power it costs to perform the computation (the electrical power for the cryogenic typically depends on $T_{\text{Q}}$), but the success probability as well (a too high temperature would induce a poor quality in the answer). Thus, in general, both the probability of success and the power depend on the family $\bm{\delta}$\footnote{Of course it is possible that one parameter in the family of parameters $\bm{\delta}$ only affect the success and not the power cost, and reciprocally.}. This minimization under constraint provides an equation that relates the resource one should spend with the probability of success of the algorithm. We also see that not only the minimum power can be found performing this minimization, but the optimum set of parameters allowing to reach this minimum, $\bm{\delta}_{\text{opt}}$ will also be found.

Unfortunately, directly solving this problem is too complicated in general. Indeed it is usually not possible to directly find the function $p_{\text{success}}(\bm{\delta})$ as it would usually require to know the density matrix at the end of the algorithm. If this is a requirement the method would have no interest because it would mean that the circuit can be efficiently simulated classically\footnote{As the goal is to implement an algorithm on a quantum computer, this algorithm must present advantages compared to a classical simulation.}. For this reason, we will take a slightly different approach. We will not try to estimate the success probability of the algorithm, but we will try to estimate, or at least to bound the "quantity of noise" there is in the final density matrix of the algorithm (right before the measurements). This approach is slightly different because there is a unique way to define the success probability of the algorithm while there are different ways to evaluate the quantity of noise inside a density matrix (we could think about the trace distance or the fidelity with respect to the ideal state for instance). The reason to do this strategy is that it is an easier quantity to estimate, or more usually, \textit{to bound}, than the probability of success of the algorithm\footnote{Also, the different ways to quantify the noise are usually related: knowing the value of one often allows to give a bound the other.}. To give specific examples, the worst-case fidelity of an algorithm can easily be bounded by the knowledge of the worst-case fidelity of each individual gates composing it. And from this knowledge, we can then bound, or have a rough estimation of the probability of success of the algorithm (which is much more complicated to directly access theoretically). This is another important requirement we should have in the way we measure the quantity of noise: there is no point in being able to estimate the quantity of noise in the final density matrix if it doesn't give any information about the probability to have the good answer. All those requirements will give us constraints on what are the good or the bad tools that can be used to measure the quantity of noise in the final density matrix of algorithms. We call them "metrics" and write them with the letter $\mathcal{M}$ in what follows. Putting aside those issues for now on, the problem of power estimation can in the end be formulate by the following minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{\text{target}}}.
\end{align}
This equation means that we want to find the minimum power under the constraint that the quantity of noise (as quantified by the metric $\mathcal{M}$) is lower than some targetted quantity of noise $\mathcal{M}_{\text{target}}$ considered as acceptable by the experimentalist. The value of the metric $\mathcal{M}$ depends on the family of tunable parameters $\bm{\delta}$ for the exact same reason as $p_{\text{success}}$ in \eqref{eq:ideal_solve} also depended on those.
\subsection{General properties}
\subsubsection{The minimum power increases with the targetted accuracy}
Let's assume that there exist a parameter $\delta_j$ in the list of parameters  $\bm{\delta}$ such that, when we increase it, the power decreases while the quantity of noise increase. Mathematically it means that:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
One example of such parameter will often be the temperature of the qubits. If we increase the qubit temperature, the power it costs to maintain them cool will typically decrease, but the quantity of noise will usually increase because they will be submitted to more thermal noise. We will see it in a concrete manner in the parts where we will take physical examples: the hypothesis that such parameter $\delta_j$ exists will typically be true in relevant physical systems. From now on, we will assume it is the case.

This hypothesis will imply the following two properties. First, (i) the minimum power required such that the quantity of noise of the algorithm is equal \textit{or lower} to $\mathcal{M}_{\text{target}}$ is the same as the minimum power required such that the quantity of noise is \textit{equal} to $\mathcal{M}_{\text{target}}$, i.e the following equality is true:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}}
\end{align}
Let us do a proof by contradiction of this fact. We assume that the minimum power is found when $\mathcal{M} < \mathcal{M}_{\text{target}}$. As $\partial_{\delta_j} \mathcal{M}>0$, we can increase $\delta_j$ for some range without violating the condition $\mathcal{M} \leq \mathcal{M}_{\text{target}}$. Doing so, we will also decrease the power as $\partial_{\delta_j} P<0$. Thus, as soon as $\mathcal{M}<\mathcal{M}_{\text{target}}$ we do not minimize the power consumption: the minimum is necessarily reached for $\mathcal{M}=\mathcal{M}_{\text{target}}$. In the same line of thoughts, we can also prove that (ii) $P_{\min}$ is a \textit{strictly decreasing} function of $\mathcal{M}_{\text{target}}$. To show this, let us consider two targets such that $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$. Then, as:
\begin{align}
\min(P)_{\big | \mathcal{M} \leq \mathcal{M}^2_{\text{target}}}=\min(P)_{\big | \mathcal{M} = \mathcal{M}^2_{\text{target}}},
\end{align}
the minimum power obtained for $\mathcal{M}<\mathcal{M}^2_{\text{target}}$ is necessarily bigger or equal to the one obtained for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Because of that, as $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$, we deduce that: $P_{\min}(\mathcal{M}^1_{\text{target}}) \geq P_{\min}(\mathcal{M}^2_{\text{target}})$. It remains to show that they cannot be equal. We also do a proof by contradiction. Let us consider a set of parameters $\bm{\delta}$ such that: $P(\bm{\delta})=P_{\min}(\mathcal{M}^1_{\text{target}})$, and $\mathcal{M}(\bm{\delta})=\mathcal{M}^1_{\text{target}}$\footnote{We say "a" set of parameters and not "the" set of parameters as the minimum power consumption could be in principle reached for many different values of $\bm{\delta}$.}. If we increase $\delta_j$ until the moment $\mathcal{M}=\mathcal{M}^2_{\text{target}}$, as $\partial_{\delta_j} P < 0$, it has for effect to \textit{strictly} decrease the power consumption while ensuring $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Thus, the minimum power reached for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$ is necessarily \textit{strictly} lower than the one reached for $\mathcal{M}=\mathcal{M}^1_{\text{target}}$.

In summary, here we proved the following property that we will frequently use.
\begin{property}{Behavior of the minimum power}

\label{prop:behavior_min_power}
If there exists at least one parameter $\delta_j$ in the family of parameters $\bm{\delta}$ on which:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
Then, we have:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}},
\end{align}
which means that the minimum power consumption is found when we ask for an accuracy that it is exactly equal to what we target: asking for a better accuracy is necessarily more costly. We also have that
$P_{\min}$ is a strictly decreasing function of $\mathcal{M}_{\text{target}}$ (for the same reason).
\end{property}
This property establish properly the intrinsic connection between noise and power: asking for a better accuracy has an energetic cost. But again this connection is true because of the hypothesis we made on the behavior of power and metric with respect to the parameter $\delta_j$ (which will frequently be true in physical systems).
\subsubsection{Equivalence between minimum power for a targetted accuracy and maximum accuracy for a given power}
\label{sec:equivalence_minpow_maxacc}
Now, we can show that asking to minimize the power in order to reach a given accuracy is in some sense, equivalent to asking to find the best accuracy the computer can get to for a given (i.e fixed) amount of power available. This property is true as soon as $P_{\min}$ is a decreasing function of $\mathcal{M}_{\text{target}}$ (which will usually be the case as explained before).

Those two questions are equivalent in the sense of what is represented on figure \ref{fig:equivalence_minpow_maxacc}. On this curve is represented the minimum power required to implement the algorithm as a function of the maximum quantity of noise acceptable in its answer: $\mathcal{M}_{\text{target}}$. In this case, this graph can be read in two directions. Indeed, if we invert the meaning of the axis, i.e we interpret it as a curve representing a value of some quantity of noise as a function of some injected power, we can also interpret it as the \textit{minimum} quantity of noise it is possible to reach as a function of this injected power. More precisely, let us consider any couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. By definition of $P_{\min}$, if someone wants to have an accuracy $\mathcal{M}^0_{\text{target}}$, the minimum power required will be $P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. But reciprocally, if this person has a given amount of power $P^0$ available, the minimum quantity of noise it can get to (thus maximum accuracy) is $\mathcal{M}^0_{\text{target}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.5\textwidth]{chapter4/images/equivalence_minpow_maxacc}
\caption{The minimum power necessary as a function of the maximum quantity of noise acceptable targetted, $\mathcal{M}_{\text{target}}$ is represented. Because this function is monotonous, the curve can also be interpreted as the lowest quantity of noise acceptable for a given amount of power available as explained in the main text.}
\label{fig:equivalence_minpow_maxacc}
\end{center}
\end{figure}
\FloatBarrier

In order to show it, we consider again the couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. We now ask: what is the maximum accuracy, i.e the lowest quantity of noise $\mathcal{M}$ the computer can get to if it has at its disposal the power $P^0$. Necessarily, it can be \textit{at least} as accurate as $\mathcal{M}^0_{\text{target}}$: $\mathcal{M}$ must verify $\mathcal{M} \leq \mathcal{M}^0_{\text{target}}$. Indeed $\mathcal{M}^0_{\text{target}}$ is an explicit example of target reachable for an injected power $P^0$. Now it remains to prove that the strict inequality is not possible: no better accuracy is reachable for this amount of power. This can be shown using again a proof by contradiction: let's assume that we find that the best accuracy it is possible to reach for an injected power $P^0$ verifies $\mathcal{M} < \mathcal{M}^0_{\text{target}}$. We assume that this power is reached for the family of parameters $\bm{\delta}=\bm{\delta}_0$. We necessarily have $P^0=P(\bm{\delta}_0) \geq P_{\min}(\mathcal{M})$: indeed $P^0$ amount of power would be used to have an accuracy $\mathcal{M}$, but it might be possible to use less power to reach that accuracy. As on the other hand $P_0=P_{\min}(\mathcal{M}^0_{\text{target}})$, we deduce that $P_{\min}(\mathcal{M}^0_{\text{target}})\geq P_{\min}(\mathcal{M})$. Now, this result is absurd. Indeed, as $\mathcal{M}<\mathcal{M}^0_{\text{target}}$, and as $P_{\min}$ \textit{strictly} decreases as a function of $\mathcal{M}$, necessarily $P_{\min}(\mathcal{M}^0_{\text{target}}) < P_{\min}(\mathcal{M})$. 

All this shows that the curve can be read in two directions: \textit{there is an equivalence between asking to minimize the noise for a given amount of power available, and asking to minimize the power in order to target a given quantity of noise.}
\subsection{An introductive example}
\subsubsection{Description of the problem}
\label{sec:single_qubit_example}
Let us illustrate the concepts with a very simple example: we wish to minimize the power to spend in order to implement a $\pi$-pulse on a qubit. For this, we need to specify: (i) the noise model describing the physics, (ii) the way we quantify this noise, i.e which metric we are going to choose, (iii) the expression of the power we want to minimize and (iv) the list of parameters we would like to optimize in order to minimize this power.

We start to specify (i). Here, we assume that the only reason why the qubits are noisy is because of thermal noise. The noisy evolution can be modeled as:
\begin{align}
&\frac{\partial \rho}{\partial t}=\frac{1}{i \hbar}[H,\rho]+\gamma_{\text{sp}} \overline{n}_{\text{tot}} D[\sigma^{\dagger}](\rho) + \gamma_{\text{sp}}(\overline{n}_{\text{tot}}+1) D[\sigma](\rho) \label{eq:evolution_noisy_gate}\\
&D[\sigma](\rho) \equiv \left(\sigma \rho \sigma-\frac{1}{2}(\sigma^{\dagger} \sigma \rho + \rho \sigma^{\dagger} \sigma) \right),
\end{align}
%where $H$ is the Hamiltonian implementing the gate, $\overline{n}_{\text{tot}}$ represents the noise photon occupation, i.e the number of photons in the power spectral density of noise \red{to double check the vocabulary is the good one}, and $\gamma_{\text{sp}}$ is the qubit-waveguide coupling\footnote{We remind that its inverse gives the typical qubit lifetime at $0$ temperature.}. As explained in the chapter dedicated to fault tolerance, it is always possible to "decouple" the effect of the noise from the perfect implementation of the gate such that everything will behave \textit{as if} the perfect implementation of the gate occured first, then followed by some noise. If the quantum channel $\mathcal{U}$ represents the ideal (unitary) implementation of the gate, and $\mathcal{E}$ represents the noisy implementation (thus following the equation \eqref{eq:evolution_noisy_gate} integrated for the duration of the gate), we can always define $\mathcal{N}$ such that $\mathcal{E}=\mathcal{N} \circ \mathcal{U}$. With this definition, $\mathcal{N}$ represents the effect of the noise "alone" that is acting "after" the perfect implementation of the gate. Conceptually we could proceed this way here, but in order to anticipate the section dedicated to fault tolerance, we will adopt a slightly simpler way to model the noise. We will approximate this noise map $\mathcal{N}$ by considering that it can be estimated by integrating  \eqref{eq:evolution_noisy_gate} with $H=0$, for a duration equal to the gate duration. When we say that $\mathcal{N}$ is obtained by integrating this equation, it means that we consider a basis of initial states for the qubit from which we can deduce the mathematical expression of $\mathcal{N}$. This is an approximation because we can expect this result to be different than the computation of the exact evolution $\mathcal{E}$, and then defining $\mathcal{N}= \mathcal{U}^{-1} \circ \mathcal{E}$. However,  this simplification will not change in a quantitative manner our estimation of the quantity of noise introduced by such evolution \footnote{This is actually something that we checked: for a $\pi$-pulsife the expressions of the worst case and average fidelity of the "precise" or "approximated" approach are very similar.}. In the end, the map $\mathcal{N}$ is then accessible which defines our noise model. It will be a function of $\overline{n}_{\text{tot}}$, $\gamma_{\text{sp}}$ and $\tau$ the gate duration. 

Now, we specify (ii). In order to quantify the quantity of noise in the final density matrix, we will use either the worst-case or average infidelity of this channel. We call infidelity the quantity $1-F$ where $F$ is the fidelity. We find:
\begin{align}
\mathcal{M}=(X+Y \overline{n}_{\text{tot}}) \gamma_{\text{sp}} \tau,
\end{align}
where $(X_{\text{worst}},Y_{\text{worst}})=(1,1)$ and $(X_{\text{avg}},Y_{\text{avg}})=(1/3,2/3)$ for worst-case infidelity and average one respectively. The metrics are then defined. But we cannot be satisfied of those expressions because we don't know what $\overline{n}_{\text{tot}}$ is equal to, we need to explain it. 

In the case the qubit is at the temperature $T_{\text{Q}}$, and \textit{if the signals are generated at this same temperature}, we would simply have: $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}}) \equiv 1/(e^{\beta_{\text{Q}} \hbar \omega_0}-1)$, with $\beta_{\text{Q}}=1/(k_b T_{\text{Q}})$, and $\omega_0/2 \pi$ is the qubit frequency (typically around $6$ GHz). $\overline{n}_{\text{BE}}$ is the Bose Einstein population for bosons of frequency $\omega_0/2 \pi$, at temperature $T_{\text{Q}}$ \cite{cohen1998mecanique}. But if the signals are generated at a temperature $T_{\text{Gen}}$, then the thermal noise at this temperature would affect the qubit evolution. This is why attenuators are typically put on the driving lines. Their role is to remove the noise (and in particular the thermal noise) coming from the higher temperature stages. An attenuator is composed of resistive elements that will dissipate into heat any signal injected at its input as shown on figure \ref{fig:attenuator_principle}. If $P_{\text{in}}$ is the input power before the attenuator, and $P_{\text{out}}$ the power at its output, we define the attenuation ratio by $A \equiv P_{\text{out}}/P_{\text{in}}$. It is possible to show \cite{pozar2011microwave} that for signals generated at $T_{\text{Gen}}$, an attenuator put at the temperature $T_{\text{Q}}$ will generate an amount of noisy photons $\overline{n}_{\text{tot}}$ being equal to:
\begin{align}
\overline{n}_{\text{tot}}(T_{\text{Q}},T_{\text{Gen}},A)=\frac{A-1}{A} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A} \stackrel{A \gg 1}{\approx} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A}
\end{align}
Let us first comment the formula in the $A \gg 1$ regime. It means that the quantity of noisy photons felt by the qubits will be equal to the number of noisy photons at the attenuator temperature, on which we add the noisy photons coming from the higher temperature stage, but attenuated by a factor $A$. The noise is basically attenuated in the same way than the signals sent. For an infinite attenuation, the qubits will be entirely isolated from any thermal noise coming from higher temperature stages. However this cannot be the exact expression. For instance for $T_{\text{Q}}=T_{\text{Gen}}$ (if everything is thermalized at $T_{\text{Q}}$), we would not find $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})$ with the approximated expression. This is the reason why the exact expression is actually the one of the left: it correctly describes the situation when $T_{\text{Q}}=T_{\text{Gen}}$ and $A=1$ (no attenuation: everything behave as if the qubits where thermalized at $T_{\text{Gen}}$). Of course this formula should be thought as a first order description \red{to check} of the physics (what we said is not a proof that this expression is the correct one), but it is what is used to describe the propagation of noise in microwave circuits \cite{pozar2011microwave}. Physically we can understand the situation as follows: the signal generation stage can be thought as some cavity which is thermalized at $T_{\text{Gen}}$. This cavity thus emits a blackbody radiation in a one-dimensional waveguide: it is the thermal noise. Then this noise propagates in a ballistic manner in the waveguide (as a waveguide will by construction be a good conductor for microwave frequencies, the noise won't be attenuated there). This noise is then dissipated inside of the attenuator and "converted" into phonons: this is a kind of heat that can be evacuated by the cryogenics. But the attenuator, being thermalized at $T_{\text{Q}}$, also generates thermal noise that will interact with the qubits. It corresponds to $\overline{n}_{\text{BE}}(T_{\text{Q}})$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/attenuator_principle}
\caption{Principle behind the attenuation. The signals are generated at a temperature $T_{\text{Gen}}$. Thus, in addition to the signals there is noise at this temperature that is propagating inside of the waveguide as represented by the noisy blue gaussian. The qubit is preceeded by an attenuator at the temperature $T_{\text{Q}}$. The attenuator will dissipate the noise before it reaches the qubit, but it dissipates the signal in the same manner. It is the fact that the heat $\dot{Q}_{\text{Att}}$ has to be evacuated by a cryogenic unit that makes the gate energetically costly (as shown by \eqref{eq:power_single_qubit_gate}).}
\label{fig:attenuator_principle}
\end{center}
\end{figure}
\FloatBarrier
Now, in practice the effect of the thermal noise coming from the higher temperature stages will be reduced by the following strategy. First, the signal that must arrive on the qubit has a well defined value: we must have $P_{\text{out}}=P_g$, where as explained in the fist chapter of this thesis \red{put a ref} $P_g=\hbar \omega_0 \Omega^2/(4 \gamma_{\text{sp}})$ with $\Omega=\theta/\tau$. Here $\theta$ represents the angle of rotation desired for the single qubit operation ($\theta=\pi$ for us in this section). Then, the attenuation $A$ is usually chosen in such a way that $\overline{n}_{\text{BE}}(T_{\text{Gen}})/A < \overline{n}_{\text{BE}}(T_{\text{Q}})$: the noise coming from the higher temperature stage does not dominate the physics. From the knowledge of $A$ the experimentalist deduce what is the power the generated signals should have. The general philosophy is to generate signals of high enough amplitude such that after attenuation there is a high signal over noise ratio while having a signal of appropriate power for the physics of the quantum gate. At this point, we can say that the metrics we expressed are now "well defined" because we know what $\overline{n}_{\text{tot}}$ is equal to as a function of the characteristics of the problem.

Now, we need to give the expression of the power (point (iii)). Here, we will be interested in the electrical power that we need in order to remove the heat dissipated inside of the attenuators. We will assume that our cryogenic unit has a Carnot efficiency. The heat dissipated per unit time is simply equal to $P_{\text{in}}-P_{\text{out}}$\footnote{We implicitely neglect the heat that will be dissipated when the signals will "go back", i.e after reflection on the qubit. Indeed, the power that would be dissipated by this reflection will be lower than $(A-1) P_g$ and we will neglect it. This approximation is even more true in the regime $A \gg 1$ on which we are focusing.}, the low temperature stage on which the heat has to be evacuated has a temperature $T_{\text{Q}}$, and the high temperature stage is basically the laboratory at temperature $300K$. Assuming that $A \gg 1$ (if it is not the case the evolution would be way too noisy), we get:
\begin{align}
P(T_{\text{Q}},A)=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A P_g
\label{eq:power_single_qubit_gate}
\end{align}
%All that being said, we will consider that $T_{\text{Gen}}=300K$ here (the signals are generated outside of the cryogenics, in the laboratory), and we will consider that the parameters we are going to optimize will be $T_{\text{Q}}$ and $A$. The point (iii) is now specified and the last thing to do is to provide the expression of the power.
Finally, for our last point (iv), we specify the variables we want to optimize. It will be $\bm{\delta}=(T_{\text{Q}},A)$ in this first example as we will assume that $T_{\text{Gen}}=300K$ (the signals are generated outside of the cryogenics here). In the end, the problem is well defined, and we can solve the minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{(T_{\text{Q}},A)} P(T_{\text{Q}},A)_{\big | \mathcal{M}(T_{\text{Q}},A) = \mathcal{M}_{\text{target}}}
\end{align}
\subsubsection{The competition between noise and power}
We first illustrate on figure \ref{fig:competition_power_noise} in a concrete manner the intrinsic competition there is between asking for a low noise and a low power consumption. The parameters we chose for the gate are $\gamma_{\text{sp}}=1kHz$, $\tau=25 ns$ (and $\theta=\pi$: we do a $\pi$-pulse). In the rest of this thesis we will also use the decibel: "dB" unit to represent the attenuation. This unit is related to the attenuation in "natural unit", i.e when $A=P_{\text{in}}/P_{\text{out}}$ as:
\begin{align}
A_{\text{dB}}=10 \log_{10}(A)
\end{align}
For instance, a signal being attenuated of a factor $10$ will correspond to $10 \text{dB}$. A signal attenuated of a factor $10^5$ will correspond to $50 \text{dB}$. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/competition_power_noise}
\caption{Unoptimized power consumption as a function of the attenuation and the qubit temperature (color-plot). The cyan and white lines represent the iso-infidelity for respectively the average and worst case infidelity.}
\label{fig:competition_power_noise}
\end{center}
\end{figure}
\FloatBarrier
On this graph, we see that putting a high attenuation and a low qubit temperature induces a high power consumption. Reciprocally a high qubit temperature and a low attenuation leads to a small power consumption. We can also see that the regions of high power consumption correspond to regions of low noise, and regions of lower power consumption correspond to regions where the noise is high. Indeed the iso-metric lines have lower values in the bottom right part of this graph which corresponds to region of high power consumption (and higher values in the upper left part of this graph where the power is low). It illustrates the intrinsic opposite behavior between noise and power.

Let us now focus on a given iso-metric line: we wish to implement the single qubit gate in order to reach a targetted accuracy. The power consumption on those lines can drastically vary. For instance, the white iso worst-case infidelity which is at the bottom right of this graph is associated to power varying in the range (approximately) $[10^{-3},10^{-1}]$. It illustrates that choosing wisely $T_{\text{Q}}$ and $A$ is a key asset to potentially make important energetic saves: there are many possible ways to reach a given accuracy, and each of those choice can be associated to a drastically different power consumption. Of course this example is very simple as we only modeled the heat dissipated in the attenuators, but we see that it can potentially lead to quantitative saves in power consumption, and we can naturally expect that it would remain true for more complicated models\footnote{In particular because more tunable parameters will be involved, the optimum choice of parameters allowing to minimize the power consumption might be not trivial for more complicated models.}.
\subsubsection{Minimizing the power consumption}
Now, we can minimize the power consumption in order to reach a given target. This is shown on figure \ref{fig:min_power_fct_metric_1qb}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/min_power_fct_metric_1qb}
\caption{Minimum power consumption as a function of the metric target. Inset: optimum qubit temperature $T_{\text{Q}}^{\text{opt}}$ allowing to reach this minimum. Blue points: worst-case fidelity, orange: average. The black line is a guide for the eye. As explained in \ref{sec:equivalence_minpow_maxacc}, this curve can also be interpreted as the minimum metric target it is possible to reach as a function of the injected power.}
\label{fig:min_power_fct_metric_1qb}
\end{center}
\end{figure}
\FloatBarrier
We see on that graph that the minimum power is a stricly decreasing function of $\mathcal{M}_{\text{target}}$ (whatever the metric we choose: worst-case or average infidelity). This is an illustration of the property \ref{prop:behavior_min_power}. Indeed in the case we study when $T_{\text{Q}}$ increases, the power decreases while the metric increases\footnote{As a side remark, in this case we would have the same kind of behavior for $1/A$: increasing it (thus reducing the attenuation) lower the power but increases the amount of noise}. We also see from the inset \textit{how} the power consumption is being decreased for a higher target: the temperature of the qubits increases. We did not represent it here but we would also see that the optimum attenuation would decrease as a function of $\mathcal{M}_{\text{target}}$. As explained in \ref{sec:equivalence_minpow_maxacc}, we can also switch the interpretation of this curve and realize that it also represents the maximum accuracy (i.e minimum value of $\mathcal{M}_{\text{target}}$) it is possible to reach as a function of some injected power. Finally, this graph also illustrates that the minimum power required depend on the metric that is used. The worst-case fidelity as being "more demanding" will ask for a bigger power consumption to reach a given target in contrary to the average fidelity. To make a connection with the previous section, the minimum power obtained for $\mathcal{M}_{\text{target}}=10^{-4}$ for the average infidelity (it is about $2.10^{-6}$) corresponds to the minimum power we would find along the upper left cyan iso-metric line in figure \ref{fig:min_power_fct_metric_1qb}.
\section{Hardware-software "full-stack" optimization}
\subsection{General framework}
At this point, we have shown how parameters describing the "hardware" part of the computer can in principle be optimized given the competition between noise and power ($A$ and $T_{\text{Q}}$ were the variables playing this role). But our example was about a single qubit gate which is not very interesting in practice: the goal of a computer is to run algorithms composed of many gates. In this section we will explain the general approaches we can choose in order to minimize the power consumption of a quantum computer running algorithms. We will naturally generalize the optimization by including in it the "software" part of the problem, i.e the characteristics of the implemented algorithm. It will play a role for two aspects: it will allow us to find which characteristics of the algorithms play an important role in order to estimate the power consumption, but it will also allow us to \textit{optimize} the way the algorithm is compiled in order to minimize the consumption (at least in principle). Finally, we will provide a simple, yet quite general model for the power function $P(\bm{\delta})$ and noise estimation $\mathcal{M}(\bm{\delta})$. We will use a number of assumption in this part, mainly for pedagogic purpose (and also because they are enough for the work that has been done), but generalizations to more general models would often be straightforward. Finally, we will express everything here in term of \textit{physical} qubits and gates which is why all the quantities introduced will have an index $P$. This is in order to anticipate the fault tolerant adaptation of this framework that will be done later in this chapter. It will change some quantitative aspects but the overall philosophy would remain identical as we will see.
\subsubsection{A general model for metric and power}
To begin with, let us try to have some general expression of the power regardless of any optimization (i.e we focus on determining a generic expression for the function $P(\bm{\delta})$ without trying to minimize it based on the metric target). The first thing to acknowledge is that there might have a constant energetic cost regardless of what the computer is doing, i.e if it is running an algorithm or not. We call it the \textit{passive} energetic cost. One typical example of that is the heat conduction: all the cables necessary to control the qubits will always be inside of the computer, and they will bring heat that will have to be evacuated\footnote{We will see other examples of passive cost outside from heat conduction later on.} which costs electrical power for the cryogenic. Here, we will assume that the passive costs scale proportionnally with the number of (physical) qubits $Q_P$ inside the computer but we have to keep in mind that other scaling laws could be involved\footnote{For instance, in an architecture in which the qubits are implemented on a 2D grid, and for which single qubit gate can be done by sending signal in the appropriate (line,column) coordinate, the power would contain a term proportional to $\sqrt{Q_P}$. But even in this case additional terms proportional to $Q_P$ could be expected.}. A scaling proportional to $Q_P$ comes from the fact that the number of cables and amplifiers (amplifier cannot be shutdown when not used, thus they are within the passive costs) is usually increasing proportionally to the \textit{total} number of qubits inside the computer. But in addition to passive costs, there are also the \textit{active} costs. They will increase the power consumption in a manner that is time dependent. The best example of that is the power associated to signals that are being sent to the qubits: they only have to be sent if an algorithm is running and this power might also vary in time within an algorithm\footnote{One concrete example is the power required to remove the heat dissipated into the attenuators: this heat will have to be evacuated only if a gate is acting on the qubits.}. Such power will usually correspond to the moment non trivial gates (i.e not the identity operation) are being applied.\footnote{We should emphasize that it is not always the case. Indeed, there exist schemes in which applying an identity operation on qubits has an energetic cost as it requires to send pulses to \textit{keep} a coupling constant to zero (otherwise the qubit might interact in an undesired manner with the other qubits) \red{cite}.} Here, we will assume that no power is required to implement identity gates, and that some other gates might require a negligible amount of power. We also consider that the algorithm is implemented with a \textit{primitive} gateset (any gate can be expressed as a combination of gates in this gateset). The gates requiring power within this gateset will enter in a family $\mathcal{P}_{a}$ (for power "active" gates), otherwise they will enter in the family $\mathcal{P}_{n.a}$ (for power "non-active" gates). Under those assumptions, the power consumption can thus be written as the following function:
\begin{align}
P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i,
\label{eq:physical_power_gen}
\end{align}
only the family $\mathcal{P}_{a}$ has to be considered for the active power consumption. Here, $a$ represent the power it costs \textit{per qubit} to run the computer. The family of coefficients $\{b^i\}$ represent the power it costs \textit{per active (physical) gate of type "$i$"}(the type of gate corresponds to the precise gate that is being implement: cNOT, Pauli etc) to implement it. The terms $N^{(i)}_{P,\parallel}$ is the number of gate of type $i$ that are activated at a given instant in the algorithm. This quantity in principle \textit{depends} on time (because it is an \textit{active} cost), but from now on, we will assume that we are only interested in the \textit{average} power consumption such that $N^{(i)}_{P,\parallel}$ should be understood as an \textit{average} number of gates activated in parallel.

%, and that all the different gates require the same amount of power \textit{per qubit} involved their dynamic in order to be activated. It means that the active cost will be proportional to the number of physical qubits \textit{actively} participating in the calculation in term of power consumption: $Q_P^{P^a_P} \equiv N_{P,\parallel}^{1qb}+2N_{P,\parallel}^{2qb}$, where $N_{P,\parallel}^{1qb}$ and $N_{P,\parallel}^{2qb}$ respectively represent the average number of single (excluding identity) and two qubit gates acting in parallel inside of the computer\footnote{We assume that all the primitive gates used in the algorithm are either single or two qubit.}. There is no reason to assume that different gates "consume" the same amount of power. But it could be reasonable in some case: the energetic cost to perform a quantum gate is not necessarily only due to the gate physics: it can also be related to the way the signals are generated. If the electronic generating the signals can be turned off when no gates are activated, and if it dominates the details of the gate physics, our assumption would be safe for instance. But as many of the hypothesis we are doing here, it is not strictly necessary, it will just allow us to get a simple and intuitive model on which we will make physical comments. Also, we will only be interested in "order of magnitude" estimations of the energetic cost which makes our hypothesis more legitimate. With those assumptions we deduce, for some coefficients $a$ and $b$: $P=Q_P a + Q_P^{P^a_P} b$. It is usefull to rewrite this expression by introducing the notion of \textit{power-activity} of the qubits. It is defined as
%\begin{align}
%P^a_P \equiv \frac{Q_P^{P^a_P}}{Q_P}
%\end{align} 
%and it physically represents the fraction of qubits that are actively participating in the power function over the total number of qubits (we remind that we reason with average values along the algorithm here). Using this quantity the power then becomes:
%\begin{align}
%P=Q_P (a + P^a_P b).
%\end{align}
%We will make use of that notion in a few paragraphs.

We talked about the expression of the power. Now we must discuss the quantity of noise introduced by the algorithm. In the previous sections we explained why we need a metric to quantify the noise (because it is easier to access than the probability of success of the algorithm), and we gave some conditions it must satisfy (it should have a nice interpretation in such a way that the success probability can be estimated or bounded by this quantity). One requirement that we can ask for the metric to make it suitable for theoretical calculations is that from its value on each individual gates we can bound it for the entire algorithm. It assumes that the effect of the noise is local: it is possible to define a quantum channel for each quantum gate\footnote{Which means in particular that the final quantum state of a given quantum gate can be deduced by the sole knowledge of the state it had at its input.}, and from that to find how much noise a given gate introduces. A typical property allowing it is to ask that:
\begin{align}
\mathcal{M}_P^{\text{exact}} \leq \mathcal{M}_P^{\text{bound}} \equiv \sum_i \mathcal{M}^{(i)}_{P},
\label{eq:sub_additivity}
\end{align}
where $\mathcal{M}_P^{\text{exact}}$ is the \textit{exact} quantity of noise introduced by the algorithm, $\mathcal{M}^{(i)}_{P}$ is an estimation of the quantity of noise introduced by each (physical) quantum gate. The way we will quantify the noise occurring in the algorithm will be based on the best estimation we can have of $\mathcal{M}_P^{\text{exact}}$: $\mathcal{M}_P^{\text{bound}}$. Of course the tighter the bound is to the exact value the better it would be. Then, our metric will be defined as $\mathcal{M}_P=\mathcal{M}^{\text{bound}}_P$ and will verify:
\begin{align}
\mathcal{M}_P=\sum_i N_P^{(i)} \mathcal{M}^{(i)}_{P}.
\end{align}
This property of bounding the quantity of noise is pretty standard to ask, see for instance \cite{gilchrist2005distance}. 
Now, we assume that we can define a clock speed for the algorithm. It means that the algorithm will be implemented in a finite sequence of primitive timesteps all of duration $\tau_P^{\text{timestep}}$. In all of those steps a \textit{unique} primitive gate will be implemented per qubit (or per two qubit if the gate is a two qubit one). The assumption that there is a clock speed is not equivalent to say that the duration to implement all the gates are the same. It just means that if a primitive gate happens to be faster than the timestep, the qubit will then follow an identity evolution until the end of the timestep: $\tau_P^{\text{timestep}}$ thus corresponds to the longest gate in the primitive gateset. Now, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth. This is because we will neglect the final measurements in order to simplify our discussions. Indeed they will have a negligible contribution to the power consumption because they are acting "at the boundary" of the algorithm: their contribution in term of active power consumption or noise will be low compared to all the other gates. It doesn't mean that we will not take into account the cost of measurement amplification: this is usually a \textit{passive} cost that we are going to model (but this will come in the next chapter). Using the depth, we have $N_P^{(i)}=D_P N_{P,\parallel}^{(i)}$, and we can then write:
\begin{align}
\mathcal{M}_P=D_P \left(\sum_{i \in \mathcal{P}_a} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P}+\sum_{i \in \mathcal{P}_{n.a}} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P} \right)
\label{eq:physical_metric_gen}
\end{align}
We notice from this expression that \textit{any} gate occuring in the algorithm might introduce noise. There is thus a difference between being active in term of power consumption and being active in term of information processing. For instance, an identity gate will not require any power consumption but it will introduce nonetheless noise in the computation.
%where $N_P^{(i)}$ is the number of the $i$'th (physical) gate type used in the algorithm and $\mathcal{M}^{(i)}_{P}$ the quantity of noise introduced by this gate. Assuming that all the gates bring an amount of noise proportional to the number of qubit they involve, we have:
%\begin{align}
%\mathcal{M}_P=(N^{\text{1qb}}_{P}+N^{\text{Id}}_{P}+N^{\text{2qb}}_{P}) \mathcal{M}^{(0)}_P,
%\end{align}
%where $N_{P}$ represents the total number of physical gates in the algorithm, and $\mathcal{M}^{(0)}_P$ the metric of each of those gates. In a similar way as what we did for the power, we can also introduce the notion of \textit{information-activity} of the qubits. We define it as:
%\begin{align}
%I^a_P \equiv \frac{Q_P^{I_P^a}}{Q_P},
%\end{align}
%where $Q_P^{I^a_P}=Q_P^{P^a_P}+N^{\text{Id}}_{P,\parallel}$ represents the number of qubits actively participating in the algorithm \textit{on an information processing basis}. We notice that $Q_P^{I^a_P} \neq Q_P^{P^a_P}$. This is because the identity gates in our assumption do not consume any power but introduce noise during the algorithm. 
%
%Now, we can express $I^a_P$ in a more usefull manner for our purpose: assuming that all gates last for the same amount of time, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth (in general we will always neglect the measurements gates in our energetic estimations). Using this, we deduce: $N_{\text{gates}}=Q^{I^a_P}_P D_P$ and thus:
%\begin{align}
%\mathcal{M}_P=D_P Q_P I^a_P \mathcal{M}^{(0)}_P.
%\end{align}
%We see from this expression that $I^a_P$ can then also be interpreted as the portion of "information-active" \textit{gates} there are inside the algorithm over the maximum number of information-active \textit{gates} there could exist for the provided values of $D_P$ and $Q_P$: $D_P Q_P$. This fact and more detailed explanations are provided in the caption of figure \ref{fig:power_information_activity} \textbf{a)}.
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.9\textwidth]{chapter4/images/power_information_activity}
%\caption{\textbf{a)}: An algorithm implemented on four qubits having a depth equal to four. The stars represent identity operations. The square and rectangle represent power-active gates (cNOT, single qubit rotations etc). Each qubit are being measured after the last gate on them have been applied. The blue "area" of the circuit represent the information-active part of the circuit. Because some qubits can be introduced later or measured earlier than at the very beginning or very end of the algorithm, this area is smaller than $Q_P D_P$. \textbf{b)}: An equivalent description of the algorithm when we averaged in time all the dynamic. This description is equivalent in the sense that the average power and metric will be the same as for the "real" algorithm: it is a simpler representation to consider in order to make energetic estimations. We see that $I^a_P$ can be computed by either calculating the ratio of the blue area over the area $Q_P D_P$, either by calculating the average number of information active qubits divided by $Q_P$.}
%\label{fig:power_information_activity}
%\end{center}
%\end{figure}
%\FloatBarrier

\subsubsection{Physical interpretations}
At this point the general models for both power and metric are defined. We now summarize and interpret physically what we introduced. First, the power consumption is composed of a passive cost which is here whatever the gates are implemented on the computer. In addition to that there is an active cost which will only be here if gates that require power (which usually exclude the identity gates) are being implemented. This is why knowing the number of qubits inside the algorithm is not enough, one has also to know the number of gates that are actually being implemented as they will \textit{actively} participate in term of power consumption. 

Also, each gate participating in the algorithm "brings in" noise. The more gates are implemented, and the longer it lasts, the more noise there might have. This is represented by the fact $\mathcal{M}_P$ increases if (for other parameter constant) any of the $N^{(i)}_{P,\parallel}$ increases, and by the fact $\mathcal{M}_P$ is proportional to $D_P$. We notice however that because the notion of activity can be different in term of information processing and power consumption, a different counting has to be done about the number of gates acting in parallel: some gates might not require power but will bring in noise. This is represented by the fact that the metric also involve a summation over $\mathcal{P}_{n.a}$.

Once those estimations have been done, the minimization under constraint can be performed as represented on the figure  \ref{fig:general_optimization_principle}.
% NE PAS SUPPRIMER: pour l'image
%\begin{align}
%P(\bm{\alpha},\bm{\beta})=\color{blue}Q_P\color{black}(\bm{\beta})\color{purple}a\color{black}(\bm{\alpha})+\sum_{i \in \color{purple}\mathcal{P}_a\color{black}}\color{blue}N^{(i)}_{P,\parallel}\color{black}(\bm{\beta})\color{purple}b^i\color{black}(\bm{\alpha})
%\end{align}
%\begin{align}
%\mathcal{M}_P(\bm{\alpha},\bm{\beta})=\color{blue}D_P\color{black}(\bm{\alpha}) \left(\sum_{i \in \color{purple}\mathcal{P}_a\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange} \mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha})\color{black}+\sum_{i \in \color{purple}\mathcal{P}_{n.a}\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange}\mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha}) \color{black}\right)
%\end{align}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{chapter4/images/general_optimization_principle2}
\caption{Overall principle of minimization of the power cost. The role of the different components participating to the energetic cost: the algorithm, the engineering part of the computer, the noise model (and the way it is quantified) are represented in blue, purple, orange respectively. They depend on two families of parameters $\bm{\alpha}$ and $\bm{\beta}$. The first one represents the tunable parameters in the physical architecture of the computer. It usually represents the tunable hardware parameters (qubit temperature, attenuation etc) but not only as the clock-speed could also be optimized and it would enter in this family. The second one represents the tunable parameters in how the algorithm is implemented, i.e how it is compiled, and how many qubits it requires.}
\label{fig:general_optimization_principle}
\end{center}
\end{figure}
\FloatBarrier
We see there that the algorithm, the quantity of noise and the engineering part of the model have clearly identified roles. The algorithm characteristics are described by the functions $Q_P(\bm{\beta}), N_{P,\parallel}^{(i)}(\bm{\beta}), D_P(\bm{\beta})$ and they will play a role both in the power and the metric. Indeed if we increase the number of qubits or the number of power-active gates, it will increase the power consumption of the computer. But it also play a role in the metric because longer algorithms, or algorithms that use a greater amount of gates active in parallel will be noisier. Then, the functions describing the power cost (per qubit or per power-active gate) are represented by the functions $a(\bm{\alpha})$ and $b^j(\bm{\alpha})$. Those functions will for instance represent the power efficiency of the cryogenic to remove the heat, how much heat the amplifiers are dissipating, what is the power of the pulse driving the quantum gates, etc. We can say that they represent the characteristics of the engineering aspect behind the computer and will thus only be involved in the expression of the power function. The quantity of noise introduced by the quantum gates will on the other hand only play a role in the metric as represented by the orange color. In summary, each expertise required to build a quantum computer have very well defined parameters to characterize, someone "at the end" has to regroup them and to solve the minimization under constraint which will provide all the experts the optimum tunable parameters they should choose in their respective field of expertise.

We finish by one important remark. We can notice here that despite the fact the gates in the family $\mathcal{P}_{n.a}$ do not require any active power, they will participate in an \textit{indirect} manner to the power consumption. Indeed, they will modify the expression of the metric and thus change the value of $P_{\min}$. As a concrete example, it is frequent to try to minimize the number of identity gates inside algorithms because the metric would then be lower \red{cite}. But with our approach of finding the minimum power, we will see that sometimes it can be helpful to introduce such elements because they could to reduce the amount of active gate in parallel. This will be a concrete example of the fact that despite they do not "directly" require power, identity operations "indirectly" influence the energetic cost required to run an algorithm, and we are going to illustrate it right now.
\subsection{A simple example of algorithm optimization}
Now, we can design an example in which we will optimize the shape of an algorithm that is running, in addition to the family of tunable parameters $\bm{\alpha}$ that play a role for the metric and the "engineering" part of the model. We will stay with the same model of power consumption we considered in the single qubit gate example (only the power dissipated into the attenuator will play a role). Thus, with the vocabulary we introduced, we will neglect any \textit{passive} cost involved in the computation. For the noise model, we will keep the assumption that only the thermal noise will affect the qubit and we will model it in the exact same manner as before. For the metric quantifying this noise, we will consider the worst-case infidelity of the gates as it verifies the property \ref{eq:sub_additivity} (the average infidelity wouldn't satisfy this property for instance \cite{carignan2019bounding}). Also as we are going to see we will only need two qubit and identity gates in the algorithm. The two qubit and identity gates will be assumed to last for a duration $\tau^{\text{timestep}}_P=25ns$. As we are going to keep the same noise model for each qubit as the one we introduced in the section \ref{sec:single_qubit_example}, the identity gates will be as noisy as a single qubit $\pi$-pulse (lasting $25ns$), and the two qubit gates twice as noisy as the identity gates (because two qubits are involved in their dynamic, and because they last for the same duration). Those two qubit gates will also require twice the power consumption of a $\pi$-pulse because they involve two qubits (identity gates will be "power free"). Of course there is nothing obvious behind this it is just a simple way to model the power consumption and noise behind the gates we used. This $\pi$-pulse will have the same properties than the one used in the previous section\footnote{It means that $\gamma_{\text{sp}}=1kHz, \tau=25 ns$}. Thus in this simple example we will have $\mathcal{P}_{a} = \{\text{2qb}\}$, $\mathcal{P}_{n.a} = \{\text{Id}\}$, $P=Q_P a +N^{(\text{2qb})}_{P,\parallel} b^{\text{2qb}}$ with:
\begin{align}
&a=0\\
&b^{\text{2qb}}=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A (2 \times P_g),
\label{eq:power_nisq}
\end{align}
and $\mathcal{M}_P=D_P \left(N_{P,\parallel}^{(\text{2qb})} \mathcal{M}^{(\text{2qb})}_{P}+N_{P,\parallel}^{(\text{Id})} \mathcal{M}^{(Id)}_{P}\right) $, with:
\begin{align}
 \mathcal{M}^{(\text{Id})}_{P}=\mathcal{M}^{(\text{2qb})}_{P}/2=(1+\overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(300)}{A}) \gamma_{\text{sp}} \tau_P^{\text{timestep}}.
\end{align}
We recognize $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})+\overline{n}_{\text{BE}}(300)/A$ in this expression. We also see that we assumed $A \gg 1$ (as it will anyway be necessary to reach $\mathcal{M}_P=\mathcal{M}_{\text{target}}$ in what follows). We will ask an accuracy being $\mathcal{M}_{\text{target}}=1/3$ which implies that the fidelity of the algorithm output will be better than $2/3$ (because the metric is a pessimistic estimation: the "real" output fidelity will be better than the worst case one\footnote{And also because as explained before, the expression of $\mathcal{M}_P$ is only a bound on the exact value of the worst-case fidelity of the algorithm.}). 

Now, we need to describe the algorithm which will give us access to the average number of gate acting in parallel and $D_P$. For this example, we will consider running the quantum Fourier transform that we already introduced in the previous chapter. It will be directly implemented on physical qubits (not error correction yet). Of course, such algorithm is unlikely to be applied in the next few years on NISQ platforms as qubits are way too noisy: the task it would solve would be easily solved by a classical computer. But we take this as a simple example of the principle which could then be applied to more relevant NISQ (and also fault tolerant) algorithms. In order to simplify the discussion we will remove all the Hadamard gates that are required in this algorithm (they wouldn't change the general behavior we are going to show). The algorithm is represented for $5$ qubits on the figure \ref{fig:qft_5qubits}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/qft_5qubits}
\caption{\textbf{a)}: The QFT (where Hadamard gates have been removed for simplicity) performed on $5$ qubits with no compression. The vertical dotted lines represent the different timesteps of the circuits. On some of those timesteps, some qubits are waiting as represented by the stars indicating the associated "identity gates". Some other qubits are participating in a two qubit controlled-phase gate (which we described in the previous chapter). To reduce the level of noise, we can compress the circuit. It can be done by moving toward the left the different subcomponents represented by the colors (black, gred, yellow and blue). The red arrow represents how to do the first level of compression represented on \textbf{b)}. The red, yellow and blue subcomponents are pushed toward the left for two timesteps to put the first red two qubit gate inside the red dotted rectangle (removing the identity gates that were there). \textbf{b)}: First level of compression. The red, yellow and blue circuits have been pushed toward the left such that the first red two-qubit gate is done during the third timestep in parallel of the two qubit gate performed between the first and fourth qubit. \textbf{c)}: Second level of compression. The yellow subcomponent has also be pushed on the left (inside the yellow dotted rectangle) to reduce even more the algorithm duration and thus the noise. No further compression are possible. We can thus define a compression level for any size of QFT: $\epsilon=N_{\text{comp}}/N^{\max}_{\text{comp}}$ where $N_{\text{comp}}$ is the number of compression done and $N^{\max}_{\text{comp}}$ the maximum one (which is equal to $2$ in this example).}
\label{fig:qft_5qubits}
\end{center}
\end{figure}
As we see there are different way to actually implement it. Either we run the algorithm in an "uncompressed" manner as on the figure \ref{fig:qft_5qubits} \textbf{a)}, either we try to compress its length in such a way that the moments where qubits are waiting is minimized (on \textbf{c)}). The standard vision to implement algorithms is to make them the shortest possible. Indeed doing things this way the quantity of noise that is introduced is then minimal. But it might not be the best way to do things in order to minimize power consumption \textit{under the constraint} of aiming a targetted fidelity. Indeed, if the algorithm is highly compressed then a lot of gates are running in parallel which induces a big amount of active power consumption. More precisely, in this regime, the noise might be low (which implies that the qubits can be at higher temperature), but the heat dissipated in the attenuators will be high. Thus on one hand the power cost is minimized because the Carnot efficiency is higher, but we have more heat to evacuate. In the other limit it is the opposite. If the algorithm is minimally compressed (i.e more qubits are waiting), the noise will be higher (the qubits have to be colder) but the heat dissipated will be lower. In the end, the optimal way to compress the algorithm is not obvious if one wants to minimize the power consumption. To choose the optimal way we should compress the algorithm, we then introduce the parameter $\epsilon \in [0,1]$. It is defined as the number of compression it is possible to do over the maximum number of compression we can do: $\epsilon=N_{\text{comp}}/N_{\text{comp}}^{\max}$. The exact definition of a compression is given in the caption of the figure \ref{fig:qft_5qubits}. The other parameters we will optimize will be as previously $T_{\text{Q}}$ and $A$.
 
%It brings us to the last point: we explained which noise model, metric and resource to minimize (the expression of the power). The last thing to provide is the set of parameters on which the optimization can be performed. We are interested in the minimum power to implement this algorithm assuming that we can tune $T_{\text{Q}},A$ and $\beta \in [0,1]$, where $\beta \in [0,1]$ is the compression level which is defined in the caption of figure \ref{fig:qft_5qubits}. They are thus the parameters on which the optimization should be performed. But to get intuition behind the role of the compression factor, we will calculate the minimum power, minimized on the set $\bm{\alpha}=\{T_{\text{Q}},A\}$ for different values of $\beta$, and we will see for which value of $\beta$ the curve reaches a minimum. 

We now represent the minimum power consumption (minimized on $T_{\text{Q}},A$) as a function of $\epsilon$ in order to visualize the influence of the compression. It is represented on the figure \ref{fig:min_power_fct_compression}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/min_power_fct_compression}
\caption{Minimum power for a QFT implemented on $30$ qubits (minimized on $T_{\text{Q}},A$) as a function of the compression factor $\epsilon$. Bottom left inset: zoom around the minimum. Upper right inset: optimal temperature $T_{\text{Q}}^{\text{opt}}$ as a function of the compression factor. On this curve, we see that the algorithm should be implemented with a compression factor about $\epsilon^{\text{opt}} \approx 0.75$. The bigger the compression is, the higher the temperature can be which improves the Carnot efficiency. But at the same time, more power-active gates are implemented in parallel which dissipates more heat into the attenuators. The optimal compression factor results from this competition.}
\label{fig:min_power_fct_compression}
\end{center}
\end{figure}
\FloatBarrier
In this curve, we see that as expected there is an optimal compression factor on which the algorithm should be implemented in order to minimize the power consumption. It results from the competition we just described. This curve has been represented for a QFT implemented on $30$ qubits but when we increased the size of the QFT, the same kind of behavior remained: there were an optimal compression factor to choose resulting from the competition between noise and power. We also see that the optimization can be quantitative: the curve varies on more than one order of magnitude on the range of compression factor we considered. We could however consider that the conclusion of this curve is that the algorithm should anyway be close to a maximum compression (the power for a maximal compression would not be much higher than the minimum). But in practice we can expect the conclusion to be very system dependant: it highly depends on the characteristics of the algorithm implemented, the engineering aspect behind the computer, the noise model behind the quantum gates and the metric used to quantify it. We mainly took this specific example of the QFT because we already introduced the algorithm (and we will reuse it later on). 

The message we want to give here is simply that it is possible to optimize algorithms to make them minimize the power of the computer, and this minimization should at the same time involve the physical "hardware" parameters describing the computer. Here we took the simplest possible example which consisted in adding or removing identity operations, but the overall principle would remain if a given algorithm can be implemented in various manner. For instance, if different kind of gates can be used: some consume low power but introduce a high noise (and reciprocally), the optimal way to compile the algorithm could be deduced allowing to introduce energetic considerations in algorithm compilation problems.
\section{Adapting the framework for fault tolerance}

Now, that the concepts have been provided for a computer not using quantum error correction, we would like to adapt them to fault tolerant quantum computing. This is the role of this section where we will consider a complete "full-stack" model of fault-tolerant quantum computer, which means that we will try to have an entire description of the components that participate to the energetic balance: the electronic amplifying or generating the signals, the heat conduction in the cables, etc. One of the reason why we wanted to focus our detailed analysis to the fault-tolerance regime are because we will keep simple assumptions for the noise model: only the thermal noise will act. This assumption of having such good qubits should be more appropriate for the moment fault-tolerant quantum computing will be available. Also, we believe that the problematics of energetics for NISQ computing are probably not as crucial as for fault tolerance. Indeed, between hundred of thousands of to potentially billions of physical qubits might be required to achieve quantum supremacy in an error-protected quantum computer. Optimizing the computer to make it energy efficient is then much more crucial than for a computer composed of less than a thousand qubits. Also, the role of noise is not entirely clear for variational algorithms which are frequently used in NISQ \red{cite}. Indeed, sometimes the presence of noise can help the algorithm to find a better answer or to converge to the solution faster \red{cite}. This is not something that can be catched in the general assumption we did where the noise is necessarily an enemy. Our approach could however potentially be adapted in those cases: we discuss all this in further details at the very end of this chapter. All those reasons explain why we decided to focus on fault-tolerant quantum computing for the full-stack scenario.

\subsection{Adapting the concepts to fault tolerance}
To begin with, we must explain what changes if we consider fault tolerance. What are the implications of that in the estimation of the power function or the metric quantifying the noise introduced by the algorithm. Ideally, we would like to keep the same interpretation of those quantities and replace all the physical quantities such as physical depth, number of qubits, power and number of active parallel gates by their logical equivalent. Under some approximations it is possible to do so.
\subsubsection{Metrics on the logical level}
Let us talk about the metric first. For that, we will use the tools that we already introduced: the probability of error of a logical gate\footnote{We remind that in general $p_L$ has not necessarily the interpretation of a probability, in more general case it is a mathematical norm (which can usually be related to a probabilistic interpretation). It will be the case if the noise model behind the physical gate is probabilistic. To keep the explanations simple we nonetheless assume the probabilistic interpretation to be appropriate.}. Calling it $p_L$, the probability that any of the gate in a computation composed of $N_L$ logical gates fails is simply $N_L p_L$. The implicit assumption here is that all gates have the same failure probability. This is not true but fault tolerance very frequently reason on worst-case scenario (because more accurate estimations are complicated). Thus, here, $p_L$ actually corresponds to the probability of failure of the "worst" logical gate: $N_L p_L$ is an over estimation of the probability of error that will be our estimation of the quantity of noise introduced in the algorithm. In some sense, considering the algorithm as a big logical gate, $p_L$ will play the role of what measures the quantity of noise in a (logical) gate, and will verify the sub-additivity property \eqref{eq:sub_additivity}. Because of that the general description we did is still valid on the logical level, and we have a particular case of \eqref{eq:physical_metric_gen}:
\begin{align}
&\mathcal{M}_L=D_L \left(\sum_{i \in \mathcal{P}_a \cup \mathcal{P}_{n.a}} N_{L,\parallel}^{(i)} \right) \mathcal{M}^{(0)}_{L}\\
&\mathcal{M}^{(0)}_{L} = p_L
\end{align}
With that, we notice that the metric we used before is simply switched on the logical level. Everything behave in the exact same manner.
\subsubsection{Power on the logical level}
Now, we can talk about the power part of the problem. One question is to wonder if it is possible to define it in an "effective manner" on the logical level. Can we just replace all the physical quantities entering in this expression by their logical counterpart and keep the same interpretation ? To answer this question, we need to find the expression of the power (thus breaking down the fault-tolerant algorithm into its physical components) to try to then "recognize" the logical components with the hope that it can lead to a nice expression. The first step will thus be to estimate the number of physical components (qubits and gates) that are required in a fault-tolerant algorithm. This is the role of this section. 

\textbf{Reminding the general construction behind FT logical gates}\\
To begin, we need to remind the how a level-1 logical gate is constructed from physical elements, more precisely, a 1-Rec as defined in the chapter 2. It is represented for a single qubit logical gate on the figure \ref{fig:steane_method_full_ch4}. The construction of a two qubit logical gate such as a cNOT follows the same structure excepted that error correction will be performed on the two logical data qubits.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/steane_method_full}
\caption{Fault-tolerant implementation of a single qubit logical gate for one concatenation, based on Steane method. Each horizontal line represents a logical qubit for one concatenation level, composed of seven physical qubits (because we use Steane code). The first line represents the logical data qubit: i.e the logical qubit participating in the calculation. The four bottom line are the four \textit{ancilla} logical qubits that are required to implement fault-tolerantly the error correction. We need at least (further details in the text) two syndrome ancilla (which are interacting with the logical data qubit to measure the syndrome), and two verifier logical ancilla (which are here to check that the syndrome ancilla do not contain error that could damage the data qubits). The preparation procedure for the ancilla qubits is represented on the figure \ref{fig:preparation_0logical_ch4}.}
\label{fig:steane_method_full_ch4}
\end{center}
\end{figure}
\FloatBarrier
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/preparation_0logical}
\caption{Preparation of the $\ket{0_L}$ logical state. The preparation of the $\ket{+_L}$ logical state can be done via a similar procedure where (i) the direction of all the cNOT is being reversed (ii) four hadamard are added on the four qubits not affected by Hadamard here, right after their initialization in $\ket{0}$, (iii) the three Hadamard of this figure are being removed.}
\label{fig:preparation_0logical_ch4}
\end{center}
\end{figure}
\FloatBarrier
The role of each of those components has already been explained in the second chapter of this thesis, but we briefly remind them. The unprotected "naked" logical gate is implemented right before the purple box. It is implemented by a transversal implementation of the gate (i.e if the logical gate is Hadamard, the 1-Ga is implemented by applying a Hadamard on each physical qubit). It is then followed by quantum error correction which requires two "syndrome" logical ancilla corresponding to the second and third black lines. Their role is to detect $X$ and $Z$ errors occuring on the data qubits to know which appropriate correction should be implemented. The correction can then be applied. However, it is not strictly a requirement in practice: indeed it is enough to "keep track" of the errors with a classical computer, more precisely to keep in memory the result of the syndrome\footnote{In principle the correction only must be applied only before the non-transversal gates which are done through a different procedure as the one shown on figure \ref{fig:steane_method_full_ch4}. We come back on that point later.}. This is why in the calculations we will not include the cost of the correction following the syndrome\footnote{\red{Comment about magic gate for this}}. Now, for the construction to be fault-tolerant, verifier logical ancilla are required and represented by the third and last black line. They are interacting with the syndrome logical ancilla before being measured. This measurement is here to ensure that the potential faults that might have occured during the preparation of the syndrome ancilla will not corrupt the logical data qubit. Given the value of this measurement, the syndrome ancilla will either be accepted (and interact with the data qubit to detect the potential errors), or will be rejected. In the scenario it is rejected, new verifiers and syndromes ancilla have to be generated until the moment the verification succeeds. In principle, "many" syndromes and verifiers ancilla have to be prepared in parallel so that one will always be accepted when needed. In practice, the extra amount of those ancilla required will be negligible. Indeed based on the fact that it is more probable for an ancilla to be accepted, the extra amount of ancilla one would need to prepare in the case of failure will be much smaller than the number of ancilla we would need in case the acceptation always succeeds. It will then be possible to neglect them in our energetic estimation (we prove this more rigorously later in this chapter). In the end, this circuit, drawed for each logical gate we want to implement, and the principle behind the concatenation is all what we need conceptually to deduce the number of physical qubits and gates that are required in a 1-Ec after $k$ level of concatenations. The exact counting of the number of physical element will differ for each logical gate one want to implement but the principle will be the same.

We show the principle of the calculation for a single qubit logical gate and single qubit identity gate. What we refer as single qubit physical gate will either be Pauli or Hadamard (in our energetic estimation we will identify those gates as if they were the same). We assume that we want to implement a 1-Rec for such single qubit logical gate. Assuming that the syndrome ancilla are always accepted, we need $7 \times 5 = 35$ physical qubits: $7$ for the logical data qubit, $7 \times 2$ for the syndrome ancilla qubits and $7 \times 2$ for the verifier ancilla qubits. We can also find the number of physical gates required. In order to make this counting, we assume that we can only do measurement in the computational basis ($Z$-measurement): measuring in the $X$ basis requires to apply Hadamard gates before a $Z$-measurement. We also assume that qubits can only be available in their ground state $\ket{0}$ (preparing $\ket{+}$ requires to apply an Hadamard on $\ket{0}$). With those assumptions we find that we need $7 \times 4+9 \times 4=64$ cNOT: $7 \times 4$ for the transversal implementation of the cNOT represented on the figure \ref{fig:steane_method_full_ch4}, and $9 \times 4$ for the preparation of the $\ket{+_L}$ and $\ket{0_L}$ states for the ancilla (see figure \ref{fig:preparation_0logical_ch4}). For the measurement gates, we need $7 \times 4$ of them to measure all the ancilla. We also need single qubit gates: $7$ for the transversal implementation of the gate on the logical data qubit, $7 \times 2$ Hadamard to apply before the $X$-measurement (because we can only to $Z$-measurements), and $3 \times 2 + 4 \times 2 = 14$ Hadamard for the preparation of the ancilla states as explained in the caption of figure \ref{fig:preparation_0logical_ch4}. It gives us $35$ single qubit gates to apply. We also need to make some qubits necessarily wait at some point. For instance, the syndrome logical qubit has to wait for the measurement outcome of the verifier to know if they can be injected or not: they are then doing a noisy physical identity. We won't go in the detail of this counting but in the end, we would find $36$ physical identity gates by looking at all the places the physical qubits composing the logical ones necessarily have to wait. In the end, doing an appropriate counting for each type of logical gate that has to be implemented, we have access to the table \ref{table:FT_gate_breakdown} which represents for each level-1 gate (on the line), the number of physical elements (on the column) its 1-Rec is composed of \footnote{To be very precise, the 1-Rec of a measurement is defined as 1-Ec followed by 1-measurement (the 1-Ec is "before" the naked gate). This is defined this way for theoretical reason to prove the threshold. As we are interested to find the number of physical elements when concatenating, the elements in this 1-Ec would already have been counted by the gate before the measurement such that here we assume the 1-Rec associated to a 1-measurement as only composed of the naked measurement gate.}. We see from this table that as we could expect, a logical identity is the same as a logical single qubit gate excepted that the transversal operation is composed of identity gates. This is why it contains $7$ less single qubit gate but $7$ more identity gates than a logical single qubit gate.
\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
	\hline
	& lvl-0 cNOT & lvl-0 Single & lvl-0 Identity & lvl-0 Measurement\\
	\hline
   lvl-1 cNOT & $135$ & $56$ & $72$ & $56$ \\
   \hline
   lvl-1 Single & $64$ & $35$ & $36$ & $28$ \\
   \hline
   lvl-1 Identity & $64$ & $28$ & $43$ & $28$\\
   \hline
   lvl-1 Measurement & $0$ & $0$ & $0$ & $7$\\
   \hline
\end{tabular}
\caption{Each row lists a FT logical gate and tabulates the lower level components required for the listed gate as columns. Those level-0 components are thus physical gates. The single qubit gates here are either Hadamard or Pauli gates.}
\label{table:FT_gate_breakdown}
\end{center}
\end{table*}
\FloatBarrier
\textbf{Estimation of the number of physical gates acting in parallel}\\
This table allows us to deduce, based on a recursive reasoning the number of physical qubits and gates of each type that are required for a level-k logical gate. Let us start with the number of physical gates. We assume that we have $N_L^{\text{cNOT}}$, $N_L^{\text{1qb}}$, $N_L^{\text{Id}}$ logical cNOT, single qubit and identity gates on the algorithm, and $0$ measurement gates. We assume $0$ measurement gates here because (i) we will only be interested in the average number of gates acting in parallel in a few paragraphs (the measurement gates are at the boundary and will count for a negligible portion of gates), and (ii) as we will assume the active cost to measure (i.e the cost to send the readout pulses) to be negligible in comparison to performing a single or two qubit gate\footnote{But we will take into account the passive cost associated to the amplifier amplifying the readout signals. This is a passive cost because amplifier cannot usually be dynamically turned on and off.}, for this reason, we will always neglect the number of measurement gates in our energetic estimations. We put the number of logical gates required by the algorithm in a three dimensional vector $X_0=(N_L^{\text{cNOT}},N_L^{\text{1qb}},N_L^{\text{Id}} )^T$. We can deduce the number of physical gates of each type after $k$ level of concatenations via the recursive formula $X_k=A^k X_0$, where:
\begin{align}
& A=\begin{pmatrix} 135 & 64 & 64 \\ 56 & 35 & 28 \\ 72 & 36 & 43 \end{pmatrix}.
\end{align}
The formula for $k=1$ is just applying the table \ref{table:FT_gate_breakdown} to the number of gates implemented in the algorithm (removing the measurement from the counting for reason explained above). It gives us the number of physical gates after the first concatenation level. Each of them are then "promoted" into 1-Rec for the second concatenation level: we just have to "reuse" this table another time on the vector $X_1=A X_0$. The same principle applies recursively for further concatenation levels which explains why $X_k=A^k X_0$. In the end, from the knowledge of the number of gates required by the algorithm, we can access the number of physical gates required in the algorithm for an arbitrary concatenation level. We deduce that we have the following \textit{total} number of physical gates required in the algorithm:
\begin{align}
X_k = \left(
\begin{array}{c}
 \frac{1}{3} 199^k (2 N_L^{\text{cNOT}}+N_L^{\text{Id}}+N_L^{\text{1qb}})+\frac{7^k}{3} \left(N_L^{\text{cNOT}} -N_L^{\text{Id}} - N_L^{\text{1qb}}\right) \\
 \frac{7}{48} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{48} \left(-14 N_L^{\text{cNOT}} -7 N_L^{\text{Id}} +41\  N_L^{\text{1qb}}\right) \\
 \frac{3}{16} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{16} \left(-6 N_L^{\text{cNOT}} +13 N_L^{\text{Id}} -3\ N_L^{\text{1qb}}\right) \\
\end{array}
\right)
\label{eq:number_physical_gate_k_concat}
\end{align}
We notice from this expression that two numbers seems to have a particular importance in this formula: $199$ and $7$ (they are the only two numbers elevated to a power $k$). They correspond to the two eigenvalues of the matrix $A$.  

Now, we are only interested in the \text{average} number of physical gate that are acting in parallel. In order to access it, we need to know the average number of gate acting in parallel for the ideal algorithm (for each type: single qubit, identity and two qubit gates). Putting those number in a vector $X_0 =(\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}})^T$, we can deduce the total number of physical gate inside a logical gate on a typical "average" algorithm logical timestep (one algorithm timestep correspond to the time it takes to execute any logical gate\footnote{Some logical gates can in principle be implemented faster than others. For instance a logical identity could only last for two timestep as the transversal implementation of the gate could be done instantaneously (as the qubits wouldn't evolve). But as we need to keep all the qubits "synchronized" the longest logical gate to execute should give the duration of a logical timestep of the algorithm (even though "smart" optimizations could be performed for specific algorithms in order to reduce slightly the algorithm duration).}). It naturally corresponds to \eqref{eq:number_physical_gate_k_concat} where we replace the number of logical gates by the number of logical gates acting in parallel ($N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb}\}$). Now, this is not exactly the average number of physical gates that are acting in parallel. Indeed, a logical timestep is composed of a given number of physical timesteps. More precisely, calling $\tau_P^{\text{timestep}}$ the duration of a physical timestep (which corresponds to the duration of the longest physical gate used in the FT construction: we will assume it corresponds to cNOT in what follows), we have after $k$ concatenations a logical gate that lasts for $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. Indeed, we can see from figure \ref{fig:steane_method_full_ch4} that for one level of concatenation, the logical data qubit are going through three timesteps: the first one corresponds to the transversal implementation of the gate, followed by two timesteps used to perform the syndrome measurement\footnote{We remind that we assume the correction is not physically performed as it is enough to }. Increasing the concatenation level, each of those timestep will again be multiplied by three. This is how we deduce $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. We notice here that the ancilla must however be prepared in advance: including their preparation and the moment they can be "plugged out", the duration of this gate would be longer. But as explained on the figure \ref{fig:timestep_logical_gate}, the good timescale to consider to estimate the average number of gates would still be $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/timestep_logical_gate}
\caption{Determination of the average number of physical gates acting on an average logical timestep. On the first line of this figure are represented a sequence of three logical gates that are composed of three physical timesteps as indicated by the three red rectangles (the transversal implementation, and the measurement of the $X$ and $Z$ syndromes). Those logical gates require ancilla which are represented on the line below by the matching colors. Between the moment the ancilla are prepared and measured, there is more than three timesteps (we represented $6$ here for simplicity). However, in order to compute the average number of physical gates acting in one logical gate, everything will behave \textit{as if} those gates were actually implemented in parallel of the $3$ timesteps. Indeed, the ancilla might have gates applied on them before ($1$ and $2$ red boxes) and after the logical gate ($6$ red box), but the preceding and following logical gates would exactly compensate those missing gates. Rigorously speaking, this is true if we neglect the boundary of the algorithm and if we are interested into the average number of gates acting in parallel (which is the case).}
\label{fig:timestep_logical_gate}
\end{center}
\end{figure}
\FloatBarrier
%Finally, calling $\tau_P^{\text{1qb}}$ and $\tau_P^{\text{cNOT}}$ the duration of the physical single and cNOT gates respectively, the average number of single and two physical qubit gates acting in parallel in the algorithm can be expressed as:
Finally, the average number of single and two qubit gates acting in this logical timestep is:
\begin{align}
&\overline{N}_{L,\parallel}^{\text{1qb}}(k)=N_{\text{during } \tau_L}^{\text{1qb}}(k) /3^k
\label{eq:average_number_physical_single_cNOT_timestep1}\\
&\overline{N}_{L,\parallel}^{\text{cNOT}}(k)=N_{\text{during } \tau_L}^{\text{cNOT}}(k)/3^k
\label{eq:average_number_physical_single_cNOT_timestep2}
\end{align}
Where $N_{\text{during } \tau_L}^{\text{1qb}}(k)$ (resp $N_{\text{during } \tau_L}^{\text{cNOT}}(k)$) is the number of single (resp cNOT) physical gates that are inside an average logical timestep, i.e the number of physical gates there are assuming that $\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}}$ are acting in parallel, where those numbers represent the average number of logical gate acting in parallel in the algorithm. We remind again that those numbers are simply obtained by replacing $N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb}\}$ in \eqref{eq:number_physical_gate_k_concat}
\begin{align}
&N_{\text{during } \tau_L}^{\text{1qb}}(k)=\frac{7}{48} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{48} \left(-14 \overline{N}_{L,\parallel}^{\text{cNOT}} -7 \overline{N}_{L,\parallel}^{\text{Id}} +41\  \overline{N}_{L,\parallel}^{\text{1qb}}\right)
\label{eq:average_number_physical_single_cNOT_timestep_final1}\\
&N_{\text{during } \tau_L}^{\text{cNOT}}(k)= \frac{1}{3} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{3} \left(\overline{N}_{L,\parallel}^{\text{cNOT}} -\overline{N}_{L,\parallel}^{\text{Id}} - \overline{N}_{L,\parallel}^{\text{1qb}}\right) 
\label{eq:average_number_physical_single_cNOT_timestep_final2}
\end{align}
We notice that the second parenthesis of those expression will become negligible to the first one so that the average number of physical single and cNOT gates acting in parallel verify:
\begin{align}
&\overline{N}_{L,\parallel}^{\text{1qb}}(k) \approx \frac{7}{48} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_single_cNOT_timestep_final3}\\
&\overline{N}_{L,\parallel}^{\text{cNOT}}(k) \approx \frac{1}{3} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_single_cNOT_timestep_final4}
\end{align}
%The ratios $\frac{\tau_P^{\text{1qb}}}{\tau_L^{\text{timestep}}}$ and $\frac{\tau_P^{\text{cNOT}}}{\tau_L^{\text{timestep}}}$ in \eqref{eq:average_number_physical_single_cNOT_timestep1} and \eqref{eq:average_number_physical_single_cNOT_timestep2} represent the  fact that the associated gate might be faster than the duration of the physical timestep (we have to take in account the fact that for a given physical timestep the gate will not always be activated, it will be important for power estimations). Now, as we will assume that the cNOT is the longest physical gate we will have $\tau_P^{\text{cNOT}}=\tau_P^{\text{timestep}} \Rightarrow \frac{\tau_P^{\text{cNOT}}}{\tau_P^{\text{timestep}}}=1$ in practice. The precise explanations for this are given in the caption of the figure \ref{fig:estimation_average_number_gates}.
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.7\textwidth]{chapter4/images/estimation_average_number_gates}
%\caption{How to estimate the average number of physical gates acknowleding the fact they can be faster than $\tau_P^{\text{timestep}}$. This image also represents the difference between physical and logical timestep (for $k=1$ because $\tau_L^{\text{timestep}}=3 \tau_P^{\text{timestep}}$ here). The duration of the physical timestep is given by the longest physical gate acting in the computer (which is not represented on this image). Each of the two "lines" on this figure represent a physical qubit on which single qubit gates represented by the black rectangles are being applied. There are $N^{\text{1qb}}=6$ of them. As the gates are faster than a physical timestep, the average number of single qubit gate acting in parallel is not given by $N^{\text{1qb}}/N_{\text{timestep}}=6/3=2$. Instead, we have to calculate the black area: $N^{\text{1qb}} \tau_P^{\text{1qb}}$ and divide it by the grey are \textit{covered by one physical qubit} (thus half the total grey area in this example). It gives: $\overline{N}^{\text{1qb}}_{\parallel}=N^{\text{1qb}} \tau^{\text{1qb}}_P/\tau_P^{\text{timestep}}$. To illustrate, we can consider the case in which the single qubit gate are lasting for the entire timestep (the black area would entirely cover the grey one). In this case we would find $\overline{N}^{\text{1qb}}_{\parallel}=2$ as expected.}
%\label{fig:estimation_average_number_gates}
%\end{center}
%\end{figure}
%\FloatBarrier 
 \textbf{Estimation of the number of physical qubits used in the computer}\\ 
Now, we can estimate the number of physical qubits required by the computer for $k$ concatenations. To understand the principle of the estimation, let us reason on an algorithm composed of a unique single qubit logical gate. In order to do the estimation, we first notice that the number of ancilla qubits dominate the total number of physical qubits required. Indeed, for $k=1$ for instance we would need $28$ (resp $28 \times 2$) ancilla qubits for a single or identity (resp cNOT) logical qubit gate. Compared to the $7$ to $14$ physical data qubits, as we are only interested in order of magnitude this is a fair approximation to make. Furthermore, increasing the concatenation level would only make the number of physical ancilla qubits dominate even more. For this reason, we will only try to estimate the number of ancilla qubits. Then, we remind that the $k$'th concatenation level is obtained from the $k-1$ level in which each physical gate has been promoted into a 1-Rec. Thus, we can estimate the number of physical qubits by counting the number of physical gates on the $k-1$ level, and by multiplying it by $28$ for the single qubit and identity gates, and $28 \times 2$ for the cNOT. It would give us access to the total number of ancilla qubit after $k$ concatenation, and thus roughly the total number of physical qubits. We notice that this calculation assumes that no ancilla qubits can be recycled within this logical gate after $k$ concatenation (i.e each gate needs "fresh" ancilla). The $X$-syndrome ancilla are participating to $9$ physical timesteps. Thus, in principle, we can reuse them once they have done those $9$ timesteps. In a similar way, the verifier ancilla can be reused (even earlier because they are used for a smaller amount of timesteps). Properly counting the number of ancilla that could be reused would however be a complicated task for an arbitrary concatenation level. Furthermore, in practice we will mainly be interested in the first $3$ concatenations levels in what follows. Because of that, the number of timesteps for the logical gates on the $k-1$ level is also equal to $9$: $\tau^{\text{timestep}}_L/\tau^{\text{timestep}}_P=3^{k-1}=9$ which means that anyway the level of recycling of the syndrome ancilla qubit would be "poor" (but we might be able to recycle roughly half of the verifier ancilla qubits). We assumed in the end that the ancilla qubits are not recycled within this logical gate which gives a slight overestimation of the total number of physical qubits that would really be required. The extension to an algorithm composed of not one single logical gate but actually $(N_{L,\parallel}^{\text{cNOT}},N_{L,\parallel}^{\text{1qb}},N_{L,\parallel}^{\text{Id}})$ cNOT, single and identity logical gates acting in parallel, the principle remains the same and we can estimate:
\begin{align}
Q_P(k) \approx \frac{28}{199} 199^k (2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}})
\end{align}
physical qubits.
Now, an algorithm is composed of many logical timesteps. The number of physical qubits required is actually given by the moment in the algorithm where there are the \textit{maximum} number of qubits that are actively participating in the algorithm (which is in some way the "bottleneck" in term of physical resources required). At this moment, we would have $2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}=Q_L$\footnote{To be very accurate, we should also include the measurement gates such that the formula is in general $Q_L=2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+N_{L,\parallel}^{\text{Meas}}$. But in order to not confuse the reader by introducing at this stage a number of measurement gates acting in parallel, we simplified the story. Anyway for the calculations we are going to do in practice, this is a detail that will not matter.}. Indeed, all the logical qubits are actively participating in the algorithm at this moment, and this equality can be intuitively understood from the figure \ref{fig:bottleneck_algo_physical_qubits}. We deduce that an estimation for the total number of physical qubits required by the computer is, for $k>0$\footnote{Following the same logic of the fact the ancilla cannot be recycled, in a very worst case scenario we would need $9$ time this number if the number of logical gates required is constant for the $9$ timestep around the bottleneck point. However as we believe it is a pessimistic estimation (some ancilla could be recycled), and because we were already pessimistic by the assumption of no recycling \textit{within} a logical gate, we did not take this $\times 9$ in the expressions.}:
\begin{align}
Q_{P}(k) \approx \frac{28}{199} 199^k Q_L
\label{eq:number_physical_qubits_from_logical}
\end{align}
This formula does not apply for $k=0$ as it is based on estimating the total number of physical qubits from the number of ancilla qubits. And there are no ancilla qubits when no concatenations are performed.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/bottleneck_algo_physical_qubits}
\caption{How the number of qubits is related to the maximum number of gates acting in parallel. On this figure, we illustrate an algorithm composed of two and identity gates (we actually recognize the QFT performed on $5$ qubits). We notice that the number of qubits required by the algorithm (here they appear to be logical ones) is equal to $2 \overline{N}_{L,\parallel}^{\text{cNOT}} + \overline{N}_{L,\parallel}^{\text{1qb}}+\overline{N}_{L,\parallel}^{\text{Id}}$.}
\label{fig:bottleneck_algo_physical_qubits}
\end{center}
\end{figure}
\FloatBarrier
\textbf{Expression of the power}\\
Now, we can regroup the different thing we calculated to express the power on the logical level. On the physical level, it is a function: $P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i$ where $\mathcal{P}_{a}$ correspond to the power-active gate (that we assume here to be $\mathcal{P}_a = \{\text{1qb},\text{cNOT}\}$). Thus, from \eqref{eq:average_number_physical_single_cNOT_timestep_final3}, \eqref{eq:average_number_physical_single_cNOT_timestep_final4} and \eqref{eq:number_physical_qubits_from_logical}, we have here:
\begin{align}
&P=Q_L u(k) a + \left( b^{\text{1qb}} v(k) + b^{\text{cNOT}} w(k) \right) (N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}})\\
& u(k) \equiv \frac{28}{199} 199^k\\
& v(k) \equiv \frac{7}{48}\left(\frac{199}{3}\right)^k\\
& w(k) \equiv \frac{1}{3} \left(\frac{199}{3}\right)^k
\label{eq:logical_power}
\end{align}
We are thus able to define the power on the logical level with some adaptations. Indeed, we notice here the functions $u$,$v$,$w$ that are represent the increasing cost of the logical element when more and more error correction is being performed. They are the "translation" of the energetic cost from the logical to the physical world (where the power is "really" taken). We notice that $v$ and $w$ are both growing following the same law $(199/3)^k$. The reason is that as soon as one concatenation has been performed, there will have at the same time single and cNOT physical gates.... We also notice that $u(k)/v(k)$ and $u(k)/w(k)$ go to $0$ in the infinite concatenation level. This is based on our assumption that the ancilla qubits are not being recycled within a logical gate. Because of that, the passive cost will dominate in the $k \to \infty$ limit. In practice we can expect that with smart recycling scenario, those ratio would actually converge to some constant. \red{continuer: expliquer le $\times 2$ en face du cNOT logique et comparer au cas physique, approximer $v(k) \approx w(k)$, expliquer la generalite ou non des resultats et rappeller les approx necessaires pour arriver la.}

We also notice that th

 
\red{at this point, we computed the total number of qubits and gates acting in parallel after $k$ level of concatenation for an arbitrary algorithm}.
\subsection{Engineering model}
Now that we explained the main things that change when considering fault-tolerance. We would like to apply our calculations into a realistic model of quantum computer. In practice the "only parameters" we need to determine are thus the associated engineering parameters $a$, $b^{\text{1qb}}$ and $b^{\text{cNOT}}$ in \eqref{eq:logical_power}. This is what we are going to determine explicitely.
\subsubsection{The global picture}
Following the same philosophy than we did in the examples at the beginning of this chapter, we will only consider the energetic cost related to cryogenics. Thus, any energy spent outside (i.e at $300K$) will be considered as "free" in our estimation. The reason why we focus on the cryogenic cost is because as any power that is spent inside is usually transformed into heat that then has to be evacuated. Then, because removing $1W$ of heat will cost more than $1W$ of work (i.e electricity) at cryogenic temperatures (we can think about Carnot efficiency), focusing on the cryogenic cost would give the dominant power consumption\footnote{Of course if some elements at $300K$ consume a lot of power, they might dominate the cryogenic cost. But in practice, we believe that the dominant power consumption will anyway be related to cryogenics.}. Now, many different architectures of quantum computer could exist, we need to make some choices, we cannot be entirely general. One thing to have in mind is that a quantum computer should be seen as an hybrid quantum/classical computer. Indeed, classical electronic is required to generate the signals that will reach the qubit, but also to manage the execution of the quantum algorithm. For instance it has to keep in memory all the sequence of gates that have to be applied on the physical qubits. It must also perform some calculations that allow to deduce the value of the syndrome from the measurement outcomes. One open question is to know where it is optimal to put the electronic, in term of simplicity for the design but also in term of energy efficiency. Two extreme scenarios can be considered. First, we could imagine merging all the classical electronics with the quantum core. In this scenario the engineering would be much more simple (as it would remove a great number of cables). It would also remove the major part of heat conduction because we would only need one cable between $300K$ and the quantum core giving the instruction about which algorithm to perform\footnote{This is probably a little bit extreme but it is to give the idea: the number of cablesur required would be very small.}, and another cable extracting the measurement outcomes provided at the very end of the algorithm. However classical electronic dissipates an important amount of heat and if we assume putting it at the qubit temperature (thus in the $10-100mK$ range), the quantity of heat to remove would be phenomenal: it would be an inefficient architecture. The other extreme is to put all the electronic at $300K$. In this case we face the opposite problem: we would need to bring an important amount of cables from the laboratory to the quantum core. They would bring a very important amount of heat to evacuate and it might not be very energy efficient either. All this explains why there are strategies considered as being better for the scalability which consist in putting the electronic that is generating the signals at some intermediate temperature between $300K$ and $T_{\text{Q}}$. We call this temperature $T_{\text{Gen}}$ and it is typically considered being around $4K$ \cite{bardin201929,patra2020scalable}; the aspects of information processing being kept at $300K$. Doing this strategy, an important amount of cable would be required between $T_{\text{Gen}}$ and $T_{\text{Q}}$, but the associated temperature gradient being lower, the heat flow would be less a problem\footnote{Typical heat conduction models involve a heat flow proportional to $T_a^i-T_b^i$ where $T_a$ and $T_b$ are the temperature of the two ends of the cable, and $i$ some positive power. Thus a low temperature gradient involves a low amount of heat conduction.}. Furthermore as soon as the cable is below $\approx 10K$, superconducting microwave cables can be used which are associated with a very low heat conduction flow. On the other hand, a much smaller amount of cables would be required between $300K$ and $T_{\text{Gen}}$ because those wires would only bring digitized information about which signal should be generated for which qubit (and those cable are typically optical fibers which are insulators and thus also associated to a low heat flow). 

In summary, here, we will consider a quantum computer where the electronic generating the signals will be \textit{inside} the cryogenic at a temperature $T_{\text{Gen}}$. Our goal will then be to optimize this temperature along with the qubit temperature $T_{\text{Q}}$, the total attenuation $A$ and the concatenation level $k$ in order to minimize the power consumption through our formulation of minimization under constraint.
\subsubsection{The architecture we consider}
Now, we give more precisely the elements we are going to consider in our energetic estimations. As explained before, as we reason with the cryogenic cost we have to know how much heat they dissipate which will tell us how much electrical power will be required to evacuated that heat. We will then perform some approximations that will allow us to neglect some of those costs. The architecture of the computer we consider is represented on figure \ref{fig:quantum_computer_archi_cable_with_lab}, let us list the sources of heat dissipation it contains.
\begin{description}
\item [Heat dissipation from signal attenuation:] We already introduced it. The signals must be attenuated in order to remove the thermal noise which introduces heat.
\item [Heat conduction in all the cables connecting to the qubits:] All the cables within the quantum computer are conducting heat. The associated heat load must also be evacuated by the cryogenic.
\item [Heat dissipation from signal generation:] Generating signals has an energetic cost that is usually higher than the energy contained in the generated signal. If the signals are generated inside of the cryogenics the heat the electronic dissipates has to be evacuated.
\item [Heat dissipation from signal amplification:] The typical amplitude of the signals containing the measurement results about the state of the qubits is low such that the thermal noise might be an issue when those signals will be read. In order for the signal to remain with a high signal over noise ratio, they must be amplified at low temperatures. This process dissipates heat.
\item [Heat dissipation for multiplexing and demultiplexing:] To reduce the heat introduce by the thermal conduction, one typical strategy is to perform multiplexing and demultiplexing. It consists into putting information that should be adressed to different components into a single cable. For digital signals, it requires some electronic that will "encode" (multiplex) data so that many information can be sent into one cable. It also requires after to "decode" (demultiplex) this data. The electronic performing those operations will cost energy and thus dissipate heat.
\item [Heat dissipation from Joules effect in DC cables:] The classical electronic that is put inside of the cryogenic requires a DC power in order to work. If an important amount of power has to be provided in those cables, Joules effect induced by the resistance of those wires might introduce heat that we will need to evacuate.
\end{description}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/quantum_computer_archi_cable_with_lab}
\caption{\textbf{a)} Architecture of the computer our engineering model is based on. \textbf{b)} The same model when negligible sources of heat dissipation have been removed.}
\label{fig:quantum_computer_archi_cable_with_lab}
\end{center}
\end{figure}
\FloatBarrier
The left part of the figure \ref{fig:quantum_computer_archi_cable_with_lab} 
comports all the elements there are inside the computer that are dissipating heat, they exactly correspond to the elements we listed. The right part is what we modelled in our calculation. For reasons we are going to give, we think that the elements we removed from the left graph (to build the right one) would contribute in a negligible manner to the total energetic cost. More precisely, we will consider that an item X introduces an energetic cost negligible compared to an item Y if the power required to remove the heat dissipated from X is lower \textit{or in the same order of magnitude} to what is needed for Y. Indeed, our main goal is to estimate the order of magnitude of power consumption that we could expect to run a fault tolerant computation, we will thus not really be interested to know if the power we find is exactly $1MW$ or $7MW$ for instance, but more if it is closer to $1MW$ or to $10MW$. This is the level of accuracy we are interested in. Here, we describe the exact architecture we considered and we will talk about the approximations we made after.

We first focus on the stage of temperature $T_{\text{Gen}}$ where signals are being generated. This stage is composed of various electronic components. For the quantitative values we are going to consider, we will consider that they are based on CMOS technology where experiments have shown that it is possible to put them at low temperatures \cite{patra2020scalable}. We first recognize elements that are called DAC (for Digital to Analog Circuit). Even though a unique DAC is represented here, one per physical qubit will be necessary. The role of a DAC is to generate the pulses that are going to drive the physical qubits. The way it works is that it receives a digital information describing the shape of the pulse to generate. This information will be received as a bit-string describing a discretized approximation of the exact envelope we wish to generate. This approximated discretized version of the signal is generated by the electronics and filtered to obtain a "smooth" envelope. Finally, this envelope is multiplied with a signal being at the qubit frequency: the local oscillator, and sent to the qubits, the pulse necessary to drive the quantum gate has now been entirely created. To be a little bit more precise, two enveloppes are actually generated, they are then multiplied by the local oscillator, and a $\pi/2$ dephased version of the local oscillator. Those two enveloppes allow to make possible to control the amplitude of the signal but also its phase which is necessary for single qubit operation where the phase of the signal plays a role in the axis of rotation of the gate implemented. Also, as all qubits are not necessarily at the same frequency, the DAC can also use the local oscillator and "shift" its frequency in order to create a signal having the appropriate frequency of the qubit to be driven: it has been shown to be possible in a recent proposal \cite{patra2020scalable} on which our order of magnitude of heat dissipation will be based on. In the end, we understand why it is called a DAC: from a digitized description of the signal it generates an analog one corresponding to the pulse that is going to drive the quantum gates. The ADC (Analog to Digital Circuit) does the opposite thing. It will "convert" the analog signals coming from the measurement outcomes of the qubits. Indeed, the information about the qubit state after a measurement will be contained in a propagating analog pulse. The ADC is able to interpret the characteristic of this pulse and to convert it into digital information. There is also one ADC per physical qubit that is required. Now,   In practice to drive qubits we must control the amplitude, but also the phase of the signals that are sent. The DAC  the amplitude the pulse should have for each instant of time. Both the amplitude and the time are discretized. Then, it generates signal The pulse is described through a discretized approximation, typically the time is discretized on a given number of bits, and for each time an amplitude (also discretized) is associated.  and it will then create We first recognize one element that we called DEMUX-MUX. Its role is to (i) demultiplex the instructions coming from the laboratory about which gate has to be performed on which qubit, and to transmit this instruction to the components that will generate the signals: the DAC. It is also (ii) multiplexing the data   the appropriate DAC that will in turn generate and send the signal in the microwave cables. It is also multiplexing the data coming from the multiple ADC. Those ADC are converting into digital information the readout measurements (which is analog as it is a pulse propagating in the microwave cable). The goal of multiplexing and demultiplexing is to reduce the number of cables required between the laboratory and the signal generation stage. In addition to those optical fibers, we need wires containing DC voltages that are here to provide to the electronic the power it requires. There is also one cable that will contain the local oscillator signal. This signal is an harmonic signal at the "central" frequency of the qubits. What we mean by central frequency is that the qubits might not all be at the exact same frequencies: this is actually something to avoid in practice to avoid issues such as crosstalk \red{cite}. The central frequency of the qubits is the one at the center of the bandwith on which all the qubits have their frequencies. It is typically about $\omega_0/2 \pi \approx 6GHz$ \red{cite} for transmons (and the total bandwidth can usually be about $\Delta f \approx 3 GHz$ maximum \red{cite}). The local oscillator is used by the DAC in order to generate the signals at the appropriate frequencies.

We also recognize two amplification stages in black colors: one is done at $T_{\text{Q}}$ with parametric amplifiers, while another one is done at $T_{\text{Amp}}$ with amplifiers based on classical CMOS electronic. Classical amplifiers also require a DC power cable represented in yellow. The parametric amplifier require a microwave signal. Those kind of amplifiers are amplifying the signal by introducing a minimal amount of noise during the process \red{Is what I say true in general ?}. They are made of superconducting components and do not dissipate heat by themselves. However the pump signal they require needs to be attenuated and introduce heat dissipation. Then, we can notice all the microwave cables: some ("Readout In") are used to inject the readout signal which is interacting with the qubit to be measured and then leaves the quantum core ("Readout Out"). It is on this "leaving part" that the signals are being amplified. We also have the microwave cables here to inject the resonnant pulses that will drive the single qubit gate ("X/Y drive"). In our approach, we assumed that the two qubit gates will also be performed by injecting appropriate signals in the X/Y drive. This is for instance the principle behind the cross resonant gate scheme \cite{chow2011simple}. By sending a signal on a qubit $A$ resonnant at the frequency of a qubit $B$ ($A$ and $B$ are related by a bus), a two qubit gate between them can be implemented. We notice the absence of "Z" line which corresponds to the line where signals are usually sent to change the frequencies of the qubits. Because we assume using the cross-resonant scheme (or a similar one that would only require to send signals on the X/Y lines to perform two qubit gates), we can consider that all the qubits inside the computer are at fixed frequencies so that we don't need such line.

Finally, we notice that in addition to the three black stages doing signal generation, containing the qubits and amplifying the signals (thus the stages "fundamentally" required for the computer to work), we added extra stages in blue. They are here to help evacuating in a more progressive manner the heat dissipated into attenuators and the heat conduction. What we mean is that if we considered an extreme scenario where we would only have the qubits and the signal generation stage (let us forget about amplification), there would have a big attenuator at $T_{\text{Q}}$ dissipating a lot of heat there. The heat conduction would also have to entirely be evacuated at $T_{\text{Q}}$. It would be very energy inefficient as the total quantity of heat to evacuate would entirely be removed at a temperature having a very poor Carnot efficiency. It explains why we added those "extra" blue stages: they will help to "benefit" of higher Carnot efficiencies: the heat is evacuated more progressively. In practice, we will consider in what follows three additional stages to $T_{\text{Q}}$ and $T_{\text{Gen}}$ and their temperature will be determined as a function of $T_{\text{Q}}$ and $T_{\text{Gen}}$. 
\subsubsection{Approximations leading to our model}
Now, we will make simplifications on the model represented on the left. The simplifications we are going to do will not be valid for all the range of parameters we will consider varying in the curves we are going to present, but they will at least be valid for the most important points on those curves that we will mainly discuss.

\textbf{We can neglect the heat conduction between $300K$ and $T_{\text{Gen}}$:}\\
Let us show first that the cables between the laboratory and the signal generation stage introduce a negligible heat flow on the signal generation stage compared to the heat dissipated by the classical electronic there (DEMUX-MUX, and DAC/ADC). In order to simplify the discussion, we first assume that \textit{only} the DAC/ADC are dissipating heat. We will come back on the DEMUX-MUX element after. The typical values of heat dissipation \textit{per physical qubit} for the DAC and ADC elements are in the milliwatt range \cite{bardin201929,patra2020scalable}, which is what we will consider here. The fact it is a consumption per qubit (and not per active gate) is the current state of art of the electronic. It is based on the fact that those elements will \textit{always} generate a signal to a given physical qubit (and the signal will be of zero amplitude if the qubit doesn't have to be driven). But it could be possible in principle to turn off the electronic when it is not being used, such that the consumption would be related to active costs. We will discuss it later on.

Now, we need to estimate if the heat flow associated to the cables going toward the laboratory will be negligible compared to the heat this electronic dissipates. We start by discussing the optical fiber (blue and pink data cables). We give some reference values to keep in mind (they are justified in the supplementary). The typical heat flow associated to a cryogenic coaxial cable composed of an inner metallic conductor is in the milliwatt range \textit{if} this cable is being put between $300K$ on one hand and $0K$ on the other hand. Optical fibers (blue and pink data cables on the figure) will be composed of insulator material so that they will conduct less heat than that. But to simplify we will reason with this worst case scenario where one data cable would conduct $1mW$ of heat between the laboratory and the signal generation stage. The question is then: how many of those data cables do we need ? The answer to that question is related to how much information per unit time would have to transit in them, and how much a typical optical fiber can transmit of data per unit time. We treat the first question. Every $\tau_P^{\textit{fastest}}$, which corresponds to the duration of the fastest physical gate inside the computer, the DAC has to generate a new signal for a physical qubit. We notice that $\tau_P^{\text{fastest}}<\tau_P^{\text{timestep}}$. Indeed for instance if the computer has to generate a single qubit gate, it will have to wait after this gate has been implemented for the end of the timestep. Then, with our assumption that the DAC are always enabled, they will "generate" a signal of zero amplitude, corresponding to the identity gate, at this moment. Then, we need to know how many bits of information are required to create a pulse. A reasonable value is based on the fact that a "good" pulse can be described with $16$ points in time\cite{bardin201929}, where on each time we can attribute a voltage amplitude encoded on four bits (thus, it corresponds to $16$ possible choice of voltage amplitudes). It gives a total amount of information to describe this pulse being $4 \times 16=64$ bits. And they have to be sent every $\tau_P^{\text{fastest}}=25 ns$. In the end, we obtain a quantity of information for each physical qubit that is: $64/(25ns)\approx 2.5 Gb/s$. Then, a good optical fiber can convey $25 Gb/s$ of information \red{cite}. It tells us that about one optical fiber can convey the information for $10$ physical qubits. Given the fact that in the absolute worst case a metallic coaxial cable would conduct $1mW$ of heat over a temperature gradient of $[300K,0K]$, we would deduce with this very pessimistic estimation that the heat conduction \textit{per qubit} would be about $100 \mu W$ which is lower than the typical consumption of the DAC/ADC: we can neglect it \red{[my reasonning is correct if the optical fiber has the same size as the coaxial cable: 1mm radius: to check]}. We estimated the amount of information "going down" to create the pulses, but we also need to estimate the information "going up" toward the laboratory. This will be the information associated to the measurement outcomes. In an extremely worst case scenario (which would never occur in practice), all the physical qubits are being measured. We thus get one bit of information per physical qubit to provide to the laboratory on this timescale of $25 ns$. This will be negligible to what we already estimated so that the critical thing to estimate is the information used to drive the gates rather than the information coming from the qubits measurement. 

Later on we will also try to reduce the consumption of the DAC/ADC/ADC in order to see how it affects the global power consumption. For this reason, we would like to see until when we can reasonably neglect the heat conduction of the optical fibers. We believe that as soon as the DAC/ADC wouldn't consume less than $10 \mu W$, we could neglect the heat conduction of the optical fibers. Indeed (i)  they are made of insulating materials such that they would reasonably conduct less heat than a typical metallic coaxial cable; (ii) the value of $1mW$ is very pessimistic as it assumes that $T_{\text{Gen}} \ll 300K$ (the temperature difference between the two end of the cable would verify $\Delta T \approx 300 K$). And in the case of (ii), simply adding an extra cryogenic stage at $T_{\text{Gen}}<T<300K$ could reduce the impact of the heat conduction from those wires such that they would become negligible. Indeed, what matters for us is not really that the heat flow of the cable is negligible, but that the electrical power required to evacuate this heat would be negligible compared to the electrical power required to evacuate the heat of the electronic. This extra stage would be at a temperature where the Carnot efficiency would be much greater which would reduce significantly the impact of this heat load. This is why we consider reasonable to consider that the heat load per physical qubit for the data cables could be effectively estimated as lower than $10 \mu W$ (we assumed that those extra considerations allow us to reduce by $10$ their heat conduction): as soon as the electronic dissipates more than $10 \mu W$ of heat it can be safe to neglect the heat load associated to the optical fibers. 

There are now the DC wires that are providing the power to all the electronic. Those wires will bring heat conduction but also introduce Joules effect. In order to understand what we mean, let us consider the typical resistance of a $1m$ length cable: $R = 10m \Omega$. We assume that the electronic is working under the typical voltage of $U=5V$. We call $\dot{q}_{\text{Gen}}$ the power consumed \textit{per physical qubit} by the electronic, and $N_{\text{DC}}$ the number of DC wires we use. There is an interest into lowering the number of DC wires because we want to minimize heat conduction, but at the same time, all the electronic will require a given amount of current in order to work. The more DC wires are being used and the less Joules effect would be a problem as this current would "spread" on more wires and reduce the heat dissipated. In a more quantitative manner, the total Joules effect dissipated in the DC wires verifies: $P_J=N_{\text{DC}} R (I/N_{\text{DC}})^2$ where $I=\dot{q}_{\text{Gen}} Q_P/U$ is the current that is consumed by all the electronics (we recognize on the numerator the \textit{total} power consumed by all the electronic). What we want is $P_J/Q_P < \dot{q}_{\text{Gen}}$: we want the Joules effect \textit{per qubit} in those cable to be negligible to the heat dissipated \textit{per qubit} of all the electronics. It gives us the relation: $N_{\text{DC}}>R \dot{q}_{\text{Gen}}/U^2  Q_P$. We have $R \dot{q}_{\text{Gen}}/U^2 \approx 10^{-6}$: to have the Joules effect negligible we need more than one wire every million of physical qubits. Considering this as being our choice, the heat conduction from the DC wire will also naturally be negligible given the typical values of heat conduction we gave before. Thus, the heat load associated to DC cables can be entirely neglected.

We can also naturally neglect the heat load associated to the local oscillator: there is a unique coaxial cable for this signal.

Now, we remind that as we are going to make the power consumption of the electronic vary, it is not enough for us to consider that for ADC and DAC dissipating about $1mW$ of heat per qubit, the cables connecting the electronic to the laboratory will have a negligible contribution in term of heat load, we also need to know until which value of $\dot{q}_{\text{Gen}}$ it remains true. The critical moment those assumption will become wrong is given by the optical fibers as they are the cables that will greatly dominate in number. So, our conclusion that as soon as $\dot{q}_{\text{Gen}} > 10 \mu W$ it will be fair to neglect the influence of all the cables connecting to the laboratory would remain true.

Now, there is one last point to discuss: how much the DEMUX-MUX would dissipate? A typical value to demultiplex or multiplex data for the optical fibers we considered is $1pJ$ per bit\footnote{The cost depends on the optical fiber. Indeed optical fibers able to transmit more than $25 Gb/s$ of information do exist but the information would be encoded in a way that would require a bigger consumption for the multiplexing/demultiplexing tasks than the one we are considering here \red{to check again with Yvain}.}. We know that we have $2.5 Gb/s$ of information transiting \textit{per physical qubit} in order to manipulate them (the information entering in the DAC). The power required to demultiplex the data is then about $2.5mW$ which is comparable to the consumption of the DAC/ADC. There is also a power required to multiplex the information coming from the measurement outcomes after it has been digitized by the ADC. But as we already explained, the amount of information involved will be much smaller than the one required to drive the qubits such that the multiplexing cost would be negligible.

In the very end, we will consider $\dot{q}_{\text{Gen}}=5mW$ as a standard value. It will include the cost to demultiplex, multiplex and generate the signals. And when we will try to lower this quantity, as soon as $\dot{q}_{\text{Gen}}>10 \mu W$, the assumption about neglecting all the other cables on this stage will be considered as reasonable.

\textbf{We can neglect the energetic cost associated to parametric amplifiers}\\
We can see on figure \ref{fig:quantum_computer_archi_cable_with_lab} \textbf{b)} that we also removed all the elements associated to the parametric amplifiers. We remind that those components are made of superconducting materials and do not dissipate heat intrinsically. However they require a pump microwave signal (as represented by the blue dotted line) which needs to be attenuated. The typical total attenuation required between where the pump is being generated  and the parametric amplifier is comparable to the one that would be put on the driving lines. For this reason, assuming that the pump signal must be  activated for a duration comparable to the duration of the pulses driving the quantum gates, it will be enough for us to compare the power of the pump signal to the typical power to drive single qubit gates. The pump signal must typically be at least $100 \times$ bigger than the total power of the signal it has amplified (thus the signal at the output of the parametric amplifier). We now estimate this value.

First, we will consider a typical measurement gate duration being $\tau_{P}^{\text{Meas}}=100 ns$. From this and the assumption that the qubits can be set to different frequencies over a bandwith of $\Delta f = 1GHz$, we deduce that we can multiplex the readout signals by putting $100$ of them on the same line. Indeed, we can roughly estimate that one measurement will occupy $1/100ns$ of spectral bandwith (around the frequency of the associated qubit). We deduce that we can multiplex about $\Delta f*\tau_{P}^{\text{Meas}}=100$ signals on the readout measurement lines: each measurement on this line will occupy a well defined spectral band such that the spectral resolution for the measurements will be good enough. One parametric amplifier will then need a pump signal $100 \times$ bigger (in power) than the amplified signal associated to $100$ measurements. Parametric amplifiers typically need to amplify $100$ times the measurement signals \red{cite}. It now remains to estimate the power of a typical measurement. One measurement release one photon in the duration of the measurement, which gives $\hbar \omega_0/\tau_{P}^{\text{Meas}} \approx 10^{-17} W$. Then, using the fact that $100$ of those measurement will be amplified $100$ times and that the pump signal must typically be $100$ times bigger than the resulting amplified signal, we deduce that the pump power should be about $10^{-11} W$.

We need to compare this value to the typical power required to implement single and two qubit gates. For single qubit gates, we remind that we have a typical power $P_g \approx \hbar \omega_0 \pi^2/(4 \gamma_{\text{sp}} \tau^2)$. For $25 ns$ gates, it gives $P_g \geq 10^{-11} W$ if $\gamma_{\text{sp}}<1kHz$ (it will be the maximum value of $\gamma_{\text{sp}}$ we are going to consider in what follows). We see that the power required to drive the quantum gates is then either bigger or comparable to the pump signal. In our approach based on order of magnitudes estimations, it is then safe to neglect it.

\textbf{We can neglect the heat conduction associated to parametric amplifiers, readout lines , readout in and DC power for the classical amplifiers}\\
All those cables, excepted the DC one, will be microwave cables and they will have the same physical properties. In order to know what we can neglect, we then just have to compare the number of each type of cable used. It is given by the quantity of multiplexing we can do. The single qubit gates are the fastest and they will be the "bottleneck" in term of multiplexing. Indeed, following the same reasoning as the one above, we can drive about $1GHz*25 ns=25$ qubits with a single wire\footnote{For historical reasons we considered that $30$ qubits can be driven with a single cable, this is what there will be in our simulations}, otherwise the spectral resolution of the signals is too poor and issues such as crosstalk could occur. As explained, the measurement gates can have a greater level of multiplexing so that the associated cables readout in and readout out will be smaller in number. An even stronger reason holds for the parametric amplifiers pumps microwave cable. We need one of those cable per parametric amplifier, there is one amplifier per $100$ of readout lines, and there is one readout line per $100$ of qubits. In the end, we deduce that the heat conduction associated to measurement cable and pump signals can entirely be neglected compared to the heat conduction of the X/Y lines.

Finally, there are also classical amplifier at the typical temperature of $4K$. One of those amplifiers consumes about $5mW$ of power and will amplify the signal contained in one readout line. Those amplifier need a DC wire to receive power. But those wires can be regrouped such that one wire can provide power to many amplifiers. But it also induces Joules effect. Following the same reasonning as we did for the signal generation stage, we can easily show that both the Joules effect and heat conduction will be negligible compared to the heat dissipated by the amplifier. Indeed it is exactly the same calculation excepted that the heat \textit{per qubit} dissipated by the amplifier would become $5/100 mW=50 \mu W$. Replacing  $\dot{q}_{\text{Gen}} \to \dot{q}_{\text{Gen}}/100$ in the calculation we did would show that we would need at least $1$ wire every $10^8$ physical qubits in order to keep the Joules effect negligible. One wire for $10^8$ qubits would also give a totally negligible heat conduction compared to the $50 \mu W$ dissipated per qubit by the amplifiers. 

In conclusion here, we believe that we have good reasons to approximate the architecture by the model of figure \ref{fig:quantum_computer_archi_cable_with_lab} b), at least in the regime $\gamma \in [10Hz,10kHz]$ and $\epsilon \in [1,10^{-2}]$. In term of validity of the results.

\subsubsection{Expression of the power function for our model}
We are now ready to write down an explicit expression for the power consumption. In order to write nicely the formulas, we will call $T_{\text{Q}}=T_1$, $T_{\text{Gen}}=T_K$. Indeed we will consider adding stages between $T_1$ and $T_K$ to avoid to have to evacuate all the heat on the quantum core which would be very energy inefficient. Only heat conduction and dissipation into attenuators will have to be evacuated there.  We can write down the expression of the total power:
\begin{align}
P&=\frac{300-T_K}{T_K}\left(\dot{q}_{\text{Gen}}-\frac{1}{30}\dot{q}_{\text{Cond}}(T_{K-1},T_K) \right) Q_P \notag \\
&+\sum_{1<i<K-1}\frac{300-T_i}{T_i} \left( \frac{1}{30}(\dot{q}_{\text{Cond}}(T_{i},T_{i+1})-\dot{q}_{\text{Cond}}(T_{i-1},T_i))\right) Q_P+ (\widetilde{A}_i-\widetilde{A}_{i-1})P_g\left(\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}\overline{N}^{\text{1qb}}_{P,\parallel}+2 \overline{N}^{\text{cNOT}}_{P,\parallel}\right) \notag \\
&+ \frac{300-T_{\text{Amp}}}{T_{\text{Amp}}} \dot{q}_{\text{Amp}} \frac{Q_P}{100}\\
&+\frac{300-T_1}{T_1} \left( \frac{1}{30}\dot{q}_{\text{Cond}}(T_{i},T_{i+1})\right) Q_P+ \widetilde{A}_1 P_g\left(\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}\overline{N}^{\text{1qb}}_{P,\parallel}+2 \overline{N}^{\text{cNOT}}_{P,\parallel}\right)
\end{align}
The first line represents the stage where signal are generated. Here only the heat due to signal generation has to be evacuated. There is also heat conduction in the X/Y lines that is going to leave this stage to go to the lower stages (but it will be negligible compared to $\dot{q}_{\text{Gen}}$). The heat conduction \textit{per cable} for the X/Y lines is represented by the function $\dot{q}_{\text{Cond}}(T_{i},T_{i+1})$. The first temperature is the temperature of the colder stage (where the heat is moving toward), and the second temperature is the one of the hottest stage. The coefficients $\frac{300-T}{T}$ represent the Carnot efficiency of the stage.

The second line is associated to the blue intermediate stages of figure \ref{fig:quantum_computer_archi_cable_with_lab}. Their role is to help evacuating heat conduction and dissipation into attenuators. We recognize a first term representing the incoming and outgoing heat conduction. The second term is associated to the heat that is dissipated into the attenuators. On this stage, the attenuation is $A_i=\widetilde{A}_i/\widetilde{A}_{i-1}$, where $\widetilde{A}_i$ is the \textit{total} attenuation from $T_{1}$ up to the stage of temperature $T_i$.  The signal before attenuation on this stage thus have the power amplitude $\widetilde{A}_i P_g$. And after being attenuated this amplitude becomes $\widetilde{A}_{i-1} P_g$. Thus the total heat dissipated reads $(\widetilde{A}_i-\widetilde{A}_{i-1})P_g$. We notice that this power is then multiplied by $\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}\overline{N}^{\text{1qb}}_{P,\parallel}+2 \overline{N}^{\text{cNOT}}_{P,\parallel}$. It comes from our assumption that (i) a two qubit gate requires the same amount of power than two single qubit gate (ii) a single qubit gate is only acting for a portion of the timestep (while the cNOT last for the whole timestep). Thus the power spend to drive the single qubit gates must be weightened by $\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}$ while the cNOT must be weightened by $2$. In principle however this is a detail, given the assumption we already did we could roughly estimate that $\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}\overline{N}^{\text{1qb}}_{P,\parallel}+2 \overline{N}^{\text{cNOT}}_{P,\parallel} \approx \overline{N}^{\text{cNOT}}_{P,\parallel}$.

We notice that on the amplification stage, only the heat dissipated by the amplifiers is evacuated (no heat dissipated from attenuators and no heat from conduction). We considered this choice in our model as it simplifies the expression of the power. Thus there is no attenuators on this stage (as already represented by figure \ref{fig:quantum_computer_archi_cable_with_lab}), but the cables are also not thermalized here (we could thermalize them but given the fact we will anyway consider $K=5$, i.e there are three intermediate stages between $T_{\text{Q}}$ and $T_{\text{Gen}}$, deciding to evacuate heat conduction on the amplifier stage or not shouldn't change significantly the power we obtain.

Now, we can access the coefficients $a$, $b^{\text{1qb}}$, $b^{\text{cNOT}}$ from \eqref{eq:logical_power}. We have:
\begin{align}
a&=\frac{300-T_K}{T_K}\left(\dot{q}_{\text{Gen}}-\frac{1}{30}\dot{q}_{\text{Cond}}(T_{K-1},T_K) \right) \notag \\
&+\sum_{1<i<K-1}\frac{300-T_i}{T_i} \left( \frac{1}{30}(\dot{q}_{\text{Cond}}(T_{i},T_{i+1})-\dot{q}_{\text{Cond}}(T_{i-1},T_i))\right)\notag \\
&+ \frac{300-T_{\text{Amp}}}{T_{\text{Amp}}}  \frac{\dot{q}_{\text{Amp}}}{100} \notag \\
&+\frac{300-T_1}{T_1} \left( \frac{1}{30}\dot{q}_{\text{Cond}}(T_{i},T_{i+1})\right),
\end{align}

\begin{align}
b^{\text{1qb}}&=\frac{\tau_P^{\text{1qb}}}{\tau_P^{\text{timestep}}}  P_g  \left( \sum_{1<i<K-1}\frac{300-T_i}{T_i} (\widetilde{A}_i-\widetilde{A}_{i-1}) +\frac{300-T_1}{T_1} \widetilde{A}_1\right),
\end{align}
\begin{align}
b^{\text{cNOT}}&=2 P_g  \left( \sum_{1<i<K-1}\frac{300-T_i}{T_i} (\widetilde{A}_i-\widetilde{A}_{i-1}) +\frac{300-T_1}{T_1} \widetilde{A}_1\right)
\end{align}
\subsection{Expressing the metric}
\subsubsection{Expression as a function of the quantity of noisy photons}
Now that the expression of the power has been specified, we need to express the quantity of noise that will be felt by the qubits. The metric will be the probability of error per logical gate, $p_L$. We remind that its expression is:
\begin{align}
p_L=\eta_{\text{thr}}\left(\frac{\eta}{\eta_{\text{thr}}}\right)^{2^k},
\end{align}
with $\eta_{\text{thr}} \approx 10^{-4}$ for probabilistic noise. As done in the previous chapter, we will also consider the noise to be probabilistic with $\eta=\max_i \chi_{ii}$, where $\chi$ is the $\chi$ matrix associated to the noise map $\mathcal{N}$. 

We find that, if the noise map is acting for a duration $\tau$, we have:
\begin{align}
\eta=\frac{(1+2\overline{n}_{\text{tot}})\gamma_{\text{sp}}\tau}{4},
\end{align}
where $\overline{n}_{\text{tot}}$ is the total number of photons in the noise felt by the qubits. It is related to their temperature but also to the temperature of all the other cryogenic stages. The duration $\tau$ we need to consider is the duration associated to the longest physical gate: it corresponds to the physical timestep $\tau_P^{\text{physical}}$ and is equal to both cNOT and measurement gates duration for us.
\subsubsection{Expressing the noisy photons number as a function of the temperatures and attenuations}
As we now have $K$ temperature stages where $T_1=T_{\text{Q}}$ and $T_{K}=T_{\text{Cl}}$, we then have a family of attenuations: $\{A_i\}_{i=1,...,K-1}$ to put on all the stages below $T_K$ as shown on the Figure \ref{fig:attenuators}. We can now determine the total number of noisy photons felt by the qubit.
\begin{figure}[h!]
\centering 
\includegraphics[width=0.2\textwidth]{chapter4/images/attenuators}
\caption{Example with $K=3$: attenuators, temperature stages and signal amplitudes.}
\label{fig:attenuators}
\end{figure}
\FloatBarrier
\textbf{Total number of noisy photons at $T_1$}\\
The total number of noisy photons on the stage $i$ verifies \cite{pozar2011microwave}:
\begin{align}
\overline{n}^{(i)}_{\text{tot}}=n_{BE}(T_i) \frac{A_i-1}{A_i}+\frac{n_{\text{tot}}^{(i+1)}}{A_i}
\label{eq:ntot_recursive}
\end{align}
And to be able to deduce the number of noisy photons on the qubit temperature we need the boundary condition
\begin{align}
\overline{n}_{\text{tot}}^{(K)}=n_{BE}(T_K).
\label{eq:ntot_Cl}
\end{align}
Using \eqref{eq:ntot_recursive} and \eqref{eq:ntot_Cl}, we deduce:
\begin{align}
\overline{n}_{\text{tot}}^{(1)}=\sum_{i=1}^{K-1} n_{BE}(T_i) \frac{A_i-1}{A_1...A_i}+\frac{n_{BE}(T_K)}{A_1...A_{K-1}}
\label{eq:total_noisy_photons}
\end{align}
\textbf{Reducing the number of free parameters in the problem}\\
In principle we could imagine optimizing all the attenuations and temperatures. However this would lead to way to variables to optimize such that the computation would take too long. We would like to simplify the problem. In order to do so, we will give some "reasonable" constraints on the attenuations and temperature such that the optimization will be parametrized only by the total attenuation there is on the lines, and the qubit and signal generation temperatures $T_1$ and $T_K$.

For the temperatures, we will ask that they are regularly spaced in order of magnitudes. For instance, for $K=5$, if $T_1=10mK$ and $T_K=100K$, we would like that the rest of the temperature would verify: $T_2=100mK$, $T_3=1K$, $T_4=10K$. The reason why we would like to put the temperature stage in a regular manner in order of magnitude is because this is what is usually done in Cryostat \cite{krinner2019engineering}. Of course better choices could be possible: the best optimization for the intermediate stage depend on the attenuation that is put on them and on the heat conduction laws. Mathematically, our formulation means that the temperature are chosen as:
\begin{align}
&T_{1<i<K}=10^{x_0+(i-1)x_1},
\end{align}
where $x_0$ and $x_1$ are chosen by the boundary conditions $T_1$ and $T_K$. We deduce:
\begin{align}
&x_1=(\log(T_K)-\log(T_1))/(K-1)\\
&x_0=\log(T_1)
\end{align}
Which gives:
\begin{align}
T_i=T_1 \left(\frac{T_K}{T_1}\right)^{\frac{i-1}{K-1}}
\label{eq:choice_temp}
\end{align}
In order to reduce the number of variables used to describe the attenuations, we will consider the following. The total attenuation $A$ will be the parameter we will optimize. We will consider that the attenuation on a given stage will be proportional to the ratio between the temperature of the stage and the temperature of the closest higher stage. The motivation behind such assumption is that in the high temperature regime ($k_b T \gg \hbar \omega_0$), we have $n_{BE}(T) \approx k_b T/\hbar \omega_0$. The number of noisy photons are proportional to the temperature. Thus to make the number of noisy photons coming from higher temperature stage negligible to the number of noisy photons where the attenuator has been put, we should attenuate of a quantity typically given by the ratio of those temperatures. Now it is not clear how much attenuation should exactly be put (exactly this ratio? Two orders of magnitude bigger "for safety"?). It is also not so clear as in the low temperature regime, where the qubits are usually put, the approximation $n_{BE}(T) \approx k_b T/\hbar \omega_0$ is no longer correct. This is why we believe that optimizing the total attenuation is something that is important to do. In the end, our choice imposes
\begin{align}
&A_i=\epsilon \frac{T_{i+1}}{T_i}
\end{align}
where $\epsilon$ is the proportionality coefficient that we need to determine through the constraint $\prod_{i=1}^{K-1} A_i = A$. Now, using the fact that our temperature are chosen following \eqref{eq:choice_temp}, we deduce:
\begin{align}
A_i=A^{1/(K-1)}
\label{eq:att_per_stage}
\end{align}
The same value of attenuation is being put on each temperature stage. And this value is deduced from the total attenuation value.

\textbf{Exploiting the condition $\mathcal{M}=\mathcal{M}_{\text{target}}$}

As shown in the property \ref{prop:behavior_min_power}, the minimum power consumption will be obtained for the metric veryfing $\mathcal{M}=\mathcal{M}_{\text{target}}$. This property is usefull for our purposes. Indeed we can use it to remove one parameter from the optimization procedure.

Here, we have: $\mathcal{M}=N_L p_L$. If we want our algorithm to provide the correct answer with a probability $1-p_{\text{target}}$, $\overline{n}_{\text{tot}}$ must then verify:
\begin{align}
\overline{n}_{\text{tot}}=\frac{1}{2}\left(\frac{4 \eta_{\text{thr}}}{\gamma_{\text{sp}} \tau_{P}^{\text{timestep}}}\left( \frac{p_{\text{target}}}{\eta_{\text{thr}}N_L} \right)^{2^{-k}}-1 \right)
\end{align}
We can exploit this condition to express the total attenuation as a function of $T_1, T_K$ and $k$. Indeed, it is possible to show that injecting \eqref{eq:att_per_stage} and \eqref{eq:choice_temp} in \eqref{total_noisy_photons}, we find the following polynomial equation as a function of the variable $y=A_i=A^{1/(K-1)}$:
\begin{align}
(\overline{n}_{\text{tot}}-n_{BE}(T_1))y^{K-1}+\sum_{p=1}^{K-2} (n_{BE}(T_{K-1-p})-n_{BE}(T_{K-p}))y^p+n_{BE}(T_{K-1})-n_{BE}(T_{K})=0
\end{align}
For $K \leq 5$, there are analytic solution of this equation for the variable $y$. Keeping only the physical ones (i.e $y \geq 1$: the attenuation must be bigger than one), we deduce the value of $A$ as a function of $T_1$, $T_K$ and $k$ that will allow to verify $\mathcal{M}=\mathcal{M}_{\text{target}}$. 


%The \textbf{total} attenuation one has put on the line then reads:
%\begin{align}
%A_{\text{tot}}=A_1...A_{K-1}
%\end{align}
%We can also express the power being dissipated on the stage $i$. We have:
%\begin{align}
%\dot{Q}_i = P^i_{\text{in}}- P^i_{\text{out}}
%\end{align}
%Where:
%\begin{align}
%&P_{\text{in}}=A_1...A_i P_g\\
%&P_{\text{out}}=P_{\text{in}}/A_i
%\end{align}
%Thus, we have (see Fig \ref{fig:attenuators} to "visualize" this):
%\begin{align}
%&\dot{Q}_{i>1} = (A_1...A_i-A_1...A_{i-1})P_g=A_1...A_{i-1}(A_i-1)P_g\\
%&\dot{Q}_i=(A_1-1)P_g
%\end{align}
\red{A faire: Simplify the text of all that is after "engineering model"}
\subsection{Energetic cost of a fault tolerant QFT}
\subsubsection{Minimum power and optimal parameters}
\subsubsection{How much power is being saved}
\subsubsection{The weight of attenuation}
\subsection{Energetic cost of a fault tolerant quantum memory}
\section{Outlooks}
\begin{itemize}
\item Minimizing other resources: number of available frequencies ?
\item Comparing the energy efficiency of different codes and architectures.
\item Optimizing the amplification stage temperature.
\item Energetic interest for autonomous QEC.
\end{itemize}
\begin{appendices}

\end{appendices}


==> chapter4/chapter4_save_10_08_2021.tex <==
\chapter{The energetic cost of quantum computing: full-stack framework}
\label{chap:Fullstack1}
In this chapter, we are going to design the general method we propose in order to do resource estimation of quantum computing. We will directly apply it to the problematic of energetics, more precisely, of power consumption. Our method is said to be full-stack because it allows to include aspects from engineering, algorithms and quantum physics, in order to do the energetic estimation. The central point on which our approach is built consists in relating the quality of the algorithm output to the power that is spent inside of the quantum computer. We will see that, by asking to minimize the power consumption of the computer \textit{under the constraint} that the algorithm succeeds, we will have access to the minimum power consumption required to implement successfully the algorithm \textit{as well} as the optimal architecture the computer should have in order to reach this minimum. We will also be able to optimize the way the algorithm is implemented for the same goal of minimizing the power. In some sense, we generalize here the approach of the previous chapter as the noise will no longer have to be a function of the resource to minimize, and because we will be able to optimize the quantum computer architecture while performing the minimization. The method we propose can in principle be applied both in NISQ algorithm (with some restrictions that we will explain) and in fault-tolerance. This chapter is dedicated to explain the general principle and to provide simple toy examples where it can be applied. We will also see what are the differences between energetic estimation for algorithm implemented with or without quantum error correction. The following chapter will consist in using this method in order to make a quantitative and detailed energetic estimation of implementing an algorithm on a fault tolerant quantum computer based on superconducting qubit.
\section{The energetic cost of quantum computing: general vision}

\subsection{Formulating the question as a minimization under constraint}
The general purpose of an algorithm is to provide an answer to some computational task. What we care about is obviously to have the good answer to this task, there is no point in having a bad one. However, because of noise, there will always have a probability that the answer we find is not the good one. 
On the other hand, the probability to find a successful answer will be related to how much some resource an experimentalist is ready to invest in the calculation. Indeed, implementing successfully an algorithm (in the sense that it provides an answer having a high probability of success) has a cost. We saw examples in the previous chapter with the energy that we allowed to spend in order to create the pulses driving the qubits. When we restricted too much this energy, the algorithm had a poor success probability. Without loss of generality, we will now assume that the resource we are interested in is the \textit{power} required to implement an algorithm. We understand that there must exist a \textit{minimum} power required to implement successfully an algorithm. And we can phrase the exact question we should address in order to find it. We basically ask: "what is the minimum power I have to spend under the constraint that the algorithm I am implementing provides the good answer to the task with a probability higher or equal to some target I want.". The answer to this somewhat lengthy question is the only thing that really matters in order to be power efficient. We can phrase it in a mathematical manner as the following problem of optimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | p_{\text{success}}(\bm{\delta}) \geq p_{\text{target}}},
\label{eq:ideal_solve}
\end{align}
where $P$ is the power, $p_{\text{target}}$ is the success probability we aim for, and $p_{\text{success}}$ is the actual probability of success of the algorithm. We see that we introduced the family of parameters $\bm{\delta}$ (the fact it is a family is represented by the bold notation associated to vectors). They represent the \textit{tunable} parameters that the experimentalist can vary in order to reach the minimum. A typical example would be the qubit temperature $T_{\text{Q}}$: changing it would at the same time modify the power it costs to perform the computation (the electrical power for the cryogenic typically depends on $T_{\text{Q}}$), but the success probability as well (a too high temperature would induce a poor quality in the answer). Thus, in general, both the probability of success and the power depend on the family $\bm{\delta}$\footnote{Of course it is possible that one parameter in the family of parameters $\bm{\delta}$ only affect the success and not the power cost, and reciprocally.}. This minimization under constraint provides an equation that relates the resource one should spend with the probability of success of the algorithm. We also see that not only the minimum power can be found performing this minimization, but the optimum set of parameters allowing to reach this minimum, $\bm{\delta}_{\text{opt}}$ will also be found.

Unfortunately, directly solving this problem is too complicated in general. Indeed it is usually not possible to directly find the function $p_{\text{success}}(\bm{\delta})$ as it would usually require to know the density matrix at the end of the algorithm. If this is a requirement the method would have no interest because it would mean that the circuit can be efficiently simulated classically\footnote{As the goal is to implement an algorithm on a quantum computer, this algorithm must present advantages compared to a classical simulation.}. For this reason, we will take a slightly different approach. We will not try to estimate the success probability of the algorithm, but we will try to estimate, or at least to bound the "quantity of noise" there is in the final density matrix of the algorithm (right before the measurements). This approach is slightly different because there is a unique way to define the success probability of the algorithm while there are different ways to evaluate the quantity of noise inside a density matrix (we could think about the trace distance or the fidelity with respect to the ideal state for instance). The reason to do this strategy is that it is an easier quantity to estimate, or more usually, \textit{to bound}, than the probability of success of the algorithm\footnote{Also, the different ways to quantify the noise are usually related: knowing the value of one often allows to give a bound the other.}. To give specific examples, the worst-case fidelity of an algorithm can easily be bounded by the knowledge of the worst-case fidelity of each individual gates composing it. And from this knowledge, we can then bound, or have a rough estimation of the probability of success of the algorithm (which is much more complicated to directly access theoretically). This is another important requirement we should have in the way we measure the quantity of noise: there is no point in being able to estimate the quantity of noise in the final density matrix if it doesn't give any information about the probability to have the good answer. All those requirements will give us constraints on what are the good or the bad tools that can be used to measure the quantity of noise in the final density matrix of algorithms. We call them "metrics" and write them with the letter $\mathcal{M}$ in what follows. Putting aside those issues for now on, the problem of power estimation can in the end be formulate by the following minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{\text{target}}}.
\end{align}
This equation means that we want to find the minimum power under the constraint that the quantity of noise (as quantified by the metric $\mathcal{M}$) is lower than some targetted quantity of noise $\mathcal{M}_{\text{target}}$ considered as acceptable by the experimentalist. The value of the metric $\mathcal{M}$ depends on the family of tunable parameters $\bm{\delta}$ for the exact same reason as $p_{\text{success}}$ in \eqref{eq:ideal_solve} also depended on those.
\subsection{General properties implied by the question}
\subsubsection{The minimum power increases with the targetted accuracy}
Let's assume that there exist a parameter $\delta_j$ in the list of parameters  $\bm{\delta}$ such that, when we increase it, the power decreases while the quantity of noise increase. Mathematically it means that:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
One example of such parameter will often be the temperature of the qubits. If we increase the qubit temperature, the power it costs to maintain them cool will typically decrease, but the quantity of noise will usually increase because they will be submitted to more thermal noise. We will see it in a concrete manner in the parts where we will take physical examples: the hypothesis that such parameter $\delta_j$ exists will typically be true in relevant physical systems. From now on, we will assume it is the case.

This hypothesis will imply the following two properties. First, (i) the minimum power required such that the quantity of noise of the algorithm is equal \textit{or lower} to $\mathcal{M}_{\text{target}}$ is the same as the minimum power required such that the quantity of noise is \textit{equal} to $\mathcal{M}_{\text{target}}$, i.e the following equality is true:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}}
\end{align}
Let us do a proof by contradiction of this fact. We assume that the minimum power is found when $\mathcal{M} < \mathcal{M}_{\text{target}}$. As $\partial_{\delta_j} \mathcal{M}>0$, we can increase $\delta_j$ for some range without violating the condition $\mathcal{M} \leq \mathcal{M}_{\text{target}}$. Doing so, we will also decrease the power as $\partial_{\delta_j} P<0$. Thus, as soon as $\mathcal{M}<\mathcal{M}_{\text{target}}$ we do not minimize the power consumption: the minimum is necessarily reached for $\mathcal{M}=\mathcal{M}_{\text{target}}$. In the same line of thoughts, we can also prove that (ii) $P_{\min}$ is a \textit{strictly decreasing} function of $\mathcal{M}_{\text{target}}$. To show this, let us consider two targets such that $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$. Then, as:
\begin{align}
\min(P)_{\big | \mathcal{M} \leq \mathcal{M}^2_{\text{target}}}=\min(P)_{\big | \mathcal{M} = \mathcal{M}^2_{\text{target}}},
\end{align}
the minimum power obtained for $\mathcal{M}<\mathcal{M}^2_{\text{target}}$ is necessarily bigger or equal to the one obtained for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Because of that, as $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$, we deduce that: $P_{\min}(\mathcal{M}^1_{\text{target}}) \geq P_{\min}(\mathcal{M}^2_{\text{target}})$. It remains to show that they cannot be equal. We also do a proof by contradiction. Let us consider a set of parameters $\bm{\delta}$ such that: $P(\bm{\delta})=P_{\min}(\mathcal{M}^1_{\text{target}})$, and $\mathcal{M}(\bm{\delta})=\mathcal{M}^1_{\text{target}}$\footnote{We say "a" set of parameters and not "the" set of parameters as the minimum power consumption could be in principle reached for many different values of $\bm{\delta}$.}. If we increase $\delta_j$ until the moment $\mathcal{M}=\mathcal{M}^2_{\text{target}}$, as $\partial_{\delta_j} P < 0$, it has for effect to \textit{strictly} decrease the power consumption while ensuring $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Thus, the minimum power reached for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$ is necessarily \textit{strictly} lower than the one reached for $\mathcal{M}=\mathcal{M}^1_{\text{target}}$.

In summary, here we proved the following property that we will frequently use.
\begin{property}{Behavior of the minimum power}

\label{prop:behavior_min_power}
If there exists at least one parameter $\delta_j$ in the family of parameters $\bm{\delta}$ on which:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
Then, we have:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}},
\end{align}
which means that the minimum power consumption is found when we ask for an accuracy that it is exactly equal to what we target: asking for a better accuracy is necessarily more costly. We also have that
$P_{\min}$ is a strictly decreasing function of $\mathcal{M}_{\text{target}}$ (for the same reason).
\end{property}
This property establish properly the intrinsic connection between noise and power: asking for a better accuracy has an energetic cost. But again this connection is true because of the hypothesis we made on the behavior of power and metric with respect to the parameter $\delta_j$ (which will frequently be true in physical systems).
\subsubsection{Equivalence between minimum power for a targetted accuracy and maximum accuracy for a given power}
\label{sec:equivalence_minpow_maxacc}
Now, we can show that asking to minimize the power in order to reach a given accuracy is in some sense, equivalent to asking to find the best accuracy the computer can get to for a given (i.e fixed) amount of power available. This property is true as soon as $P_{\min}$ is a decreasing function of $\mathcal{M}_{\text{target}}$ (which will usually be the case as explained before).

Those two questions are equivalent in the sense of what is represented on figure \ref{fig:equivalence_minpow_maxacc}. On this curve is represented the minimum power required to implement the algorithm as a function of the maximum quantity of noise acceptable in its answer: $\mathcal{M}_{\text{target}}$. In this case, this graph can be read in two directions. Indeed, if we invert the meaning of the axis, i.e we interpret it as a curve representing a value of some quantity of noise as a function of some injected power, we can also interpret it as the \textit{minimum} quantity of noise it is possible to reach as a function of this injected power. More precisely, let us consider any couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. By definition of $P_{\min}$, if someone wants to have an accuracy $\mathcal{M}^0_{\text{target}}$, the minimum power required will be $P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. But reciprocally, if this person has a given amount of power $P^0$ available, the minimum quantity of noise it can get to (thus maximum accuracy) is $\mathcal{M}^0_{\text{target}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.5\textwidth]{chapter4/images/equivalence_minpow_maxacc}
\caption{The minimum power necessary as a function of the maximum quantity of noise acceptable targetted, $\mathcal{M}_{\text{target}}$ is represented. Because this function is monotonous, the curve can also be interpreted as the lowest quantity of noise acceptable for a given amount of power available as explained in the main text.}
\label{fig:equivalence_minpow_maxacc}
\end{center}
\end{figure}
\FloatBarrier

In order to show it, we consider again the couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. We now ask: what is the maximum accuracy, i.e the lowest quantity of noise $\mathcal{M}$ the computer can get to if it has at its disposal the power $P^0$. Necessarily, it can be \textit{at least} as accurate as $\mathcal{M}^0_{\text{target}}$: $\mathcal{M}$ must verify $\mathcal{M} \leq \mathcal{M}^0_{\text{target}}$. Indeed $\mathcal{M}^0_{\text{target}}$ is an explicit example of target reachable for an injected power $P^0$. Now it remains to prove that the strict inequality is not possible: no better accuracy is reachable for this amount of power. This can be shown using again a proof by contradiction: let's assume that we find that the best accuracy it is possible to reach for an injected power $P^0$ verifies $\mathcal{M} < \mathcal{M}^0_{\text{target}}$. We assume that this power is reached for the family of parameters $\bm{\delta}=\bm{\delta}_0$. We necessarily have $P^0=P(\bm{\delta}_0) \geq P_{\min}(\mathcal{M})$: indeed $P^0$ amount of power would be used to have an accuracy $\mathcal{M}$, but it might be possible to use less power to reach that accuracy. As on the other hand $P_0=P_{\min}(\mathcal{M}^0_{\text{target}})$, we deduce that $P_{\min}(\mathcal{M}^0_{\text{target}})\geq P_{\min}(\mathcal{M})$. Now, this result is absurd. Indeed, as $\mathcal{M}<\mathcal{M}^0_{\text{target}}$, and as $P_{\min}$ \textit{strictly} decreases as a function of $\mathcal{M}$, necessarily $P_{\min}(\mathcal{M}^0_{\text{target}}) < P_{\min}(\mathcal{M})$. 

All this shows that the curve can be read in two directions: \textit{there is an equivalence between asking to minimize the noise for a given amount of power available, and asking to minimize the power in order to target a given quantity of noise.}
\subsection{An introductive example: energetic cost of a single qubit gate}
\subsubsection{Description of the problem}
\label{sec:single_qubit_example}
Let us illustrate the concepts with a very simple example: we wish to minimize the power to spend in order to implement a $\pi$-pulse on a qubit. For this, we need to specify: (i) the noise model describing the physics, (ii) the way we quantify this noise, i.e which metric we are going to choose, (iii) the expression of the power we want to minimize and (iv) the list of parameters we would like to optimize in order to minimize this power.

We start to specify (i). Here, we assume that the only reason why the qubits are noisy is because of thermal noise. The noisy evolution can be modeled as:
\begin{align}
&\frac{\partial \rho}{\partial t}=\frac{1}{i \hbar}[H,\rho]+\gamma_{\text{sp}} \overline{n}_{\text{tot}} D[\sigma^{\dagger}](\rho) + \gamma_{\text{sp}}(\overline{n}_{\text{tot}}+1) D[\sigma](\rho) \label{eq:evolution_noisy_gate}\\
&D[\sigma](\rho) \equiv \left(\sigma \rho \sigma-\frac{1}{2}(\sigma^{\dagger} \sigma \rho + \rho \sigma^{\dagger} \sigma) \right),
\end{align}
%where $H$ is the Hamiltonian implementing the gate, $\overline{n}_{\text{tot}}$ represents the noise photon occupation, i.e the number of photons in the power spectral density of noise \red{to double check the vocabulary is the good one}, and $\gamma_{\text{sp}}$ is the qubit-waveguide coupling\footnote{We remind that its inverse gives the typical qubit lifetime at $0$ temperature.}. As explained in the chapter dedicated to fault-tolerance, it is always possible to "decouple" the effect of the noise from the perfect implementation of the gate such that everything will behave \textit{as if} the perfect implementation of the gate occured first, then followed by some noise. If the quantum channel $\mathcal{U}$ represents the ideal (unitary) implementation of the gate, and $\mathcal{E}$ represents the noisy implementation (thus following the equation \eqref{eq:evolution_noisy_gate} integrated for the duration of the gate), we can always define $\mathcal{N}$ such that $\mathcal{E}=\mathcal{N} \circ \mathcal{U}$. With this definition, $\mathcal{N}$ represents the effect of the noise "alone" that is acting "after" the perfect implementation of the gate. Conceptually we could proceed this way here, but in order to anticipate the section dedicated to fault-tolerance, we will adopt a slightly simpler way to model the noise. We will approximate this noise map $\mathcal{N}$ by considering that it can be estimated by integrating  \eqref{eq:evolution_noisy_gate} with $H=0$, for a duration equal to the gate duration. When we say that $\mathcal{N}$ is obtained by integrating this equation, it means that we consider a basis of initial states for the qubit from which we can deduce the mathematical expression of $\mathcal{N}$. This is an approximation because we can expect this result to be different than the computation of the exact evolution $\mathcal{E}$, and then defining $\mathcal{N}= \mathcal{U}^{-1} \circ \mathcal{E}$. However,  this simplification will not change in a quantitative manner our estimation of the quantity of noise introduced by such evolution \footnote{This is actually something that we checked: for a $\pi$-pulsife the expressions of the worst case and average fidelity of the "precise" or "approximated" approach are very similar.}. In the end, the map $\mathcal{N}$ is then accessible which defines our noise model. It will be a function of $\overline{n}_{\text{tot}}$, $\gamma_{\text{sp}}$ and $\tau$ the gate duration. 

Now, we specify (ii). In order to quantify the quantity of noise in the final density matrix, we will use either the worst-case or average infidelity of this channel. We call infidelity the quantity $1-F$ where $F$ is the fidelity. We find:
\begin{align}
\mathcal{M}=(X+Y \overline{n}_{\text{tot}}) \gamma_{\text{sp}} \tau,
\end{align}
where $(X_{\text{worst}},Y_{\text{worst}})=(1,1)$ and $(X_{\text{avg}},Y_{\text{avg}})=(1/3,2/3)$ for worst-case infidelity and average one respectively. The metrics are then defined. But we cannot be satisfied of those expressions because we don't know what $\overline{n}_{\text{tot}}$ is equal to, we need to explain it. 

In the case the qubit is at the temperature $T_{\text{Q}}$, and \textit{if the signals are generated at this same temperature}, we would simply have: $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}}) \equiv 1/(e^{\beta_{\text{Q}} \hbar \omega_0}-1)$, with $\beta_{\text{Q}}=1/(k_b T_{\text{Q}})$, and $\omega_0/2 \pi$ is the qubit frequency (typically around $6$ GHz). $\overline{n}_{\text{BE}}$ is the Bose Einstein population for bosons of frequency $\omega_0/2 \pi$, at temperature $T_{\text{Q}}$ \cite{cohen1998mecanique}. But if the signals are generated at a temperature $T_{\text{Gen}}$, then the thermal noise at this temperature would affect the qubit evolution. This is why attenuators are typically put on the driving lines. Their role is to remove the noise (and in particular the thermal noise) coming from the higher temperature stages. An attenuator is composed of resistive elements that will dissipate into heat any signal injected at its input as shown on figure \ref{fig:attenuator_principle}. If $P_{\text{in}}$ is the input power before the attenuator, and $P_{\text{out}}$ the power at its output, we define the attenuation ratio by $A \equiv P_{\text{out}}/P_{\text{in}}$. It is possible to show \cite{pozar2011microwave} that for signals generated at $T_{\text{Gen}}$, an attenuator put at the temperature $T_{\text{Q}}$ will generate an amount of noisy photons $\overline{n}_{\text{tot}}$ being equal to:
\begin{align}
\overline{n}_{\text{tot}}(T_{\text{Q}},T_{\text{Gen}},A)=\frac{A-1}{A} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A} \stackrel{A \gg 1}{\approx} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A}
\end{align}
Let us first comment the formula in the $A \gg 1$ regime. It means that the quantity of noisy photons felt by the qubits will be equal to the number of noisy photons at the attenuator temperature, on which we add the noisy photons coming from the higher temperature stage, but attenuated by a factor $A$. The noise is basically attenuated in the same way than the signals sent. For an infinite attenuation, the qubits will be entirely isolated from any thermal noise coming from higher temperature stages. However this cannot be the exact expression. For instance for $T_{\text{Q}}=T_{\text{Gen}}$ (if everything is thermalized at $T_{\text{Q}}$), we would not find $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})$ with the approximated expression. This is the reason why the exact expression is actually the one of the left: it correctly describes the situation when $T_{\text{Q}}=T_{\text{Gen}}$ and $A=1$ (no attenuation: everything behave as if the qubits where thermalized at $T_{\text{Gen}}$). Of course this formula should be thought as a first order description \red{to check} of the physics (what we said is not a proof that this expression is the correct one), but it is what is used to describe the propagation of noise in microwave circuits \cite{pozar2011microwave}. Physically we can understand the situation as follows: the signal generation stage can be thought as some cavity which is thermalized at $T_{\text{Gen}}$. This cavity thus emits a blackbody radiation in a one-dimensional waveguide: it is the thermal noise. Then this noise propagates in a ballistic manner in the waveguide (as a waveguide will by construction be a good conductor for microwave frequencies, the noise won't be attenuated there). This noise is then dissipated inside of the attenuator and "converted" into phonons: this is a kind of heat that can be evacuated by the cryogenics. But the attenuator, being thermalized at $T_{\text{Q}}$, also generates thermal noise that will interact with the qubits. It corresponds to $\overline{n}_{\text{BE}}(T_{\text{Q}})$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/attenuator_principle}
\caption{Principle behind the attenuation. The signals are generated at a temperature $T_{\text{Gen}}$. Thus, in addition to the signals there is noise at this temperature that is propagating inside of the waveguide as represented by the noisy blue gaussian. The qubit is preceeded by an attenuator at the temperature $T_{\text{Q}}$. The attenuator will dissipate the noise before it reaches the qubit, but it dissipates the signal in the same manner. It is the fact that the heat $\dot{Q}_{\text{Att}}$ has to be evacuated by a cryogenic unit that makes the gate energetically costly (as shown by \eqref{eq:power_single_qubit_gate}).}
\label{fig:attenuator_principle}
\end{center}
\end{figure}
\FloatBarrier
Now, in practice the effect of the thermal noise coming from the higher temperature stages will be reduced by the following strategy. First, the signal that must arrive on the qubit has a well defined value: we must have $P_{\text{out}}=P_g$, where as explained in the fist chapter of this thesis \red{put a ref} $P_g=\hbar \omega_0 \Omega^2/(4 \gamma_{\text{sp}})$ with $\Omega=\theta/\tau$. Here $\theta$ represents the angle of rotation desired for the single qubit operation ($\theta=\pi$ for us in this section). Then, the attenuation $A$ is usually chosen in such a way that $\overline{n}_{\text{BE}}(T_{\text{Gen}})/A < \overline{n}_{\text{BE}}(T_{\text{Q}})$: the noise coming from the higher temperature stage does not dominate the physics. From the knowledge of $A$ the experimentalist deduce what is the power the generated signals should have. The general philosophy is to generate signals of high enough amplitude such that after attenuation there is a high signal over noise ratio while having a signal of appropriate power for the physics of the quantum gate. At this point, we can say that the metrics we expressed are now "well defined" because we know what $\overline{n}_{\text{tot}}$ is equal to as a function of the characteristics of the problem.

Now, we need to give the expression of the power (point (iii)). Here, we will be interested in the electrical power that we need in order to remove the heat dissipated inside of the attenuators. We will assume that our cryogenic unit has a Carnot efficiency. The heat dissipated per unit time is simply equal to $P_{\text{in}}-P_{\text{out}}$\footnote{We implicitely neglect the heat that will be dissipated when the signals will "go back", i.e after reflection on the qubit. Indeed, the power that would be dissipated by this reflection will be lower than $(A-1) P_g$ and we will neglect it. This approximation is even more true in the regime $A \gg 1$ on which we are focusing.}, the low temperature stage on which the heat has to be evacuated has a temperature $T_{\text{Q}}$, and the high temperature stage is basically the laboratory at temperature $300K$. Assuming that $A \gg 1$ (if it is not the case the evolution would be way too noisy), we get:
\begin{align}
P(T_{\text{Q}},A)=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A P_g
\label{eq:power_single_qubit_gate}
\end{align}
%All that being said, we will consider that $T_{\text{Gen}}=300K$ here (the signals are generated outside of the cryogenics, in the laboratory), and we will consider that the parameters we are going to optimize will be $T_{\text{Q}}$ and $A$. The point (iii) is now specified and the last thing to do is to provide the expression of the power.
Finally, for our last point (iv), we specify the variables we want to optimize. It will be $\bm{\delta}=(T_{\text{Q}},A)$ in this first example as we will assume that $T_{\text{Gen}}=300K$ (the signals are generated outside of the cryogenics here). In the end, the problem is well defined, and we can solve the minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{(T_{\text{Q}},A)} P(T_{\text{Q}},A)_{\big | \mathcal{M}(T_{\text{Q}},A) = \mathcal{M}_{\text{target}}}
\end{align}
\subsubsection{The competition between noise and power}
We first illustrate on figure \ref{fig:competition_power_noise} in a concrete manner the intrinsic competition there is between asking for a low noise and a low power consumption. The parameters we chose for the gate are $\gamma_{\text{sp}}=1kHz$, $\tau=25 ns$ (and $\theta=\pi$: we do a $\pi$-pulse). In the rest of this thesis we will also use the decibel: "dB" unit to represent the attenuation. This unit is related to the attenuation in "natural unit", i.e when $A=P_{\text{in}}/P_{\text{out}}$ as:
\begin{align}
A_{\text{dB}}=10 \log_{10}(A)
\end{align}
For instance, a signal being attenuated of a factor $10$ will correspond to $10 \text{dB}$. A signal attenuated of a factor $10^5$ will correspond to $50 \text{dB}$. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/competition_power_noise}
\caption{Unoptimized power consumption as a function of the attenuation and the qubit temperature (color-plot). The cyan and white lines represent the iso-infidelity for respectively the average and worst case infidelity.}
\label{fig:competition_power_noise}
\end{center}
\end{figure}
\FloatBarrier
On this graph, we see that putting a high attenuation and a low qubit temperature induces a high power consumption. Reciprocally a high qubit temperature and a low attenuation leads to a small power consumption. We can also see that the regions of high power consumption correspond to regions of low noise, and regions of lower power consumption correspond to regions where the noise is high. Indeed the iso-metric lines have lower values in the bottom right part of this graph which corresponds to region of high power consumption (and higher values in the upper left part of this graph where the power is low). It illustrates the intrinsic opposite behavior between noise and power.

Let us now focus on a given iso-metric line: we wish to implement the single qubit gate in order to reach a targetted accuracy. The power consumption on those lines can drastically vary. For instance, the white iso worst-case infidelity which is at the bottom right of this graph is associated to power varying in the range (approximately) $[10^{-3},10^{-1}]$. It illustrates that choosing wisely $T_{\text{Q}}$ and $A$ is a key asset to potentially make important energetic saves: there are many possible ways to reach a given accuracy, and each of those choice can be associated to a drastically different power consumption. Of course this example is very simple as we only modeled the heat dissipated in the attenuators, but we see that it can potentially lead to quantitative saves in power consumption, and we can naturally expect that it would remain true for more complicated models\footnote{In particular because more tunable parameters will be involved, the optimum choice of parameters allowing to minimize the power consumption might be not trivial for more complicated models.}.
\subsubsection{Minimizing the power consumption}
Now, we can minimize the power consumption in order to reach a given target. This is shown on figure \ref{fig:min_power_fct_metric_1qb}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/min_power_fct_metric_1qb}
\caption{Minimum power consumption as a function of the metric target. Inset: optimum qubit temperature $T_{\text{Q}}^{\text{opt}}$ allowing to reach this minimum. Blue points: worst-case fidelity, orange: average. The black line is a guide for the eye. As explained in \ref{sec:equivalence_minpow_maxacc}, this curve can also be interpreted as the minimum metric target it is possible to reach as a function of the injected power.}
\label{fig:min_power_fct_metric_1qb}
\end{center}
\end{figure}
\FloatBarrier
We see on that graph that the minimum power is a stricly decreasing function of $\mathcal{M}_{\text{target}}$ (whatever the metric we choose: worst-case or average infidelity). This is an illustration of the property \ref{prop:behavior_min_power}. Indeed in the case we study when $T_{\text{Q}}$ increases, the power decreases while the metric increases\footnote{As a side remark, in this case we would have the same kind of behavior for $1/A$: increasing it (thus reducing the attenuation) lower the power but increases the amount of noise}. We also see from the inset \textit{how} the power consumption is being decreased for a higher target: the temperature of the qubits increases. We did not represent it here but we would also see that the optimum attenuation would decrease as a function of $\mathcal{M}_{\text{target}}$. As explained in \ref{sec:equivalence_minpow_maxacc}, we can also switch the interpretation of this curve and realize that it also represents the maximum accuracy (i.e minimum value of $\mathcal{M}_{\text{target}}$) it is possible to reach as a function of some injected power. Finally, this graph also illustrates that the minimum power required depend on the metric that is used. The worst-case fidelity as being "more demanding" will ask for a bigger power consumption to reach a given target in contrary to the average fidelity. To make a connection with the previous section, the minimum power obtained for $\mathcal{M}_{\text{target}}=10^{-4}$ for the average infidelity (it is about $2.10^{-6}$) corresponds to the minimum power we would find along the upper left cyan iso-metric line in figure \ref{fig:min_power_fct_metric_1qb}.
\section{Establishing a full-stack framework: hardware, software, noise, resource approach}
\subsection{Establishing the framework}
At this point, we have shown how parameters describing the "hardware" part of the computer can in principle be optimized given the competition between noise and power ($A$ and $T_{\text{Q}}$ were the variables playing this role). But our example was about a single qubit gate which is not very interesting in practice: the goal of a computer is to run algorithms composed of many gates. In this section we will explain the general approaches we can choose in order to minimize the power consumption of a quantum computer running algorithms. We will naturally generalize the optimization by including in it the "software" part of the problem, i.e the characteristics of the implemented algorithm. It will play a role for two aspects: it will allow us to find which characteristics of the algorithms play an important role in order to estimate the power consumption, but it will also allow us to \textit{optimize} the way the algorithm is compiled in order to minimize the consumption (at least in principle). Finally, we will provide a simple, yet quite general model for the power function $P(\bm{\delta})$ and noise estimation $\mathcal{M}(\bm{\delta})$. We will use a number of assumption in this part, mainly for pedagogic purpose (and also because they are enough for the work that has been done), but generalizations to more general models would often be straightforward. Finally, we will express everything here in term of \textit{physical} qubits and gates which is why all the quantities introduced will have an index $P$. This is in order to anticipate the fault tolerant adaptation of this framework that will be done later in this chapter. It will change some quantitative aspects but the overall philosophy would remain identical as we will see.
\subsubsection{General model behind the resource (power) and the quantity of noise}
\label{sec:formulation_problem_physical}
To begin with, let us try to have some general expression of the power regardless of any optimization (i.e we focus on determining a generic expression for the function $P(\bm{\delta})$ without trying to minimize it based on the metric target). The first thing to acknowledge is that there might have a constant energetic cost regardless of what the computer is doing, i.e if it is running an algorithm or not. We call it the \textit{passive} energetic cost. One typical example of that is the heat conduction: all the cables necessary to control the qubits will always be inside of the computer, and they will bring heat that will have to be evacuated\footnote{We will see other examples of passive cost outside from heat conduction later on.} which costs electrical power for the cryogenic. Here, we will assume that the passive costs scale proportionnally with the number of (physical) qubits $Q_P$ inside the computer but we have to keep in mind that other scaling laws could be involved\footnote{For instance, in an architecture in which the qubits are implemented on a 2D grid, and for which single qubit gate can be done by sending signal in the appropriate (line,column) coordinate, the power would contain a term proportional to $\sqrt{Q_P}$. But even in this case additional terms proportional to $Q_P$ could be expected.}. A scaling proportional to $Q_P$ comes from the fact that the number of cables and amplifiers (amplifier cannot be shutdown when not used, thus they are within the passive costs) is usually increasing proportionally to the \textit{total} number of qubits inside the computer. But in addition to passive costs, there are also the \textit{active} costs. They will increase the power consumption in a manner that is time dependent. The best example of that is the power associated to signals that are being sent to the qubits: they only have to be sent if an algorithm is running and this power might also vary in time within an algorithm\footnote{One concrete example is the power required to remove the heat dissipated into the attenuators: this heat will have to be evacuated only if a gate is acting on the qubits.}. Such power will usually correspond to the moment non trivial gates (i.e not the identity operation) are being applied.\footnote{We should emphasize that it is not always the case. Indeed, there exist schemes in which applying an identity operation on qubits has an energetic cost as it requires to send pulses to \textit{keep} a coupling constant to zero (otherwise the qubit might interact in an undesired manner with the other qubits) \red{cite}.} Here, we will assume that no power is required to implement identity gates, and that some other gates might require a negligible amount of power. We also consider that the algorithm is implemented with a \textit{primitive} gateset (any gate can be expressed as a combination of gates in this gateset). The gates requiring power within this gateset will enter in a family $\mathcal{P}_{a}$ (for power "active" gates), otherwise they will enter in the family $\mathcal{P}_{n.a}$ (for power "non-active" gates). Under those assumptions, the power consumption can thus be written as the following function:
\begin{align}
P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i,
\label{eq:physical_power_gen}
\end{align}
only the family $\mathcal{P}_{a}$ has to be considered for the active power consumption. Here, $a$ represent the power it costs \textit{per qubit} to run the computer. The family of coefficients $\{b^i\}$ represent the power it costs \textit{per active (physical) gate of type "$i$"}(the type of gate corresponds to the precise gate that is being implement: cNOT, Pauli etc) to implement it. The terms $N^{(i)}_{P,\parallel}$ is the number of gate of type $i$ that are activated at a given instant in the algorithm. This quantity in principle \textit{depends} on time (because it is an \textit{active} cost), but from now on, we will assume that we are only interested in the \textit{average} power consumption such that $N^{(i)}_{P,\parallel}$ should be understood as an \textit{average} number of gates activated in parallel.

%, and that all the different gates require the same amount of power \textit{per qubit} involved their dynamic in order to be activated. It means that the active cost will be proportional to the number of physical qubits \textit{actively} participating in the calculation in term of power consumption: $Q_P^{P^a_P} \equiv N_{P,\parallel}^{1qb}+2N_{P,\parallel}^{2qb}$, where $N_{P,\parallel}^{1qb}$ and $N_{P,\parallel}^{2qb}$ respectively represent the average number of single (excluding identity) and two qubit gates acting in parallel inside of the computer\footnote{We assume that all the primitive gates used in the algorithm are either single or two qubit.}. There is no reason to assume that different gates "consume" the same amount of power. But it could be reasonable in some case: the energetic cost to perform a quantum gate is not necessarily only due to the gate physics: it can also be related to the way the signals are generated. If the electronic generating the signals can be turned off when no gates are activated, and if it dominates the details of the gate physics, our assumption would be safe for instance. But as many of the hypothesis we are doing here, it is not strictly necessary, it will just allow us to get a simple and intuitive model on which we will make physical comments. Also, we will only be interested in "order of magnitude" estimations of the energetic cost which makes our hypothesis more legitimate. With those assumptions we deduce, for some coefficients $a$ and $b$: $P=Q_P a + Q_P^{P^a_P} b$. It is usefull to rewrite this expression by introducing the notion of \textit{power-activity} of the qubits. It is defined as
%\begin{align}
%P^a_P \equiv \frac{Q_P^{P^a_P}}{Q_P}
%\end{align} 
%and it physically represents the fraction of qubits that are actively participating in the power function over the total number of qubits (we remind that we reason with average values along the algorithm here). Using this quantity the power then becomes:
%\begin{align}
%P=Q_P (a + P^a_P b).
%\end{align}
%We will make use of that notion in a few paragraphs.

We talked about the expression of the power. Now we must discuss the quantity of noise introduced by the algorithm. In the previous sections we explained why we need a metric to quantify the noise (because it is easier to access than the probability of success of the algorithm), and we gave some conditions it must satisfy (it should have a nice interpretation in such a way that the success probability can be estimated or bounded by this quantity). One requirement that we can ask for the metric to make it suitable for theoretical calculations is that from its value on each individual gates we can bound it for the entire algorithm. It assumes that the effect of the noise is local: it is possible to define a quantum channel for each quantum gate\footnote{Which means in particular that the final quantum state of a given quantum gate can be deduced by the sole knowledge of the state it had at its input.}, and from that to find how much noise a given gate introduces. A typical property allowing it is to ask that:
\begin{align}
\mathcal{M}_P^{\text{exact}} \leq \mathcal{M}_P^{\text{bound}} \equiv \sum_i \mathcal{M}^{(i)}_{P},
\label{eq:sub_additivity}
\end{align}
where $\mathcal{M}_P^{\text{exact}}$ is the \textit{exact} quantity of noise introduced by the algorithm, $\mathcal{M}^{(i)}_{P}$ is an estimation of the quantity of noise introduced by each (physical) quantum gate. The way we will quantify the noise occurring in the algorithm will be based on the best estimation we can have of $\mathcal{M}_P^{\text{exact}}$: $\mathcal{M}_P^{\text{bound}}$. Of course the tighter the bound is to the exact value the better it would be. Then, our metric will be defined as $\mathcal{M}_P=\mathcal{M}^{\text{bound}}_P$ and will verify:
\begin{align}
\mathcal{M}_P=\sum_i N_P^{(i)} \mathcal{M}^{(i)}_{P}.
\end{align}
This property of bounding the quantity of noise is pretty standard to ask, see for instance \cite{gilchrist2005distance}. 
Now, we assume that we can define a clock speed for the algorithm. It means that the algorithm will be implemented in a finite sequence of primitive timesteps all of duration $\tau_P^{\text{timestep}}$. In all of those steps a \textit{unique} primitive gate will be implemented per qubit (or per two qubit if the gate is a two qubit one). The assumption that there is a clock speed is not equivalent to say that the duration to implement all the gates are the same. It just means that if a primitive gate happens to be faster than the timestep, the qubit will then follow an identity evolution until the end of the timestep: $\tau_P^{\text{timestep}}$ thus corresponds to the longest gate in the primitive gateset. Now, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth. This is because we will neglect the final measurements in order to simplify our discussions. Indeed they will have a negligible contribution to the power consumption because they are acting "at the boundary" of the algorithm: their contribution in term of active power consumption or noise will be low compared to all the other gates. It doesn't mean that we will not take into account the cost of measurement amplification: this is usually a \textit{passive} cost that we are going to model (but this will come in the next chapter). Using the depth, we have $N_P^{(i)}=D_P N_{P,\parallel}^{(i)}$, and we can then write:
\begin{align}
\mathcal{M}_P=D_P \left(\sum_{i \in \mathcal{P}_a} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P}+\sum_{i \in \mathcal{P}_{n.a}} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P} \right)
\label{eq:physical_metric_gen}
\end{align}
We notice from this expression that \textit{any} gate occuring in the algorithm might introduce noise. There is thus a difference between being active in term of power consumption and being active in term of information processing. For instance, an identity gate will not require any power consumption but it will introduce nonetheless noise in the computation.
%where $N_P^{(i)}$ is the number of the $i$'th (physical) gate type used in the algorithm and $\mathcal{M}^{(i)}_{P}$ the quantity of noise introduced by this gate. Assuming that all the gates bring an amount of noise proportional to the number of qubit they involve, we have:
%\begin{align}
%\mathcal{M}_P=(N^{\text{1qb}}_{P}+N^{\text{Id}}_{P}+N^{\text{2qb}}_{P}) \mathcal{M}^{(0)}_P,
%\end{align}
%where $N_{P}$ represents the total number of physical gates in the algorithm, and $\mathcal{M}^{(0)}_P$ the metric of each of those gates. In a similar way as what we did for the power, we can also introduce the notion of \textit{information-activity} of the qubits. We define it as:
%\begin{align}
%I^a_P \equiv \frac{Q_P^{I_P^a}}{Q_P},
%\end{align}
%where $Q_P^{I^a_P}=Q_P^{P^a_P}+N^{\text{Id}}_{P,\parallel}$ represents the number of qubits actively participating in the algorithm \textit{on an information processing basis}. We notice that $Q_P^{I^a_P} \neq Q_P^{P^a_P}$. This is because the identity gates in our assumption do not consume any power but introduce noise during the algorithm. 
%
%Now, we can express $I^a_P$ in a more usefull manner for our purpose: assuming that all gates last for the same amount of time, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth (in general we will always neglect the measurements gates in our energetic estimations). Using this, we deduce: $N_{\text{gates}}=Q^{I^a_P}_P D_P$ and thus:
%\begin{align}
%\mathcal{M}_P=D_P Q_P I^a_P \mathcal{M}^{(0)}_P.
%\end{align}
%We see from this expression that $I^a_P$ can then also be interpreted as the portion of "information-active" \textit{gates} there are inside the algorithm over the maximum number of information-active \textit{gates} there could exist for the provided values of $D_P$ and $Q_P$: $D_P Q_P$. This fact and more detailed explanations are provided in the caption of figure \ref{fig:power_information_activity} \textbf{a)}.
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.9\textwidth]{chapter4/images/power_information_activity}
%\caption{\textbf{a)}: An algorithm implemented on four qubits having a depth equal to four. The stars represent identity operations. The square and rectangle represent power-active gates (cNOT, single qubit rotations etc). Each qubit are being measured after the last gate on them have been applied. The blue "area" of the circuit represent the information-active part of the circuit. Because some qubits can be introduced later or measured earlier than at the very beginning or very end of the algorithm, this area is smaller than $Q_P D_P$. \textbf{b)}: An equivalent description of the algorithm when we averaged in time all the dynamic. This description is equivalent in the sense that the average power and metric will be the same as for the "real" algorithm: it is a simpler representation to consider in order to make energetic estimations. We see that $I^a_P$ can be computed by either calculating the ratio of the blue area over the area $Q_P D_P$, either by calculating the average number of information active qubits divided by $Q_P$.}
%\label{fig:power_information_activity}
%\end{center}
%\end{figure}
%\FloatBarrier

\subsubsection{The separate roles of hardware, software and noise in the resource estimation}
At this point the general models for both power and metric are defined. We now summarize and interpret physically what we introduced. First, the power consumption is composed of a passive cost which is here whatever the gates are implemented on the computer. In addition to that there is an active cost which will only be here if gates that require power (which usually exclude the identity gates) are being implemented. This is why knowing the number of qubits inside the algorithm is not enough, one has also to know the number of gates that are actually being implemented as they will \textit{actively} participate in term of power consumption. 

Also, each gate participating in the algorithm "brings in" noise. The more gates are implemented, and the longer it lasts, the more noise there might have. This is represented by the fact $\mathcal{M}_P$ increases if (for other parameter constant) any of the $N^{(i)}_{P,\parallel}$ increases, and by the fact $\mathcal{M}_P$ is proportional to $D_P$. We notice however that because the notion of activity can be different in term of information processing and power consumption, a different counting has to be done about the number of gates acting in parallel: some gates might not require power but will bring in noise. This is represented by the fact that the metric also involve a summation over $\mathcal{P}_{n.a}$.

Once those estimations have been done, the minimization under constraint can be performed as represented on the figure  \ref{fig:general_optimization_principle}.
% NE PAS SUPPRIMER: pour l'image
%\begin{align}
%P(\bm{\alpha},\bm{\beta})=\color{blue}Q_P\color{black}(\bm{\beta})\color{purple}a\color{black}(\bm{\alpha})+\sum_{i \in \color{purple}\mathcal{P}_a\color{black}}\color{blue}N^{(i)}_{P,\parallel}\color{black}(\bm{\beta})\color{purple}b^i\color{black}(\bm{\alpha})
%\end{align}
%\begin{align}
%\mathcal{M}_P(\bm{\alpha},\bm{\beta})=\color{blue}D_P\color{black}(\bm{\alpha}) \left(\sum_{i \in \color{purple}\mathcal{P}_a\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange} \mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha})\color{black}+\sum_{i \in \color{purple}\mathcal{P}_{n.a}\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange}\mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha}) \color{black}\right)
%\end{align}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{chapter4/images/general_optimization_principle2}
\caption{Overall principle of minimization of the power cost. The role of the different components participating to the energetic cost: the algorithm, the engineering part of the computer, the noise model (and the way it is quantified) are represented in blue, purple, orange respectively. They depend on two families of parameters $\bm{\alpha}$ and $\bm{\beta}$. The first one represents the tunable parameters in the physical architecture of the computer. It usually represents the tunable hardware parameters (qubit temperature, attenuation etc) but not only as the clock-speed could also be optimized and it would enter in this family. The second one represents the tunable parameters in how the algorithm is implemented, i.e how it is compiled, and how many qubits it requires.}
\label{fig:general_optimization_principle}
\end{center}
\end{figure}
\FloatBarrier
We see there that the algorithm, the quantity of noise and the engineering part of the model have clearly identified roles. The algorithm characteristics are described by the functions $Q_P(\bm{\beta}), N_{P,\parallel}^{(i)}(\bm{\beta}), D_P(\bm{\beta})$ and they will play a role both in the power and the metric. Indeed if we increase the number of qubits or the number of power-active gates, it will increase the power consumption of the computer. But it also play a role in the metric because longer algorithms, or algorithms that use a greater amount of gates active in parallel will be noisier. Then, the functions describing the power cost (per qubit or per power-active gate) are represented by the functions $a(\bm{\alpha})$ and $b^j(\bm{\alpha})$. Those functions will for instance represent the power efficiency of the cryogenic to remove the heat, how much heat the amplifiers are dissipating, what is the power of the pulse driving the quantum gates, etc. We can say that they represent the characteristics of the engineering aspect behind the computer and will thus only be involved in the expression of the power function. The quantity of noise introduced by the quantum gates will on the other hand only play a role in the metric as represented by the orange color. In summary, each expertise required to build a quantum computer have very well defined parameters to characterize, someone "at the end" has to regroup them and to solve the minimization under constraint which will provide all the experts the optimum tunable parameters they should choose in their respective field of expertise.

We finish by one important remark. We can notice here that despite the fact the gates in the family $\mathcal{P}_{n.a}$ do not require any active power, they will participate in an \textit{indirect} manner to the power consumption. Indeed, they will modify the expression of the metric and thus change the value of $P_{\min}$. As a concrete example, it is frequent to try to minimize the number of identity gates inside algorithms because the metric would then be lower \red{cite}. But with our approach of finding the minimum power, we will see that sometimes it can be helpful to introduce such elements because they could to reduce the amount of active gate in parallel. This will be a concrete example of the fact that despite they do not "directly" require power, identity operations "indirectly" influence the energetic cost required to run an algorithm, and we are going to illustrate it right now.
\subsection{Example: application to the energetic cost of an algorithm}
Now, we can design an example in which we will optimize the shape of an algorithm that is running, in addition to the family of tunable parameters $\bm{\alpha}$ that play a role for the metric and the "engineering" part of the model. We will stay with the same model of power consumption we considered in the single qubit gate example (only the power dissipated into the attenuator will play a role). Thus, with the vocabulary we introduced, we will neglect any \textit{passive} cost involved in the computation. For the noise model, we will keep the assumption that only the thermal noise will affect the qubit and we will model it in the exact same manner as before. For the metric quantifying this noise, we will consider the worst-case infidelity of the gates as it verifies the property \ref{eq:sub_additivity} (the average infidelity wouldn't satisfy this property for instance \cite{carignan2019bounding}). Also as we are going to see we will only need two qubit and identity gates in the algorithm. The two qubit and identity gates will be assumed to last for a duration $\tau^{\text{timestep}}_P=25ns$. As we are going to keep the same noise model for each qubit as the one we introduced in the section \ref{sec:single_qubit_example}, the identity gates will be as noisy as a single qubit $\pi$-pulse (lasting $25ns$), and the two qubit gates twice as noisy as the identity gates (because two qubits are involved in their dynamic, and because they last for the same duration). Those two qubit gates will also require twice the power consumption of a $\pi$-pulse because they involve two qubits (identity gates will be "power free"). Of course there is nothing obvious behind this it is just a simple way to model the power consumption and noise behind the gates we used. This $\pi$-pulse will have the same properties than the one used in the previous section\footnote{It means that $\gamma_{\text{sp}}=1kHz, \tau=25 ns$}. Thus in this simple example we will have $\mathcal{P}_{a} = \{\text{2qb}\}$, $\mathcal{P}_{n.a} = \{\text{Id}\}$, $P=Q_P a +N^{(\text{2qb})}_{P,\parallel} b^{\text{2qb}}$ with:
\begin{align}
&a=0\\
&b^{\text{2qb}}=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A (2 \times P_g),
\label{eq:power_nisq}
\end{align}
and $\mathcal{M}_P=D_P \left(N_{P,\parallel}^{(\text{2qb})} \mathcal{M}^{(\text{2qb})}_{P}+N_{P,\parallel}^{(\text{Id})} \mathcal{M}^{(Id)}_{P}\right) $, with:
\begin{align}
 \mathcal{M}^{(\text{Id})}_{P}=\mathcal{M}^{(\text{2qb})}_{P}/2=(1+\overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(300)}{A}) \gamma_{\text{sp}} \tau_P^{\text{timestep}}.
\end{align}
We recognize $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})+\overline{n}_{\text{BE}}(300)/A$ in this expression. We also see that we assumed $A \gg 1$ (as it will anyway be necessary to reach $\mathcal{M}_P=\mathcal{M}_{\text{target}}$ in what follows). We will ask an accuracy being $\mathcal{M}_{\text{target}}=1/3$ which implies that the fidelity of the algorithm output will be better than $2/3$ (because the metric is a pessimistic estimation: the "real" output fidelity will be better than the worst case one\footnote{And also because as explained before, the expression of $\mathcal{M}_P$ is only a bound on the exact value of the worst-case fidelity of the algorithm.}). 

Now, we need to describe the algorithm which will give us access to the average number of gate acting in parallel and $D_P$. For this example, we will consider running the quantum Fourier transform that we already introduced in the previous chapter. It will be directly implemented on physical qubits (not error correction yet). Of course, such algorithm is unlikely to be applied in the next few years on NISQ platforms as qubits are way too noisy: the task it would solve would be easily solved by a classical computer. But we take this as a simple example of the principle which could then be applied to more relevant NISQ (and also fault tolerant) algorithms. In order to simplify the discussion we will remove all the Hadamard gates that are required in this algorithm (they wouldn't change the general behavior we are going to show). The algorithm is represented for $5$ qubits on the figure \ref{fig:qft_5qubits}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/qft_5qubits}
\caption{\textbf{a)}: The QFT (where Hadamard gates have been removed for simplicity) performed on $5$ qubits with no compression. The vertical dotted lines represent the different timesteps of the circuits. On some of those timesteps, some qubits are waiting as represented by the stars indicating the associated "identity gates". Some other qubits are participating in a two qubit controlled-phase gate (which we described in the previous chapter). To reduce the level of noise, we can compress the circuit. It can be done by moving toward the left the different subcomponents represented by the colors (black, gred, yellow and blue). The red arrow represents how to do the first level of compression represented on \textbf{b)}. The red, yellow and blue subcomponents are pushed toward the left for two timesteps to put the first red two qubit gate inside the red dotted rectangle (removing the identity gates that were there). \textbf{b)}: First level of compression. The red, yellow and blue circuits have been pushed toward the left such that the first red two-qubit gate is done during the third timestep in parallel of the two qubit gate performed between the first and fourth qubit. \textbf{c)}: Second level of compression. The yellow subcomponent has also be pushed on the left (inside the yellow dotted rectangle) to reduce even more the algorithm duration and thus the noise. No further compression are possible. We can thus define a compression level for any size of QFT: $\epsilon=N_{\text{comp}}/N^{\max}_{\text{comp}}$ where $N_{\text{comp}}$ is the number of compression done and $N^{\max}_{\text{comp}}$ the maximum one (which is equal to $2$ in this example).}
\label{fig:qft_5qubits}
\end{center}
\end{figure}
As we see there are different way to actually implement it. Either we run the algorithm in an "uncompressed" manner as on the figure \ref{fig:qft_5qubits} \textbf{a)}, either we try to compress its length in such a way that the moments where qubits are waiting is minimized (on \textbf{c)}). The standard vision to implement algorithms is to make them the shortest possible. Indeed doing things this way the quantity of noise that is introduced is then minimal. But it might not be the best way to do things in order to minimize power consumption \textit{under the constraint} of aiming a targetted fidelity. Indeed, if the algorithm is highly compressed then a lot of gates are running in parallel which induces a big amount of active power consumption. More precisely, in this regime, the noise might be low (which implies that the qubits can be at higher temperature), but the heat dissipated in the attenuators will be high. Thus on one hand the power cost is minimized because the Carnot efficiency is higher, but we have more heat to evacuate. In the other limit it is the opposite. If the algorithm is minimally compressed (i.e more qubits are waiting), the noise will be higher (the qubits have to be colder) but the heat dissipated will be lower. In the end, the optimal way to compress the algorithm is not obvious if one wants to minimize the power consumption. To choose the optimal way we should compress the algorithm, we then introduce the parameter $\epsilon \in [0,1]$. It is defined as the number of compression it is possible to do over the maximum number of compression we can do: $\epsilon=N_{\text{comp}}/N_{\text{comp}}^{\max}$. The exact definition of a compression is given in the caption of the figure \ref{fig:qft_5qubits}. The other parameters we will optimize will be as previously $T_{\text{Q}}$ and $A$.
 
%It brings us to the last point: we explained which noise model, metric and resource to minimize (the expression of the power). The last thing to provide is the set of parameters on which the optimization can be performed. We are interested in the minimum power to implement this algorithm assuming that we can tune $T_{\text{Q}},A$ and $\beta \in [0,1]$, where $\beta \in [0,1]$ is the compression level which is defined in the caption of figure \ref{fig:qft_5qubits}. They are thus the parameters on which the optimization should be performed. But to get intuition behind the role of the compression factor, we will calculate the minimum power, minimized on the set $\bm{\alpha}=\{T_{\text{Q}},A\}$ for different values of $\beta$, and we will see for which value of $\beta$ the curve reaches a minimum. 

We now represent the minimum power consumption (minimized on $T_{\text{Q}},A$) as a function of $\epsilon$ in order to visualize the influence of the compression. It is represented on the figure \ref{fig:min_power_fct_compression}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/min_power_fct_compression}
\caption{Minimum power for a QFT implemented on $30$ qubits (minimized on $T_{\text{Q}},A$) as a function of the compression factor $\epsilon$. Bottom left inset: zoom around the minimum. Upper right inset: optimal temperature $T_{\text{Q}}^{\text{opt}}$ as a function of the compression factor. On this curve, we see that the algorithm should be implemented with a compression factor about $\epsilon^{\text{opt}} \approx 0.75$. The bigger the compression is, the higher the temperature can be which improves the Carnot efficiency. But at the same time, more power-active gates are implemented in parallel which dissipates more heat into the attenuators. The optimal compression factor results from this competition.}
\label{fig:min_power_fct_compression}
\end{center}
\end{figure}
\FloatBarrier
In this curve, we see that as expected there is an optimal compression factor on which the algorithm should be implemented in order to minimize the power consumption. It results from the competition we just described. This curve has been represented for a QFT implemented on $30$ qubits but when we increased the size of the QFT, the same kind of behavior remained: there were an optimal compression factor to choose resulting from the competition between noise and power. We also see that the optimization can be quantitative: the curve varies on more than one order of magnitude on the range of compression factor we considered. We could however consider that the conclusion of this curve is that the algorithm should anyway be close to a maximum compression (the power for a maximal compression would not be much higher than the minimum). But in practice we can expect the conclusion to be very system dependant: it highly depends on the characteristics of the algorithm implemented, the engineering aspect behind the computer, the noise model behind the quantum gates and the metric used to quantify it. We mainly took this specific example of the QFT because we already introduced the algorithm (and we will reuse it later on). 

The message we want to give here is simply that it is possible to optimize algorithms to make them minimize the power of the computer, and this minimization should at the same time involve the physical "hardware" parameters describing the computer. Here we took the simplest possible example which consisted in adding or removing identity operations, but the overall principle would remain if a given algorithm can be implemented in various manner. For instance, if different kind of gates can be used: some consume low power but introduce a high noise (and reciprocally), the optimal way to compile the algorithm could be deduced allowing to introduce energetic considerations in algorithm compilation problems.
\section{Adapting the full-stack framework for fault-tolerance}

Now, that the concepts have been provided for a computer not using quantum error correction, we would like to adapt them to fault tolerant quantum computing. This is the role of this section. Ideally, we would like to keep the same interpretation of those quantities and replace all the physical quantities such as physical depth, number of qubits, power and number of active parallel gates by their logical equivalent. Under some approximations, we will see that it is possible to do so, at least for concatenated codes. However we will also see that some differences will remain: the notion of power and information activity will be a little bit different here.
\subsection{Metrics at the logical level}
Let us talk about the metric first. For that, we will use the tools that we already introduced: the probability of error of a logical gate\footnote{We remind that in general $p_L$ has not necessarily the interpretation of a probability, in more general case it is a mathematical norm (which can usually be related to a probabilistic interpretation). It will be the case if the noise model behind the physical gate is probabilistic. To keep the explanations simple we nonetheless assume the probabilistic interpretation to be appropriate.}. Calling it $p_L$, the probability that any of the gate in a computation composed of $N_L$ logical gates fails is simply $N_L p_L$. The implicit assumption here is that all gates have the same failure probability. This is not true but fault-tolerance very frequently reason on worst-case scenario (because more accurate estimations are complicated). Thus, here, $p_L$ actually corresponds to the probability of failure of the "worst" logical gate: $N_L p_L$ is an over estimation of the probability of error that will be our estimation of the quantity of noise introduced in the algorithm. In some sense, considering the algorithm as a big logical gate, $p_L$ will play the role of what measures the quantity of noise in a (logical) gate, and will verify the sub-additivity property \eqref{eq:sub_additivity}. Because of that the general description we did is still valid at the logical level, and we have a particular case of \eqref{eq:physical_metric_gen}:
\begin{align}
&\mathcal{M}_L=D_L \left(\sum_{i \in \mathcal{P}_{L,a} \cup \mathcal{P}_{L,n.a}} N_{L,\parallel}^{(i)} \right) \mathcal{M}^{(0)}_{L}\\
&\mathcal{M}^{(0)}_{L} = p_L,
\end{align}
where $\mathcal{P}_{L,a}$ and $\mathcal{P}_{L,n.a}$ represent the family of power-active and power non-active logical gates (we will actually see that in fault-tolerance, $\mathcal{P}_{L,a}=\mathcal{P}_{L,n.a}$). In the end, we notice that the metric we used before is simply switched at the logical level. Everything behave in the exact same manner.
\subsection{Power at the logical level}
Now, we can talk about the power part of the problem. One question is to wonder if it is possible to define it in an "effective manner" at the logical level. Can we just replace all the physical quantities entering in this expression by their logical counterpart and keep the same interpretation ? To answer this question, we need to find the expression of the power (thus breaking down the fault-tolerant algorithm into its physical components) to try to then "recognize" the logical components with the hope that it can lead to a nice expression, analog to \eqref{eq:physical_power_gen}. The first step will thus be to estimate the number of physical components (qubits and gates) that are required in a fault-tolerant algorithm. This is the role of this section. 

\subsubsection{The general construction behind FT logical gates}
To begin, we need to remind the how a level-1 logical gate is constructed from physical elements, more precisely, a 1-Rec as defined in the chapter 2. It is represented for a single qubit logical gate on the figure \ref{fig:steane_method_full_ch4}. The construction of a two qubit logical gate such as a cNOT follows the same structure excepted that error correction will be performed on the two logical data qubits (thus, we would need all the structure involving the ancilla "twice", one per logical qubit).
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/steane_method_full}
\caption{Fault-tolerant implementation of a single qubit logical gate for one concatenation, based on Steane method. Each horizontal line represents a logical qubit for one concatenation level, composed of seven physical qubits (because we use Steane code). The first line represents the logical data qubit: i.e the logical qubit participating in the calculation. The four bottom line are the four \textit{ancilla} logical qubits that are required to implement fault-tolerantly the error correction. We need at least (further details in the text) two syndrome ancilla (which are interacting with the logical data qubit to measure the syndrome), and two verifier logical ancilla (which are here to check that the syndrome ancilla do not contain error that could damage the data qubits). The preparation procedure for the ancilla qubits is represented on the figure \ref{fig:preparation_0logical_ch4}.}
\label{fig:steane_method_full_ch4}
\end{center}
\end{figure}
\FloatBarrier
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/preparation_0logical}
\caption{Preparation of the $\ket{0_L}$ logical state. The preparation of the $\ket{+_L}$ logical state can be done via a similar procedure where (i) the direction of all the cNOT is being reversed (ii) four hadamard are added on the four qubits not affected by Hadamard here, right after their initialization in $\ket{0}$, (iii) the three Hadamard of this figure are being removed.}
\label{fig:preparation_0logical_ch4}
\end{center}
\end{figure}
\FloatBarrier
The role of each of those components has already been explained in the second chapter of this thesis, but we briefly remind them. The unprotected 1-Ga logical gate is implemented right before the purple box. It is implemented by a transversal implementation of the gate (i.e if the logical gate is Hadamard, the 1-Ga is implemented by applying a Hadamard on each physical qubit). It is then followed by quantum error correction called 1-Ec which requires two "syndrome" logical ancilla corresponding to the second and third black lines of figure \ref{fig:steane_method_full_ch4}. Their role is to detect $X$ and $Z$ errors occuring on the data qubits to know which appropriate correction should be implemented. The correction can then be applied. However, it is not strictly a requirement in practice: indeed it is enough to "keep track" of the errors with a classical computer, more precisely to keep in memory the result of the syndrome\footnote{In principle the correction must be applied only before a non-transversal gate which is done through a different procedure as the one shown on figure \ref{fig:steane_method_full_ch4}. Those gates, called magic-gates go beyond the scope of this thesis.}. This is why in the calculations we will not include the cost of the correction following the syndrome\footnote{\red{Comment about magic gate for this}}. Now, for the construction to be fault-tolerant, verifier logical ancilla are required and represented by the third and last black line. They are interacting with the syndrome logical ancilla before being measured. This measurement is here to ensure that the potential faults that might have occured during the preparation of the syndrome ancilla will not corrupt the logical data qubit. Given the value of this measurement, the syndrome ancilla will either be accepted (and interact with the data qubit to detect the potential errors), or will be rejected. In the scenario it is rejected, new verifiers and syndromes ancilla have to be generated until the moment the verification succeeds. In principle, "many" syndromes and verifiers ancilla have to be prepared in parallel so that one will always be accepted when needed. In practice, the extra amount of those ancilla required will be negligible. Indeed based on the fact that it is more probable for an ancilla to be accepted (because in fault-tolerance the probability of errors are anyway low), the extra amount of ancilla one would need to prepare in the case of failure will be smaller than the number of ancilla we would need in case the acceptation always succeeds. It will then be possible to neglect them in our energetic estimation. We show this property more rigorously in the appendix \red{to write down}. In the end, this circuit, drawed for each logical gate we want to implement, and the principle behind the concatenation is all what we need conceptually to deduce the number of physical qubits and gates that are required in a 1-Ec after $k$ level of concatenations. The exact counting of the number of physical element will differ for each logical gate one want to implement but the principle will be the same.

We show the principle of the calculation for a single qubit logical gate and single qubit identity gate. What we refer as single qubit physical gate will either be Pauli or Hadamard (in our energetic estimation we will identify those gates as if they were the same). We assume that we want to implement a 1-Rec for such single qubit logical gate. Assuming that the syndrome ancilla are always accepted, we need $7 \times 5 = 35$ physical qubits: $7$ for the logical data qubit, $7 \times 2$ for the syndrome ancilla qubits and $7 \times 2$ for the verifier ancilla qubits. We can also find the number of physical gates required. In order to make this counting, we assume that we can only do measurement in the computational basis ($Z$-measurement): measuring in the $X$ basis requires to apply Hadamard gates before a $Z$-measurement. We also assume that qubits can only be available in their ground state $\ket{0}$ (preparing $\ket{+}$ requires to apply an Hadamard on $\ket{0}$). With those assumptions we find that we need $7 \times 4+9 \times 4=64$ cNOT: $7 \times 4$ for the transversal implementation of the cNOT represented on the figure \ref{fig:steane_method_full_ch4}, and $9 \times 4$ for the preparation of the $\ket{+_L}$ and $\ket{0_L}$ states for the ancilla (see figure \ref{fig:preparation_0logical_ch4}). For the measurement gates, we need $7 \times 4$ of them to measure all the ancilla. We also need single qubit gates: $7$ for the transversal implementation of the gate at the logical data qubit, $7 \times 2$ Hadamard to apply before the $X$-measurement (because we can only to $Z$-measurements), and $3 \times 2 + 4 \times 2 = 14$ Hadamard for the preparation of the ancilla states as explained in the caption of figure \ref{fig:preparation_0logical_ch4}. It gives us $35$ single qubit gates to apply. We also need to make some qubits necessarily wait at some point. For instance, the syndrome logical qubits have to wait for the measurement outcome of the verifier to know if they can be injected or not: they are then doing a noisy physical identity. We won't go in the detail of this counting but in the end, we would find $36$ physical identity gates by looking at all the places the physical qubits composing the logical ones necessarily have to wait. In the end, doing an appropriate counting for each type of logical gate that has to be implemented, we have access to the table \ref{table:FT_gate_breakdown} which represents for each level-1 gate (on the line), the number of physical elements (on the column) its 1-Rec is composed of \footnote{To be very precise, the 1-Rec of a measurement is defined as 1-Ec followed by 1-measurement (the 1-Ec is "before" the 1-Ga measurement gate). This is defined this way for theoretical reason to prove the threshold \cite{aliferis2005quantum}. As we are interested to find the number of physical elements when concatenating, the elements in this 1-Ec would already have been counted by the gate before the measurement: taking them into account "again" would lead to an overcounting of the number of physical elements. This is why we remove the elements that would be in the 1-Ec before the measurement gates which explains why the last line of table \ref{table:FT_gate_breakdown} is composed of three zeros.}. We see from this table that as we could expect, a logical identity is the same as a logical single qubit gate excepted that the transversal operation is composed of identity gates. This is why it contains $7$ less single qubit gate but $7$ more identity gates than a logical single qubit gate.
\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
	\hline
	& lvl-0 cNOT & lvl-0 Single & lvl-0 Identity & lvl-0 Measurement\\
	\hline
   lvl-1 cNOT & $135$ & $56$ & $72$ & $56$ \\
   \hline
   lvl-1 Single & $64$ & $35$ & $36$ & $28$ \\
   \hline
   lvl-1 Identity & $64$ & $28$ & $43$ & $28$\\
   \hline
   lvl-1 Measurement & $0$ & $0$ & $0$ & $7$\\
   \hline
\end{tabular}
\caption{Each row lists a FT logical gate and tabulates the lower level components required for the listed gate as columns. Those level-0 components are thus physical gates. The single qubit gates here are either Hadamard or Pauli gates.}
\label{table:FT_gate_breakdown}
\end{center}
\end{table*}
\FloatBarrier
\subsubsection{Estimation of the number of physical gates acting in parallel}
\ref{sec:estimation_physical_gates}
This table allows us to deduce, based on a recursive reasoning the number of physical qubits and gates of each type that are required for a level-k logical gate. Let us start with the number of physical gates. We assume that we have $N_L^{\text{cNOT}}$, $N_L^{\text{1qb}}$, $N_L^{\text{Id}}$,$N_L^{\text{Meas}}$ logical cNOT, single qubit, identity gates and measurement gates in the algorithm. We put the number of logical gates required by the algorithm in a three dimensional vector $X_0=(N_L^{\text{cNOT}},N_L^{\text{1qb}},N_L^{\text{Id}},N_L^{\text{Meas}} )^T$. We can deduce the number of physical gates of each type after $k$ level of concatenations via the recursive formula $X_k=A^k X_0$, where:
\begin{align}
& A=\begin{pmatrix} 135 & 64 & 64 & 56\\ 56 & 35 & 28 & 28\\ 72 & 36 & 43 & 28 \\ 0 & 0 & 0 & 7\end{pmatrix},
\end{align}
and where the first line of $X_k$ will represent the number of physical cNOT, the second line, the number of physical single qubit (either Hadamard or Pauli), the third line the number of physical identity gates where the qubits have to wait for one physical timestep, and the last one the number of physical measurement gates. The formula for $k=1$ is just applying the table \ref{table:FT_gate_breakdown} to the number of gates implemented in the algorithm. It gives us the number of physical gates after the first concatenation level. Each of them are then "promoted" into 1-Rec for the second concatenation level: we just have to "reuse" this table another time on the vector $X_1=A X_0$. The same principle applies recursively for further concatenation levels which explains why $X_k=A^k X_0$. In the end, from the knowledge of the number of gates required by the algorithm, we can access the number of physical gates required in the algorithm for an arbitrary concatenation level. We deduce that we have the following \textit{total} number of physical gates required in the algorithm:
\begin{align}
X_k = \left(
\begin{array}{c}
 \frac{1}{3} 199^k (2 N_L^{\text{cNOT}}+N_L^{\text{Id}}+N_L^{\text{1qb}})+\frac{7^k}{3} \left(N_L^{\text{cNOT}} -N_L^{\text{Id}} - N_L^{\text{1qb}}\right) \\
 \frac{7}{48} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{48} \left(-14 N_L^{\text{cNOT}} -7 N_L^{\text{Id}} +41\  N_L^{\text{1qb}}\right) \\
 \frac{3}{16} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{16} \left(-6 N_L^{\text{cNOT}} +13 N_L^{\text{Id}} -3\ N_L^{\text{1qb}}\right) \\
 \frac{7}{48} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{48}\left(-14 N_L^{\text{cNOT}} -7 N_L^{\text{Id}}+48N_L^{\text{Meas}}-7N_L^{\text{1qb}}\right)\\
\end{array}
\right)
\label{eq:number_physical_gate_k_concat}
\end{align}
We notice from this expression that two numbers seems to have a particular importance in this formula: $199$ and $7$ (they are the only two numbers elevated to a power $k$). They correspond to the two eigenvalues of the matrix $A$. In order to interpret their signification, let us first neglect the term proportional to $7^k$. Doing this, we realize that $X_k \propto (2 N_L^{\text{cNOT}}+N_L^{\text{Id}}+N_L^{\text{1qb}})$. It means that whatever the physical gate we are looking at, the exact type of gates implemented by the algorithm does not really matter, what matters is the \textit{total number} of logical gates involved (counting twice the cNOT, and removing the measurement gates at the logical level for a reason given in a few lines). For instance, if we had implemented $1$ logical identity, or $1$ single qubit logical gate (and no other gates), the number of physical components of each type wouldn't change. It symbolises the fact that the fault tolerant construction of the gates contains a dominant part that does not really depend on the gate that is being implemented, and we can understand that from the figure \ref{fig:steane_method_full_ch4}: whatever the 1-Ga has to be protected, the error correction structure (i.e the 1-Ec) is the same for any of the logical gate to implement. But this has two exceptions: first we need two implementation of error correction for a cNOT because it involves two logical qubits, it explains the $\times 2$ in front of $N_L^{\text{cNOT}}$. Then, the measurement gates will not be followed by error correction (because the information becomes classical when qubits are being measured). It explains why $N_L^{\text{Meas}}$ does not appear in the term proportional to $199^k$: the number of logical measurement gates does not play a significant role in the number of physical elements when concatenations are being performed. But the error correction is not everything, there is also the transversal implementation of the gate (the 1-Ga). And this part will differ depending on the exact logical gate we want to implement. For instance a logical identity gate would require $7$ less single qubit gate and $7$ more identity gates to be implemented. Those little differences are expressed by the much smaller eigenvalue $7$. And we see that the terms proportional to this eigenvalue are not the same for each physical gates (because here, there are variation depending at the logical gates that have been implemented). 

Now, we are here interested in the \text{average} number of physical gate that are acting in parallel. In order to access it, we need to know the average number of gate acting in parallel for the ideal algorithm (for each type: single qubit, identity and two qubit gates). Putting those number in a vector $X_0=(\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}},\overline{N}_{L,\parallel}^{\text{Meas}})^T$, we can deduce the total number of physical gate inside an average algorithm logical timestep (one algorithm timestep correspond to the time it takes to execute any logical gate\footnote{Some logical gates can in principle be implemented faster than others. For instance a logical identity could only last for two timestep as the transversal implementation of the gate could be done instantaneously (as an identity operation can be performed instantaneously). But as we need to keep all the qubits "synchronized" the longest logical gate to execute should give the duration of a logical timestep of the algorithm (even though "smart" optimizations could be performed for specific algorithms in order to reduce slightly the algorithm duration).}). It naturally corresponds to \eqref{eq:number_physical_gate_k_concat} where we replace the number of logical gates by the number of logical gates acting in parallel ($N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb},\text{Meas}\}$). Now, this is not exactly the average number of physical gates that are acting in parallel. Indeed, a logical timestep is composed of a given number of physical timesteps. More precisely, calling $\tau_P^{\text{timestep}}$ the duration of a physical timestep (which corresponds to the duration of the longest physical gate used in the FT construction: we will assume it corresponds to both the duration of a cNOT and measurement gates in what follows), we have after $k$ concatenations a logical gate that lasts for $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. Indeed, we can see from figure \ref{fig:steane_method_full_ch4} that for one level of concatenation, the logical data qubit are going through three timesteps: the first one corresponds to the transversal implementation of the gate, followed by two timesteps used to perform the syndrome measurement\footnote{We remind that we assume the correction is not physically performed with out assumptions of "keeping track" of the syndrome with a classical processing.}. Increasing the concatenation level, each of those timestep will again be multiplied by three. This is how we deduce $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. We notice here that the ancilla must however be prepared in advance: including their preparation and the moment they can be "plugged out", the duration of this gate would be longer. But as explained on the figure \ref{fig:timestep_logical_gate}, the good timescale to consider to estimate the average number of gates would still be $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/timestep_logical_gate}
\caption{Determination of the average number of physical gates acting on an average logical timestep. On the first line of this figure are represented a sequence of three logical gates that are composed of three physical timesteps as indicated by the three red rectangles (the transversal implementation, and the measurement of the $X$ and $Z$ syndromes). Those logical gates require ancilla which are represented on the line below by the matching colors. Between the moment the ancilla are prepared and measured, there is more than three timesteps (we represented $6$ here for simplicity, but the exact number would be different and would actually depend on the ancilla we are looking at). However, in order to compute the average number of physical gates acting in one logical gate, everything will behave \textit{as if} those gates were actually implemented in parallel of the $3$ timesteps. Indeed, if we focus on the red logical gate, the ancilla might have gates applied on them before ($1$ and $2$ red boxes) and after the logical gate ($6$ red box), but the preceding and following logical gates would exactly compensate those missing gates. More precisely, this is true if we neglect the boundary of the algorithm and if we are interested into the average number of gates acting in parallel (which is the case).}
\label{fig:timestep_logical_gate}
\end{center}
\end{figure}
\FloatBarrier
%Finally, calling $\tau_P^{\text{1qb}}$ and $\tau_P^{\text{cNOT}}$ the duration of the physical single and cNOT gates respectively, the average number of single and two physical qubit gates acting in parallel in the algorithm can be expressed as:
Finally, the average number of $x \in \{\text{cNOT}, \text{Id}, \text{1qb},\text{Meas}\}$ physical gates in this logical timestep is:
\begin{align}
&\overline{N}_{L,\parallel}^{x}(k)=N_{\text{during } \tau_L}^{x}(k) /3^k
\label{eq:average_number_physical_gate_timestep}
\end{align}
Where $N_{\text{during } \tau_L}^{x}(k)$ is the number of $x$ type physical gates that are inside an average logical timestep, i.e the number of $x$ physical gates there are assuming that $\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}},\overline{N}_{L,\parallel}^{\text{Meas}}$ logical gates are acting in parallel in the algorithm. We find (those numbers are simply obtained by replacing $N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb}\}$ in \eqref{eq:number_physical_gate_k_concat}):
\begin{align}
&N_{\text{during } \tau_L}^{\text{cNOT}}(k)= \frac{1}{3} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{3} \left(\overline{N}_{L,\parallel}^{\text{cNOT}} -\overline{N}_{L,\parallel}^{\text{Id}} - \overline{N}_{L,\parallel}^{\text{1qb}}\right)
\label{eq:tot_number_physical_gate_timestep1}\\
&N_{\text{during } \tau_L}^{\text{1qb}}(k)=\frac{7}{48} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{48} \left(-14 \overline{N}_{L,\parallel}^{\text{cNOT}} -7 \overline{N}_{L,\parallel}^{\text{Id}} +41\  \overline{N}_{L,\parallel}^{\text{1qb}}\right)
\label{eq:tot_number_physical_gate_timestep2}\\
&N_{\text{during } \tau_L}^{\text{Id}}(k)= \frac{3}{16} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{16} \left(-6\overline{N}_{L,\parallel}^{\text{cNOT}} +13\overline{N}_{L,\parallel}^{\text{Id}} - 3 \overline{N}_{L,\parallel}^{\text{1qb}}\right) 
\label{eq:tot_number_physical_gate_timestep3}\\
&N_{\text{during } \tau_L}^{\text{Meas}}(k)= \frac{7}{48} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{48} \left(-14 \overline{N}_{L,\parallel}^{\text{cNOT}} -7 \overline{N}_{L,\parallel}^{\text{Id}}+48 \overline{N}_{L,\parallel}^{\text{Meas}} - 7 \overline{N}_{L,\parallel}^{\text{1qb}}\right) 
\label{eq:tot_number_physical_gate_timestep4}
\end{align}
The second parenthesis of those expressions becoming negligible\footnote{We are only interested in order of magnitude estimations. So for us a quantity will be negligible with respect to another one as soon as it is smaller (or equal) to it which is clearly the case here.} to the first one as soon as $k=1$, and because we won't need to find the average number of physical identity gates (because they are not consuming any power), we will approximate the average number of physical single, cNOT and measurement gates by:
\begin{align}
&\overline{N}_{L,\parallel}^{\text{cNOT}}(k) \approx \frac{1}{3} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep1}\\
&\overline{N}_{L,\parallel}^{\text{1qb}}(k) \approx \frac{7}{48} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep2}\\
&\overline{N}_{L,\parallel}^{\text{Meas}}(k) \approx \frac{7}{48} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep3}
\end{align}
We notice that the number of physical measurements is roughly the same as  the number of the other physical gates (actually it is exactly equal to the number of single qubit gates for instance). This is an important difference with the case where no error correction is being performed. Indeed when no error correction is performed it is fine to neglect the active cost associated to measurements because they only affect the boundaries of the algorithm. Here, because error correction is being performed, measurements are performed on each logical timestep and their active energetic cost might not be negligible.
\subsubsection{Estimation of the number of physical qubits used in the computer}
\ref{sec:estimation_physical_qubits}
The number of physical gates being estimated for a given concatenation level $k$, it remains to estimate the number of physical qubits to be able to finally write down the expression of the power. For the physical gates, we were interested in finding their average number because the associated power consumption was an active type. For the physical qubits, we need to find the bottleneck of the algorithm. Indeed physical qubits cannot be removed from the computer when they are not being used, so we need to find the moment when the maximum number of physical qubits will be required to estimate their number. 

In order to do the estimation, we notice that the number of ancilla qubits dominates the total number of physical qubits required. Indeed, for $k=1$ for instance we would need $28$ (resp $28 \times 2$) ancilla qubits for a single or identity (resp cNOT) logical qubit gate. Compared to the $7$ to $14$ physical data qubits, as we are only interested in order of magnitude this is a fair approximation to make. Furthermore, increasing the concatenation level would only make the number of physical ancilla qubits dominate even more. For this reason, we will only try to estimate the number of ancilla qubits. Then, we remind that the $k$'th concatenation level is obtained from the $k-1$ level in which each physical gate has been promoted into a 1-Rec. Thus, we can estimate the number of physical qubits. We first assume that the algorithm requires a unique logical timestep composed of $(N_{L,\parallel}^{\text{cNOT}},N_{L,\parallel}^{\text{1qb}},N_{L,\parallel}^{\text{Id}},N_{L,\parallel}^{\text{Meas}})$ cNOT, single, identity and measurement logical gates acting in parallel. From this knowledge, we can find the the total number of physical gates required on the $k-1$ level. Multiplying this number by $28$ for the single qubit and identity gates, and $28 \times 2$ for the cNOT, we deduce the total number of ancilla qubits required. We notice that we don't multiply measurement gates by $28$ because they do not require ancilla (because they are not followed by a quantum error correction procedure). It would give us access to the total number of ancilla qubit after $k$ concatenation, and thus roughly the total number of physical qubits. We notice that this calculation assumes that no ancilla qubits can be recycled after $k$ concatenation (i.e each gate on the $k-1$ level needs "fresh" ancilla). The $X$-syndrome ancilla are participating to $9$ physical timesteps. Thus, in principle, we can reuse them once they have done those $9$ timesteps. In a similar way, the verifier ancilla can be reused (even earlier because they are used for a smaller amount of timesteps). Properly counting the number of ancilla that could be reused would however be a complicated task for an arbitrary concatenation level. Furthermore, in practice we will mainly be interested in the first $3$ concatenations levels in the next chapter (more concatenation level would imply an unrealistic power demands for all practical purposes, with the models we will consider in the following chapter). Because of that, the number of timesteps for the logical gates on the $k-1$ level is also equal to $9$: $\tau^{\text{timestep}}_L/\tau^{\text{timestep}}_P=3^{k-1}=9$ which means that anyway the level of recycling of the syndrome ancilla qubit would be "poor" (but we might be able to recycle roughly half of the verifier ancilla qubits). We assumed in the end that the ancilla qubits are not recycled within this logical gate which gives a slight overestimation of the total number of physical qubits that would really be required. In summary, using \eqref{eq:tot_number_physical_gate_timestep1},\eqref{eq:tot_number_physical_gate_timestep2} and \eqref{eq:tot_number_physical_gate_timestep3}, we can estimate that the total number of physical qubits required in an algorithm composed of a unique logical timestep having $(N_{L,\parallel}^{\text{cNOT}},N_{L,\parallel}^{\text{1qb}},N_{L,\parallel}^{\text{Id}},N_{L,\parallel}^{\text{Meas}})$ cNOT, single, identity and measurement logical gates acting in parallel is $Q_P(k) \approx \frac{28}{199} 199^k (2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}})$. Now, an algorithm is composed of many logical timesteps. With our assumption where the ancilla qubits are not being recycled within a logical gate, the number of physical qubits required is given by the moment in the algorithm where $2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}$ will be \textit{maximum} (which is in some way the "bottleneck" in term of physical resources required). Thus, the number of physical qubits can be written as:
\begin{align}
Q_P(k) \approx \frac{28}{199} 199^k \max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]
\label{eq:number_physical_qubits_k_concat}
\end{align}
where $i$ denotes the logical timestep on which there are $N_{L,\parallel,i}^{\text{cNOT}}$, $N_{L,\parallel,i}^{\text{1qb}}$, $N_{L,\parallel,i}^{\text{Id}}$ logical cNOT, single qubit and identity gates acting in parallel. In principle, for the same reason that consecutive gates on the $k-1$ level had to use fresh ancilla, we cannot use the same ancilla for consecutive logical gates because the ancilla preparation takes longer than the duration of the logical gate. Fortunately, as shown in the appendix \red{to write and double check}, the most pessimistic estimation of that would lead to only multiply $Q_P$ by $4$ in \eqref{eq:number_physical_qubits_k_concat}: it wouldn't change its order of magnitude such that we won't take this coefficient into account. At this point we can then consider that \eqref{eq:number_physical_qubits_k_concat} is the number of physical qubits used after $k$ concatenations.

However, to define the power at the logical level, we would like to "make appear" the number of logical qubits $Q_L$. In order to do it, we can notice that we have\footnote{It assumes that the algorithm uses the minimal number of logical qubits it conceptually need. Indeed, this equation means that the moment the maximum number of logical qubits are doing something "together" is equal to the number of logical qubits. But we could imagine inefficient implementation where this wouldn't be true.} $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}+N_{L,\parallel,i}^{\text{Meas}} \right]=Q_L$, where $N_{L,\parallel,i}^{\text{Meas}}$ is the number of logical measurement gates at the timestep $i$. The reason behind this equation can intuitively be understood from the figure \ref{fig:bottleneck_algo_physical_qubits}. We remind that $N_{L,\parallel,i}^{\text{Meas}}$ did not appear in \eqref{eq:number_physical_qubits_k_concat} because measurement gates do not require ancilla, and our estimation of the number of physical qubits was given by the number of ancilla (as they dominate). Calling $i_0$ the associated logical timestep, we deduce that an estimation for the total number of physical qubits required by the computer is, for $k>0$:
\begin{align}
Q_{P}(k) \approx \frac{28}{199} 199^k (Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx \frac{28}{199} 199^k Q_L,
\label{eq:number_physical_qubits_from_logical}
\end{align}
where $N_{L,\parallel,i_0}^{\text{Meas}}$ corresponds to the number of logical measurement gates active in parallel at this "bottleneck timestep" $i_0$. We explain why $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ in a few lines. This formula does not apply for $k=0$ as it is based on estimating the total number of physical qubits from the number of ancilla qubits. And there are no ancilla qubits when no concatenations are performed. For all practical purpose, we can comment that it will frequently be true for algorithm to have $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ (where $\approx$ means same order of magnitude). Indeed, if this equation is not true, it means that on the timestep $i_0$, the dominant number of logical gates are measurement gates. At the logical timestep right before, all those measurement gates were either logical identity, single qubit or cNOT gates. It implies that $2 N_{L,\parallel,i_0-1}^{\text{cNOT}} + N_{L,\parallel,i_0-1}^{\text{1qb}}+N_{L,\parallel,i_0-1}^{\text{Id}} > N_{L,\parallel,i_0}^{\text{Meas}}$ (this is a strict inequality because on the timestep $i_0-1$, the measurements are replaced by other logical gates, but qubits that were not measured in $i_0$ might be affected by some other logical gates). Thus, $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]>N_{L,\parallel,i_0}^{\text{Meas}}$. And as $N_{L,\parallel,i_0}^{\text{Meas}}$ was the dominant number of gates on timestep $i_0$, it shows that $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]$ gives a good estimation to $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}+N_{L,\parallel,i}^{\text{Meas}}\right]$, and thus that $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$. In what follows, we will always assume $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ as we only care about order of magnitudes estimations. We illustrate this on figure \ref{fig:bottleneck_algo_physical_qubits} b).
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/bottleneck_algo_physical_qubits}
\caption{\textbf{a)} How the number of qubits is related to the maximum number of gates acting in parallel. On this figure, we illustrate an algorithm composed of two and identity gates. We notice that the number of qubits required by the algorithm (here they appear to be logical ones) is equal to $\max[2 \overline{N}_{L,\parallel}^{\text{cNOT}} + \overline{N}_{L,\parallel}^{\text{1qb}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{Meas}}]=5$, it happens on the red rectangle (but also on the following timestep). \textbf{b)} Intuitive understanding of why we can expect that $Q_L \approx \max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}} \right]$. The red box rectangle verifies $2 \overline{N}_{L,\parallel}^{\text{cNOT}} + \overline{N}_{L,\parallel}^{\text{1qb}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{Meas}}=Q_L$ exactly. But because the measurement gates dominate on this timestep, and that they are identity, single or two qubit gates on the timestep before (we assume that a qubit will never directly be measured as it would be useless for an algorithm), the result is close to $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]=4$.}
\label{fig:bottleneck_algo_physical_qubits}
\end{center}
\end{figure}
\FloatBarrier
\subsubsection{Expression of the power}
Now, we can regroup the different thing we calculated to express the power at the logical level. On the physical level, it is a function: $P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i$ where $\mathcal{P}_{a}$ correspond to the power-active gate (that we assume here to be $\mathcal{P}_a = \{\text{1qb},\text{cNOT},\text{Meas}\}$). Thus, from \eqref{eq:average_number_physical_gate_timestep1}, \eqref{eq:average_number_physical_gate_timestep2}, \eqref{eq:average_number_physical_gate_timestep3} and \eqref{eq:number_physical_qubits_from_logical}, we have here:
\begin{align}
&P=Q_L t(k) a + \left( b^{\text{1qb}} u(k) + b^{\text{cNOT}} v(k)+ b^{\text{Meas}} w(k)\right) (N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}}) \label{eq:logical_power}\\
& t(k) \equiv \frac{28}{199} 199^k\\
& u(k) \equiv \frac{7}{48}\left(\frac{199}{3}\right)^k\\
& v(k) \equiv \frac{1}{3} \left(\frac{199}{3}\right)^k\\
& w(k) \equiv \frac{7}{48} \left(\frac{199}{3}\right)^k
\end{align}
We remind that we only focused on the transversal logical gates. An algorithm would in principle required other gates than cNOT, what we called single qubit gates here (which were Hadamard or Pauli), identity or measurement gates. Those other gates such as the $T$-gate have to be implemented with a completely different protocole which goes beyond the scope of this thesis. Taking them into account would in principle add additional terms in this power function. That being said, we see that we were able to define the power at the logical level with some adaptations. We have to keep in mind that each term involved in this equation might vary from a coefficient $\epsilon$ roughly between $1$ and $10$ as we only estimated quantities in their order of magnitudes. Now, we can remind the most important hypothesis that lead us here. For the passive costs, we only took into account the ancilla qubits because they give the dominant contribution in the total number of physical qubits. We also assumed that no recycling is being performed for the all ancilla qubits that are inside a given logical gate, and we did not take into account a factor $\approx 4$ symbolizing that at the logical level, consecutive gates might have overlapping for ancilla preparations \red{I will maybe add this $\times 4$ to remove this critic}. We also assumed that the number of physical qubits is proportional to $Q_L$. This will be true for some algorithms, and only an approximation for some others (it depends if the moment when the maximum number of logical qubits are involved at the same time corresponds to a moment some logical qubits are being measured). If this happen to not be true, this approximation should still be fair (see previous discussions). For the active costs, the main assumption that we did is to neglect the "variation" in the concatenated construction between the different kind of logical gates. It allowed us to have a number of physical gates proportional to $(N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}})$. Now, we believe that the most "critical" assumptions, the ones that would change by more than $100 \%$ some of the numbers in \eqref{eq:logical_power} are (i) the assumption that the number of physical qubits is proportional to $Q_L$, (ii) the assumptions behind the qubits recycling. The other considerations should not change our result quantitatively. 

Now, we comment the expressions we obtained. We notice here the functions $t$,$u$,$v$,$w$. They are representing the increasing power cost of the logical elements when more and more error correction is being performed (because more and more physical components are there). They are the "translation" of the energetic cost from the logical to the physical world (where the power is "really" taken in the laboratory). We notice that $u$, $v$ and $w$ are growing following the same law $(199/3)^k$ (with a different prefactor). This law comes from the recursive construction, as the 1-Ec is the same whatever the 1-Ga was, the scaling in the number of physical components will be identical for all the kind of physical gates \red{double check if that's really the reason}. But there is not exactly the same number of cNOT, single qubit gates and measurement gates inside a 1-Ec, this is what explains the different prefactors. In the section \ref{sec:formulation_problem_physical}, we said that we would neglect the active cost related to measurement. This was a fair assumption to do because physical measurements only occured on the boundary of the algorithm (and will thus have a negligible "weight" in term of parallel operation compared to all the other gates occupying the "volume" of the algorithm). Here, as we are doing quantum error correction, physical measurements are done "very frequently in time" (thus inside the "volume") to detect errors. In principle we can no longer neglect them\footnote{Actually as in practice measurement require much less active power than single qubit gate we will still be able to neglect them, but we wanted to emphasize on this difference anyway.}, this is why there is a cost per physical measurement gate represented by $b^{\text{Meas}}$ in \eqref{eq:logical_power}. We also notice that $t(k)/u(k)$, $t(k)/v(k)$ and $t(k)/w(k)$ diverge in the infinite concatenation level. This is based on our assumption that the ancilla qubits are not being recycled within a logical gate. Because of that, the passive cost will dominate in the $k \to \infty$ limit. In practice we can expect that with smart recycling scenarios, those ratios would actually converge toward some constant. We can also see that the passive costs are proportional to the total quantity $(N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}})$. It means that the exact logical gate that is being implemented in the algorithm doesn't matter, what matters is the average number of logical qubits that are actively participating on an information processing level. It also allows us to notice that in the opposite of what we saw without error correction, logical identity gates require an active power consumption. The reason is that it costs energy to protect the information: an error-protected quantum memory \textit{has} an \textit{active} energetic cost. More generally, in fault tolerant quantum computing, because error correction is being performed for any gate, all the logical gates are active in term of power consumption such that we can say $\mathcal{P}_{L,a}=\mathcal{P}_{L,n.a}$ (we remind that $\mathcal{P}_a$ and $\mathcal{P}_{n.a}$ represented the power-active and not active gates in the section \ref{sec:formulation_problem_physical}).
 
\section{Conclusion}
In this chapter, we proposed a formulation for the question of the resource cost of quantum computing. A resource is in principle any cost function, but here we used the power consumption as our resource of interest. This formulation is based on a minimization under constraint: we ask to minimize the power it costs to run an algorithm \textit{under the constraint} that the noise contained in its output, as quantified by some metric, is not higher than a given target chosen by the experimentalist. Formulating the question this way allows to optimize all the parameters the experimentalist can tune in order to reach this minimum. Then, we proposed some generic model for the expression of the power and the metric. We saw that some part of the power are associated to passive energetic cost, i.e they do not depend on what the algorithm is doing at a given instant of time while some other depends on what it is actually doing. We also saw that the algorithm, the engineering and the gate physics play well identified and separated role in this formulation.  We then applied this model in different simple examples to see how the power consumption can be minimized. It allowed us to see under which perspective energetic considerations can be considered in algorithm compilations problems, allowing us to explain what it means for an algorithm to be energy efficient. The examples we did were however to simple to really show a practical interest, which is the goal of the next chapter.

Finally, we adapted the generic model for power and metric to fault-tolerant quantum computing working with concatenated codes. The metric at the logical level is the natural generalization of the metric on the physical level. For the power consumption it is however less straightforward, and some approximations are required in order to be able to define it at the logical level. Once those approximations have been made, we were able to see important differences between the physical and logical power. For instance, because error correction is being applied, all the logical gates will at first order require the same amount of power to be implemented which is not the case on the physical level. We also saw that the ratio between active and passive cost might evolve with the level of protection.
\begin{appendices}
\end{appendices}


==> chapter4/chapter5.tex <==
\chapter{The energetic cost of quantum computing: formulation of the question}
\section{Introduction}
In this chapter, we are going to design the general method behind energetic estimation of quantum computing. This method can in principle be applied both in NISQ algorithm (with some restrictions that we will explain) and in fault tolerance. This chapter will however be dedicated to explain the general principle of the method and to provide simple examples where it can be applied. The estimations we will do behind those examples shouldn't however be taken too seriously because of the many simplified assumption we are going to do. They are just here to allow to grasp the concept in a concrete manner. We will also see what are the differences between energetic estimation for algorithm implemented with or without quantum error correction: in the end of this chapter we will adapt the approach to fault tolerance. The following chapter will consist in using this method in order to make a more realistic energetic estimation of implementing an algorithm on a fault tolerant quantum computer.
\section{Formulating the question}

\subsection{The principle}
The general purpose of an algorithm is to provide an answer to some computational task. What we care about is obviously to have the good answer to this task, there is no point in having a bad one. However, because of noise, there will always have a probability that the answer we find is not the good one. On the other hand, the probability to find a successful answer will be related to how much some resource an experimentalist is ready to invest in the calculation. Indeed, implementing successfully an algorithm (in the sense that it provides an answer having a high probability of success) has a cost. We saw examples in the previous chapter with the energy that we allowed to spend in order to create the pulses driving the qubits. When we restricted too much this energy, the algorithm had a poor success probability. Without loss of generality, we will now assume that the resource we are interested in is the \textit{power} required to implement an algorithm. We understand that there must exist a \textit{minimum} power required to implement successfully an algorithm. And we can phrase the exact question we should address in order to find it. We basically ask: "what is the minimum power I have to spend under the constraint that the algorithm I am implementing provides the good answer to the task with a probability higher or equal to some target I want.". The answer to this somewhat lengthy question is the only thing that really matters in order to be power efficient. We can phrase it in a mathematical manner as the following problem of optimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | p_{\text{success}}(\bm{\delta}) \geq p_{\text{target}}},
\label{eq:ideal_solve}
\end{align}
where $P$ is the power, $p_{\text{target}}$ is the success probability we aim for, and $p_{\text{success}}$ is the actual probability of success of the algorithm. We see that we introduced the family of parameters $\bm{\delta}$ (the fact it is a family is represented by the bold notation associated to vectors). They represent the \textit{tunable} parameters that the experimentalist can vary in order to reach the minimum. A typical example would be the qubit temperature $T_{\text{Q}}$: changing it would at the same time modify the power it costs to perform the computation (the electrical power for the cryogenic typically depends on $T_{\text{Q}}$), but the success probability as well (a too high temperature would induce a poor quality in the answer). Thus, in general, both the probability of success and the power depend on the family $\bm{\delta}$\footnote{Of course it is possible that one parameter in the family of parameters $\bm{\delta}$ only affect the success and not the power cost, and reciprocally.}. This minimization under constraint provides an equation that relates the resource one should spend with the probability of success of the algorithm. We also see that not only the minimum power can be found performing this minimization, but the optimum set of parameters allowing to reach this minimum, $\bm{\delta}_{\text{opt}}$ will also be found.

Unfortunately, directly solving this problem is too complicated in general. Indeed it is usually not possible to directly find the function $p_{\text{success}}(\bm{\delta})$ as it would usually require to know the density matrix at the end of the algorithm. If this is a requirement the method would have no interest because it would mean that the circuit can be efficiently simulated classically\footnote{As the goal is to implement an algorithm on a quantum computer, this algorithm must present advantages compared to a classical simulation.}. For this reason, we will take a slightly different approach. We will not try to estimate the success probability of the algorithm, but we will try to estimate, or at least to bound the "quantity of noise" there is in the final density matrix of the algorithm (right before the measurements). This approach is slightly different because there is a unique way to define the success probability of the algorithm while there are different ways to evaluate the quantity of noise inside a density matrix (we could think about the trace distance or the fidelity with respect to the ideal state for instance). The reason to do this strategy is that it is an easier quantity to estimate, or more usually, \textit{to bound}, than the probability of success of the algorithm\footnote{Also, the different ways to quantify the noise are usually related: knowing the value of one often allows to give a bound the other.}. To give specific examples, the worst-case fidelity of an algorithm can easily be bounded by the knowledge of the worst-case fidelity of each individual gates composing it. And from this knowledge, we can then bound, or have a rough estimation of the probability of success of the algorithm (which is much more complicated to directly access theoretically). This is another important requirement we should have in the way we measure the quantity of noise: there is no point in being able to estimate the quantity of noise in the final density matrix if it doesn't give any information about the probability to have the good answer. All those requirements will give us constraints on what are the good or the bad tools that can be used to measure the quantity of noise in the final density matrix of algorithms. We call them "metrics" and write them with the letter $\mathcal{M}$ in what follows. Putting aside those issues for now on, the problem of power estimation can in the end be formulate by the following minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{\bm{\delta}}(P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{\text{target}}}.
\end{align}
This equation means that we want to find the minimum power under the constraint that the quantity of noise (as quantified by the metric $\mathcal{M}$) is lower than some targetted quantity of noise $\mathcal{M}_{\text{target}}$ considered as acceptable by the experimentalist. The value of the metric $\mathcal{M}$ depends on the family of tunable parameters $\bm{\delta}$ for the exact same reason as $p_{\text{success}}$ in \eqref{eq:ideal_solve} also depended on those.
\subsection{General properties}
\subsubsection{The minimum power increases with the targetted accuracy}
Let's assume that there exist a parameter $\delta_j$ in the list of parameters  $\bm{\delta}$ such that, when we increase it, the power decreases while the quantity of noise increase. Mathematically it means that:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
One example of such parameter will often be the temperature of the qubits. If we increase the qubit temperature, the power it costs to maintain them cool will typically decrease, but the quantity of noise will usually increase because they will be submitted to more thermal noise. We will see it in a concrete manner in the parts where we will take physical examples: the hypothesis that such parameter $\delta_j$ exists will typically be true in relevant physical systems. From now on, we will assume it is the case.

This hypothesis will imply the following two properties. First, (i) the minimum power required such that the quantity of noise of the algorithm is equal \textit{or lower} to $\mathcal{M}_{\text{target}}$ is the same as the minimum power required such that the quantity of noise is \textit{equal} to $\mathcal{M}_{\text{target}}$, i.e the following equality is true:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}}
\end{align}
Let us do a proof by contradiction of this fact. We assume that the minimum power is found when $\mathcal{M} < \mathcal{M}_{\text{target}}$. As $\partial_{\delta_j} \mathcal{M}>0$, we can increase $\delta_j$ for some range without violating the condition $\mathcal{M} \leq \mathcal{M}_{\text{target}}$. Doing so, we will also decrease the power as $\partial_{\delta_j} P<0$. Thus, as soon as $\mathcal{M}<\mathcal{M}_{\text{target}}$ we do not minimize the power consumption: the minimum is necessarily reached for $\mathcal{M}=\mathcal{M}_{\text{target}}$. In the same line of thoughts, we can also prove that (ii) $P_{\min}$ is a \textit{strictly decreasing} function of $\mathcal{M}_{\text{target}}$. To show this, let us consider two targets such that $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$. Then, as:
\begin{align}
\min(P)_{\big | \mathcal{M} \leq \mathcal{M}^2_{\text{target}}}=\min(P)_{\big | \mathcal{M} = \mathcal{M}^2_{\text{target}}},
\end{align}
the minimum power obtained for $\mathcal{M}<\mathcal{M}^2_{\text{target}}$ is necessarily bigger or equal to the one obtained for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Because of that, as $\mathcal{M}^1_{\text{target}}<\mathcal{M}^2_{\text{target}}$, we deduce that: $P_{\min}(\mathcal{M}^1_{\text{target}}) \geq P_{\min}(\mathcal{M}^2_{\text{target}})$. It remains to show that they cannot be equal. We also do a proof by contradiction. Let us consider a set of parameters $\bm{\delta}$ such that: $P(\bm{\delta})=P_{\min}(\mathcal{M}^1_{\text{target}})$, and $\mathcal{M}(\bm{\delta})=\mathcal{M}^1_{\text{target}}$\footnote{We say "a" set of parameters and not "the" set of parameters as the minimum power consumption could be in principle reached for many different values of $\bm{\delta}$.}. If we increase $\delta_j$ until the moment $\mathcal{M}=\mathcal{M}^2_{\text{target}}$, as $\partial_{\delta_j} P < 0$, it has for effect to \textit{strictly} decrease the power consumption while ensuring $\mathcal{M}=\mathcal{M}^2_{\text{target}}$. Thus, the minimum power reached for $\mathcal{M}=\mathcal{M}^2_{\text{target}}$ is necessarily \textit{strictly} lower than the one reached for $\mathcal{M}=\mathcal{M}^1_{\text{target}}$.

In summary, here we proved the following property that we will frequently use.
\begin{property}{Behavior of the minimum power}

\label{prop:behavior_min_power}
If there exists at least one parameter $\delta_j$ in the family of parameters $\bm{\delta}$ on which:
\begin{align}
&\partial_{\delta_j} P<0\\
&\partial_{\delta_j} \mathcal{M}>0
\end{align}
Then, we have:
\begin{align}
P_{\min} \equiv \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) \leq \mathcal{M}_{target}} = \min (P(\bm{\delta}))_{\big | \mathcal{M}(\bm{\delta}) = \mathcal{M}_{target}},
\end{align}
which means that the minimum power consumption is found when we ask for an accuracy that it is exactly equal to what we target: asking for a better accuracy is necessarily more costly. We also have that
$P_{\min}$ is a strictly decreasing function of $\mathcal{M}_{\text{target}}$ (for the same reason).
\end{property}
This property establish properly the intrinsic connection between noise and power: asking for a better accuracy has an energetic cost. But again this connection is true because of the hypothesis we made on the behavior of power and metric with respect to the parameter $\delta_j$ (which will frequently be true in physical systems).
\subsubsection{Equivalence between minimum power for a targetted accuracy and maximum accuracy for a given power}
\label{sec:equivalence_minpow_maxacc}
Now, we can show that asking to minimize the power in order to reach a given accuracy is in some sense, equivalent to asking to find the best accuracy the computer can get to for a given (i.e fixed) amount of power available. This property is true as soon as $P_{\min}$ is a decreasing function of $\mathcal{M}_{\text{target}}$ (which will usually be the case as explained before).

Those two questions are equivalent in the sense of what is represented on figure \ref{fig:equivalence_minpow_maxacc}. On this curve is represented the minimum power required to implement the algorithm as a function of the maximum quantity of noise acceptable in its answer: $\mathcal{M}_{\text{target}}$. In this case, this graph can be read in two directions. Indeed, if we invert the meaning of the axis, i.e we interpret it as a curve representing a value of some quantity of noise as a function of some injected power, we can also interpret it as the \textit{minimum} quantity of noise it is possible to reach as a function of this injected power. More precisely, let us consider any couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. By definition of $P_{\min}$, if someone wants to have an accuracy $\mathcal{M}^0_{\text{target}}$, the minimum power required will be $P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. But reciprocally, if this person has a given amount of power $P^0$ available, the minimum quantity of noise it can get to (thus maximum accuracy) is $\mathcal{M}^0_{\text{target}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.5\textwidth]{chapter4/images/equivalence_minpow_maxacc}
\caption{The minimum power necessary as a function of the maximum quantity of noise acceptable targetted, $\mathcal{M}_{\text{target}}$ is represented. Because this function is monotonous, the curve can also be interpreted as the lowest quantity of noise acceptable for a given amount of power available as explained in the main text.}
\label{fig:equivalence_minpow_maxacc}
\end{center}
\end{figure}
\FloatBarrier

In order to show it, we consider again the couple $(\mathcal{M}^0_{\text{target}},P^0 \equiv P_{\min}(\mathcal{M}^0_{\text{target}}))$. We now ask: what is the maximum accuracy, i.e the lowest quantity of noise $\mathcal{M}$ the computer can get to if it has at its disposal the power $P^0$. Necessarily, it can be \textit{at least} as accurate as $\mathcal{M}^0_{\text{target}}$: $\mathcal{M}$ must verify $\mathcal{M} \leq \mathcal{M}^0_{\text{target}}$. Indeed $\mathcal{M}^0_{\text{target}}$ is an explicit example of target reachable for an injected power $P^0$. Now it remains to prove that the strict inequality is not possible: no better accuracy is reachable for this amount of power. This can be shown using again a proof by contradiction: let's assume that we find that the best accuracy it is possible to reach for an injected power $P^0$ verifies $\mathcal{M} < \mathcal{M}^0_{\text{target}}$. We assume that this power is reached for the family of parameters $\bm{\delta}=\bm{\delta}_0$. We necessarily have $P^0=P(\bm{\delta}_0) \geq P_{\min}(\mathcal{M})$: indeed $P^0$ amount of power would be used to have an accuracy $\mathcal{M}$, but it might be possible to use less power to reach that accuracy. As on the other hand $P_0=P_{\min}(\mathcal{M}^0_{\text{target}})$, we deduce that $P_{\min}(\mathcal{M}^0_{\text{target}})\geq P_{\min}(\mathcal{M})$. Now, this result is absurd. Indeed, as $\mathcal{M}<\mathcal{M}^0_{\text{target}}$, and as $P_{\min}$ \textit{strictly} decreases as a function of $\mathcal{M}$, necessarily $P_{\min}(\mathcal{M}^0_{\text{target}}) < P_{\min}(\mathcal{M})$. 

All this shows that the curve can be read in two directions: \textit{there is an equivalence between asking to minimize the noise for a given amount of power available, and asking to minimize the power in order to target a given quantity of noise.}
\subsection{An introductive example}
\subsubsection{Description of the problem}
\label{sec:single_qubit_example}
Let us illustrate the concepts with a very simple example: we wish to minimize the power to spend in order to implement a $\pi$-pulse on a qubit. For this, we need to specify: (i) the noise model describing the physics, (ii) the way we quantify this noise, i.e which metric we are going to choose, (iii) the expression of the power we want to minimize and (iv) the list of parameters we would like to optimize in order to minimize this power.

We start to specify (i). Here, we assume that the only reason why the qubits are noisy is because of thermal noise. The noisy evolution can be modeled as:
\begin{align}
&\frac{\partial \rho}{\partial t}=\frac{1}{i \hbar}[H,\rho]+\gamma_{\text{sp}} \overline{n}_{\text{tot}} D[\sigma^{\dagger}](\rho) + \gamma_{\text{sp}}(\overline{n}_{\text{tot}}+1) D[\sigma](\rho) \label{eq:evolution_noisy_gate}\\
&D[\sigma](\rho) \equiv \left(\sigma \rho \sigma-\frac{1}{2}(\sigma^{\dagger} \sigma \rho + \rho \sigma^{\dagger} \sigma) \right),
\end{align}
%where $H$ is the Hamiltonian implementing the gate, $\overline{n}_{\text{tot}}$ represents the noise photon occupation, i.e the number of photons in the power spectral density of noise \red{to double check the vocabulary is the good one}, and $\gamma_{\text{sp}}$ is the qubit-waveguide coupling\footnote{We remind that its inverse gives the typical qubit lifetime at $0$ temperature.}. As explained in the chapter dedicated to fault tolerance, it is always possible to "decouple" the effect of the noise from the perfect implementation of the gate such that everything will behave \textit{as if} the perfect implementation of the gate occured first, then followed by some noise. If the quantum channel $\mathcal{U}$ represents the ideal (unitary) implementation of the gate, and $\mathcal{E}$ represents the noisy implementation (thus following the equation \eqref{eq:evolution_noisy_gate} integrated for the duration of the gate), we can always define $\mathcal{N}$ such that $\mathcal{E}=\mathcal{N} \circ \mathcal{U}$. With this definition, $\mathcal{N}$ represents the effect of the noise "alone" that is acting "after" the perfect implementation of the gate. Conceptually we could proceed this way here, but in order to anticipate the section dedicated to fault tolerance, we will adopt a slightly simpler way to model the noise. We will approximate this noise map $\mathcal{N}$ by considering that it can be estimated by integrating  \eqref{eq:evolution_noisy_gate} with $H=0$, for a duration equal to the gate duration. When we say that $\mathcal{N}$ is obtained by integrating this equation, it means that we consider a basis of initial states for the qubit from which we can deduce the mathematical expression of $\mathcal{N}$. This is an approximation because we can expect this result to be different than the computation of the exact evolution $\mathcal{E}$, and then defining $\mathcal{N}= \mathcal{U}^{-1} \circ \mathcal{E}$. However,  this simplification will not change in a quantitative manner our estimation of the quantity of noise introduced by such evolution \footnote{This is actually something that we checked: for a $\pi$-pulsife the expressions of the worst case and average fidelity of the "precise" or "approximated" approach are very similar.}. In the end, the map $\mathcal{N}$ is then accessible which defines our noise model. It will be a function of $\overline{n}_{\text{tot}}$, $\gamma_{\text{sp}}$ and $\tau$ the gate duration. 

Now, we specify (ii). In order to quantify the quantity of noise in the final density matrix, we will use either the worst-case or average infidelity of this channel. We call infidelity the quantity $1-F$ where $F$ is the fidelity. We find:
\begin{align}
\mathcal{M}=(X+Y \overline{n}_{\text{tot}}) \gamma_{\text{sp}} \tau,
\end{align}
where $(X_{\text{worst}},Y_{\text{worst}})=(1,1)$ and $(X_{\text{avg}},Y_{\text{avg}})=(1/3,2/3)$ for worst-case infidelity and average one respectively. The metrics are then defined. But we cannot be satisfied of those expressions because we don't know what $\overline{n}_{\text{tot}}$ is equal to, we need to explain it. 

In the case the qubit is at the temperature $T_{\text{Q}}$, and \textit{if the signals are generated at this same temperature}, we would simply have: $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}}) \equiv 1/(e^{\beta_{\text{Q}} \hbar \omega_0}-1)$, with $\beta_{\text{Q}}=1/(k_b T_{\text{Q}})$, and $\omega_0/2 \pi$ is the qubit frequency (typically around $6$ GHz). $\overline{n}_{\text{BE}}$ is the Bose Einstein population for bosons of frequency $\omega_0/2 \pi$, at temperature $T_{\text{Q}}$ \cite{cohen1998mecanique}. But if the signals are generated at a temperature $T_{\text{Gen}}$, then the thermal noise at this temperature would affect the qubit evolution. This is why attenuators are typically put on the driving lines. Their role is to remove the noise (and in particular the thermal noise) coming from the higher temperature stages. An attenuator is composed of resistive elements that will dissipate into heat any signal injected at its input as shown on figure \ref{fig:attenuator_principle}. If $P_{\text{in}}$ is the input power before the attenuator, and $P_{\text{out}}$ the power at its output, we define the attenuation ratio by $A \equiv P_{\text{out}}/P_{\text{in}}$. It is possible to show \cite{pozar2011microwave} that for signals generated at $T_{\text{Gen}}$, an attenuator put at the temperature $T_{\text{Q}}$ will generate an amount of noisy photons $\overline{n}_{\text{tot}}$ being equal to:
\begin{align}
\overline{n}_{\text{tot}}(T_{\text{Q}},T_{\text{Gen}},A)=\frac{A-1}{A} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A} \stackrel{A \gg 1}{\approx} \overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(T_{\text{Gen}})}{A}
\end{align}
Let us first comment the formula in the $A \gg 1$ regime. It means that the quantity of noisy photons felt by the qubits will be equal to the number of noisy photons at the attenuator temperature, on which we add the noisy photons coming from the higher temperature stage, but attenuated by a factor $A$. The noise is basically attenuated in the same way than the signals sent. For an infinite attenuation, the qubits will be entirely isolated from any thermal noise coming from higher temperature stages. However this cannot be the exact expression. For instance for $T_{\text{Q}}=T_{\text{Gen}}$ (if everything is thermalized at $T_{\text{Q}}$), we would not find $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})$ with the approximated expression. This is the reason why the exact expression is actually the one of the left: it correctly describes the situation when $T_{\text{Q}}=T_{\text{Gen}}$ and $A=1$ (no attenuation: everything behave as if the qubits where thermalized at $T_{\text{Gen}}$). Of course this formula should be thought as a first order description \red{to check} of the physics (what we said is not a proof that this expression is the correct one), but it is what is used to describe the propagation of noise in microwave circuits \cite{pozar2011microwave}. Physically we can understand the situation as follows: the signal generation stage can be thought as some cavity which is thermalized at $T_{\text{Gen}}$. This cavity thus emits a blackbody radiation in a one-dimensional waveguide: it is the thermal noise. Then this noise propagates in a ballistic manner in the waveguide (as a waveguide will by construction be a good conductor for microwave frequencies, the noise won't be attenuated there). This noise is then dissipated inside of the attenuator and "converted" into phonons: this is a kind of heat that can be evacuated by the cryogenics. But the attenuator, being thermalized at $T_{\text{Q}}$, also generates thermal noise that will interact with the qubits. It corresponds to $\overline{n}_{\text{BE}}(T_{\text{Q}})$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/attenuator_principle}
\caption{Principle behind the attenuation. The signals are generated at a temperature $T_{\text{Gen}}$. Thus, in addition to the signals there is noise at this temperature that is propagating inside of the waveguide as represented by the noisy blue gaussian. The qubit is preceeded by an attenuator at the temperature $T_{\text{Q}}$. The attenuator will dissipate the noise before it reaches the qubit, but it dissipates the signal in the same manner. It is the fact that the heat $\dot{Q}_{\text{Att}}$ has to be evacuated by a cryogenic unit that makes the gate energetically costly (as shown by \eqref{eq:power_single_qubit_gate}).}
\label{fig:attenuator_principle}
\end{center}
\end{figure}
\FloatBarrier
Now, in practice the effect of the thermal noise coming from the higher temperature stages will be reduced by the following strategy. First, the signal that must arrive on the qubit has a well defined value: we must have $P_{\text{out}}=P_g$, where as explained in the fist chapter of this thesis \red{put a ref} $P_g=\hbar \omega_0 \Omega^2/(4 \gamma_{\text{sp}})$ with $\Omega=\theta/\tau$. Here $\theta$ represents the angle of rotation desired for the single qubit operation ($\theta=\pi$ for us in this section). Then, the attenuation $A$ is usually chosen in such a way that $\overline{n}_{\text{BE}}(T_{\text{Gen}})/A < \overline{n}_{\text{BE}}(T_{\text{Q}})$: the noise coming from the higher temperature stage does not dominate the physics. From the knowledge of $A$ the experimentalist deduce what is the power the generated signals should have. The general philosophy is to generate signals of high enough amplitude such that after attenuation there is a high signal over noise ratio while having a signal of appropriate power for the physics of the quantum gate. At this point, we can say that the metrics we expressed are now "well defined" because we know what $\overline{n}_{\text{tot}}$ is equal to as a function of the characteristics of the problem.

Now, we need to give the expression of the power (point (iii)). Here, we will be interested in the electrical power that we need in order to remove the heat dissipated inside of the attenuators. We will assume that our cryogenic unit has a Carnot efficiency. The heat dissipated per unit time is simply equal to $P_{\text{in}}-P_{\text{out}}$\footnote{We implicitely neglect the heat that will be dissipated when the signals will "go back", i.e after reflection on the qubit. Indeed, the power that would be dissipated by this reflection will be lower than $(A-1) P_g$ and we will neglect it. This approximation is even more true in the regime $A \gg 1$ on which we are focusing.}, the low temperature stage on which the heat has to be evacuated has a temperature $T_{\text{Q}}$, and the high temperature stage is basically the laboratory at temperature $300K$. Assuming that $A \gg 1$ (if it is not the case the evolution would be way too noisy), we get:
\begin{align}
P(T_{\text{Q}},A)=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A P_g
\label{eq:power_single_qubit_gate}
\end{align}
%All that being said, we will consider that $T_{\text{Gen}}=300K$ here (the signals are generated outside of the cryogenics, in the laboratory), and we will consider that the parameters we are going to optimize will be $T_{\text{Q}}$ and $A$. The point (iii) is now specified and the last thing to do is to provide the expression of the power.
Finally, for our last point (iv), we specify the variables we want to optimize. It will be $\bm{\delta}=(T_{\text{Q}},A)$ in this first example as we will assume that $T_{\text{Gen}}=300K$ (the signals are generated outside of the cryogenics here). In the end, the problem is well defined, and we can solve the minimization under constraint:
\begin{align}
P_{\min} \equiv \min_{(T_{\text{Q}},A)} P(T_{\text{Q}},A)_{\big | \mathcal{M}(T_{\text{Q}},A) = \mathcal{M}_{\text{target}}}
\end{align}
\subsubsection{The competition between noise and power}
We first illustrate on figure \ref{fig:competition_power_noise} in a concrete manner the intrinsic competition there is between asking for a low noise and a low power consumption. The parameters we chose for the gate are $\gamma_{\text{sp}}=1kHz$, $\tau=25 ns$ (and $\theta=\pi$: we do a $\pi$-pulse). In the rest of this thesis we will also use the decibel: "dB" unit to represent the attenuation. This unit is related to the attenuation in "natural unit", i.e when $A=P_{\text{in}}/P_{\text{out}}$ as:
\begin{align}
A_{\text{dB}}=10 \log_{10}(A)
\end{align}
For instance, a signal being attenuated of a factor $10$ will correspond to $10 \text{dB}$. A signal attenuated of a factor $10^5$ will correspond to $50 \text{dB}$. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/competition_power_noise}
\caption{Unoptimized power consumption as a function of the attenuation and the qubit temperature (color-plot). The cyan and white lines represent the iso-infidelity for respectively the average and worst case infidelity.}
\label{fig:competition_power_noise}
\end{center}
\end{figure}
\FloatBarrier
On this graph, we see that putting a high attenuation and a low qubit temperature induces a high power consumption. Reciprocally a high qubit temperature and a low attenuation leads to a small power consumption. We can also see that the regions of high power consumption correspond to regions of low noise, and regions of lower power consumption correspond to regions where the noise is high. Indeed the iso-metric lines have lower values in the bottom right part of this graph which corresponds to region of high power consumption (and higher values in the upper left part of this graph where the power is low). It illustrates the intrinsic opposite behavior between noise and power.

Let us now focus on a given iso-metric line: we wish to implement the single qubit gate in order to reach a targetted accuracy. The power consumption on those lines can drastically vary. For instance, the white iso worst-case infidelity which is at the bottom right of this graph is associated to power varying in the range (approximately) $[10^{-3},10^{-1}]$. It illustrates that choosing wisely $T_{\text{Q}}$ and $A$ is a key asset to potentially make important energetic saves: there are many possible ways to reach a given accuracy, and each of those choice can be associated to a drastically different power consumption. Of course this example is very simple as we only modeled the heat dissipated in the attenuators, but we see that it can potentially lead to quantitative saves in power consumption, and we can naturally expect that it would remain true for more complicated models\footnote{In particular because more tunable parameters will be involved, the optimum choice of parameters allowing to minimize the power consumption might be not trivial for more complicated models.}.
\subsubsection{Minimizing the power consumption}
Now, we can minimize the power consumption in order to reach a given target. This is shown on figure \ref{fig:min_power_fct_metric_1qb}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.8\textwidth]{chapter4/images/min_power_fct_metric_1qb}
\caption{Minimum power consumption as a function of the metric target. Inset: optimum qubit temperature $T_{\text{Q}}^{\text{opt}}$ allowing to reach this minimum. Blue points: worst-case fidelity, orange: average. The black line is a guide for the eye. As explained in \ref{sec:equivalence_minpow_maxacc}, this curve can also be interpreted as the minimum metric target it is possible to reach as a function of the injected power.}
\label{fig:min_power_fct_metric_1qb}
\end{center}
\end{figure}
\FloatBarrier
We see on that graph that the minimum power is a stricly decreasing function of $\mathcal{M}_{\text{target}}$ (whatever the metric we choose: worst-case or average infidelity). This is an illustration of the property \ref{prop:behavior_min_power}. Indeed in the case we study when $T_{\text{Q}}$ increases, the power decreases while the metric increases\footnote{As a side remark, in this case we would have the same kind of behavior for $1/A$: increasing it (thus reducing the attenuation) lower the power but increases the amount of noise}. We also see from the inset \textit{how} the power consumption is being decreased for a higher target: the temperature of the qubits increases. We did not represent it here but we would also see that the optimum attenuation would decrease as a function of $\mathcal{M}_{\text{target}}$. As explained in \ref{sec:equivalence_minpow_maxacc}, we can also switch the interpretation of this curve and realize that it also represents the maximum accuracy (i.e minimum value of $\mathcal{M}_{\text{target}}$) it is possible to reach as a function of some injected power. Finally, this graph also illustrates that the minimum power required depend on the metric that is used. The worst-case fidelity as being "more demanding" will ask for a bigger power consumption to reach a given target in contrary to the average fidelity. To make a connection with the previous section, the minimum power obtained for $\mathcal{M}_{\text{target}}=10^{-4}$ for the average infidelity (it is about $2.10^{-6}$) corresponds to the minimum power we would find along the upper left cyan iso-metric line in figure \ref{fig:min_power_fct_metric_1qb}.
\section{Hardware-software "full-stack" optimization}
\subsection{General framework}
At this point, we have shown how parameters describing the "hardware" part of the computer can in principle be optimized given the competition between noise and power ($A$ and $T_{\text{Q}}$ were the variables playing this role). But our example was about a single qubit gate which is not very interesting in practice: the goal of a computer is to run algorithms composed of many gates. In this section we will explain the general approaches we can choose in order to minimize the power consumption of a quantum computer running algorithms. We will naturally generalize the optimization by including in it the "software" part of the problem, i.e the characteristics of the implemented algorithm. It will play a role for two aspects: it will allow us to find which characteristics of the algorithms play an important role in order to estimate the power consumption, but it will also allow us to \textit{optimize} the way the algorithm is compiled in order to minimize the consumption (at least in principle). Finally, we will provide a simple, yet quite general model for the power function $P(\bm{\delta})$ and noise estimation $\mathcal{M}(\bm{\delta})$. We will use a number of assumption in this part, mainly for pedagogic purpose (and also because they are enough for the work that has been done), but generalizations to more general models would often be straightforward. Finally, we will express everything here in term of \textit{physical} qubits and gates which is why all the quantities introduced will have an index $P$. This is in order to anticipate the fault tolerant adaptation of this framework that will be done later in this chapter. It will change some quantitative aspects but the overall philosophy would remain identical as we will see.
\subsubsection{A general model for metric and power}
\label{sec:formulation_problem_physical}
To begin with, let us try to have some general expression of the power regardless of any optimization (i.e we focus on determining a generic expression for the function $P(\bm{\delta})$ without trying to minimize it based on the metric target). The first thing to acknowledge is that there might have a constant energetic cost regardless of what the computer is doing, i.e if it is running an algorithm or not. We call it the \textit{passive} energetic cost. One typical example of that is the heat conduction: all the cables necessary to control the qubits will always be inside of the computer, and they will bring heat that will have to be evacuated\footnote{We will see other examples of passive cost outside from heat conduction later on.} which costs electrical power for the cryogenic. Here, we will assume that the passive costs scale proportionnally with the number of (physical) qubits $Q_P$ inside the computer but we have to keep in mind that other scaling laws could be involved\footnote{For instance, in an architecture in which the qubits are implemented on a 2D grid, and for which single qubit gate can be done by sending signal in the appropriate (line,column) coordinate, the power would contain a term proportional to $\sqrt{Q_P}$. But even in this case additional terms proportional to $Q_P$ could be expected.}. A scaling proportional to $Q_P$ comes from the fact that the number of cables and amplifiers (amplifier cannot be shutdown when not used, thus they are within the passive costs) is usually increasing proportionally to the \textit{total} number of qubits inside the computer. But in addition to passive costs, there are also the \textit{active} costs. They will increase the power consumption in a manner that is time dependent. The best example of that is the power associated to signals that are being sent to the qubits: they only have to be sent if an algorithm is running and this power might also vary in time within an algorithm\footnote{One concrete example is the power required to remove the heat dissipated into the attenuators: this heat will have to be evacuated only if a gate is acting on the qubits.}. Such power will usually correspond to the moment non trivial gates (i.e not the identity operation) are being applied.\footnote{We should emphasize that it is not always the case. Indeed, there exist schemes in which applying an identity operation on qubits has an energetic cost as it requires to send pulses to \textit{keep} a coupling constant to zero (otherwise the qubit might interact in an undesired manner with the other qubits) \red{cite}.} Here, we will assume that no power is required to implement identity gates, and that some other gates might require a negligible amount of power. We also consider that the algorithm is implemented with a \textit{primitive} gateset (any gate can be expressed as a combination of gates in this gateset). The gates requiring power within this gateset will enter in a family $\mathcal{P}_{a}$ (for power "active" gates), otherwise they will enter in the family $\mathcal{P}_{n.a}$ (for power "non-active" gates). Under those assumptions, the power consumption can thus be written as the following function:
\begin{align}
P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i,
\label{eq:physical_power_gen}
\end{align}
only the family $\mathcal{P}_{a}$ has to be considered for the active power consumption. Here, $a$ represent the power it costs \textit{per qubit} to run the computer. The family of coefficients $\{b^i\}$ represent the power it costs \textit{per active (physical) gate of type "$i$"}(the type of gate corresponds to the precise gate that is being implement: cNOT, Pauli etc) to implement it. The terms $N^{(i)}_{P,\parallel}$ is the number of gate of type $i$ that are activated at a given instant in the algorithm. This quantity in principle \textit{depends} on time (because it is an \textit{active} cost), but from now on, we will assume that we are only interested in the \textit{average} power consumption such that $N^{(i)}_{P,\parallel}$ should be understood as an \textit{average} number of gates activated in parallel.

%, and that all the different gates require the same amount of power \textit{per qubit} involved their dynamic in order to be activated. It means that the active cost will be proportional to the number of physical qubits \textit{actively} participating in the calculation in term of power consumption: $Q_P^{P^a_P} \equiv N_{P,\parallel}^{1qb}+2N_{P,\parallel}^{2qb}$, where $N_{P,\parallel}^{1qb}$ and $N_{P,\parallel}^{2qb}$ respectively represent the average number of single (excluding identity) and two qubit gates acting in parallel inside of the computer\footnote{We assume that all the primitive gates used in the algorithm are either single or two qubit.}. There is no reason to assume that different gates "consume" the same amount of power. But it could be reasonable in some case: the energetic cost to perform a quantum gate is not necessarily only due to the gate physics: it can also be related to the way the signals are generated. If the electronic generating the signals can be turned off when no gates are activated, and if it dominates the details of the gate physics, our assumption would be safe for instance. But as many of the hypothesis we are doing here, it is not strictly necessary, it will just allow us to get a simple and intuitive model on which we will make physical comments. Also, we will only be interested in "order of magnitude" estimations of the energetic cost which makes our hypothesis more legitimate. With those assumptions we deduce, for some coefficients $a$ and $b$: $P=Q_P a + Q_P^{P^a_P} b$. It is usefull to rewrite this expression by introducing the notion of \textit{power-activity} of the qubits. It is defined as
%\begin{align}
%P^a_P \equiv \frac{Q_P^{P^a_P}}{Q_P}
%\end{align} 
%and it physically represents the fraction of qubits that are actively participating in the power function over the total number of qubits (we remind that we reason with average values along the algorithm here). Using this quantity the power then becomes:
%\begin{align}
%P=Q_P (a + P^a_P b).
%\end{align}
%We will make use of that notion in a few paragraphs.

We talked about the expression of the power. Now we must discuss the quantity of noise introduced by the algorithm. In the previous sections we explained why we need a metric to quantify the noise (because it is easier to access than the probability of success of the algorithm), and we gave some conditions it must satisfy (it should have a nice interpretation in such a way that the success probability can be estimated or bounded by this quantity). One requirement that we can ask for the metric to make it suitable for theoretical calculations is that from its value on each individual gates we can bound it for the entire algorithm. It assumes that the effect of the noise is local: it is possible to define a quantum channel for each quantum gate\footnote{Which means in particular that the final quantum state of a given quantum gate can be deduced by the sole knowledge of the state it had at its input.}, and from that to find how much noise a given gate introduces. A typical property allowing it is to ask that:
\begin{align}
\mathcal{M}_P^{\text{exact}} \leq \mathcal{M}_P^{\text{bound}} \equiv \sum_i \mathcal{M}^{(i)}_{P},
\label{eq:sub_additivity}
\end{align}
where $\mathcal{M}_P^{\text{exact}}$ is the \textit{exact} quantity of noise introduced by the algorithm, $\mathcal{M}^{(i)}_{P}$ is an estimation of the quantity of noise introduced by each (physical) quantum gate. The way we will quantify the noise occurring in the algorithm will be based on the best estimation we can have of $\mathcal{M}_P^{\text{exact}}$: $\mathcal{M}_P^{\text{bound}}$. Of course the tighter the bound is to the exact value the better it would be. Then, our metric will be defined as $\mathcal{M}_P=\mathcal{M}^{\text{bound}}_P$ and will verify:
\begin{align}
\mathcal{M}_P=\sum_i N_P^{(i)} \mathcal{M}^{(i)}_{P}.
\end{align}
This property of bounding the quantity of noise is pretty standard to ask, see for instance \cite{gilchrist2005distance}. 
Now, we assume that we can define a clock speed for the algorithm. It means that the algorithm will be implemented in a finite sequence of primitive timesteps all of duration $\tau_P^{\text{timestep}}$. In all of those steps a \textit{unique} primitive gate will be implemented per qubit (or per two qubit if the gate is a two qubit one). The assumption that there is a clock speed is not equivalent to say that the duration to implement all the gates are the same. It just means that if a primitive gate happens to be faster than the timestep, the qubit will then follow an identity evolution until the end of the timestep: $\tau_P^{\text{timestep}}$ thus corresponds to the longest gate in the primitive gateset. Now, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth. This is because we will neglect the final measurements in order to simplify our discussions. Indeed they will have a negligible contribution to the power consumption because they are acting "at the boundary" of the algorithm: their contribution in term of active power consumption or noise will be low compared to all the other gates. It doesn't mean that we will not take into account the cost of measurement amplification: this is usually a \textit{passive} cost that we are going to model (but this will come in the next chapter). Using the depth, we have $N_P^{(i)}=D_P N_{P,\parallel}^{(i)}$, and we can then write:
\begin{align}
\mathcal{M}_P=D_P \left(\sum_{i \in \mathcal{P}_a} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P}+\sum_{i \in \mathcal{P}_{n.a}} N_{P,\parallel}^{(i)} \mathcal{M}^{(i)}_{P} \right)
\label{eq:physical_metric_gen}
\end{align}
We notice from this expression that \textit{any} gate occuring in the algorithm might introduce noise. There is thus a difference between being active in term of power consumption and being active in term of information processing. For instance, an identity gate will not require any power consumption but it will introduce nonetheless noise in the computation.
%where $N_P^{(i)}$ is the number of the $i$'th (physical) gate type used in the algorithm and $\mathcal{M}^{(i)}_{P}$ the quantity of noise introduced by this gate. Assuming that all the gates bring an amount of noise proportional to the number of qubit they involve, we have:
%\begin{align}
%\mathcal{M}_P=(N^{\text{1qb}}_{P}+N^{\text{Id}}_{P}+N^{\text{2qb}}_{P}) \mathcal{M}^{(0)}_P,
%\end{align}
%where $N_{P}$ represents the total number of physical gates in the algorithm, and $\mathcal{M}^{(0)}_P$ the metric of each of those gates. In a similar way as what we did for the power, we can also introduce the notion of \textit{information-activity} of the qubits. We define it as:
%\begin{align}
%I^a_P \equiv \frac{Q_P^{I_P^a}}{Q_P},
%\end{align}
%where $Q_P^{I^a_P}=Q_P^{P^a_P}+N^{\text{Id}}_{P,\parallel}$ represents the number of qubits actively participating in the algorithm \textit{on an information processing basis}. We notice that $Q_P^{I^a_P} \neq Q_P^{P^a_P}$. This is because the identity gates in our assumption do not consume any power but introduce noise during the algorithm. 
%
%Now, we can express $I^a_P$ in a more usefull manner for our purpose: assuming that all gates last for the same amount of time, we can define the depth $D_P$ of the algorithm as the number of timesteps between the preparation of the qubits and their measurements. In this thesis we took the convention of not including the final measurements inside of the depth (in general we will always neglect the measurements gates in our energetic estimations). Using this, we deduce: $N_{\text{gates}}=Q^{I^a_P}_P D_P$ and thus:
%\begin{align}
%\mathcal{M}_P=D_P Q_P I^a_P \mathcal{M}^{(0)}_P.
%\end{align}
%We see from this expression that $I^a_P$ can then also be interpreted as the portion of "information-active" \textit{gates} there are inside the algorithm over the maximum number of information-active \textit{gates} there could exist for the provided values of $D_P$ and $Q_P$: $D_P Q_P$. This fact and more detailed explanations are provided in the caption of figure \ref{fig:power_information_activity} \textbf{a)}.
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.9\textwidth]{chapter4/images/power_information_activity}
%\caption{\textbf{a)}: An algorithm implemented on four qubits having a depth equal to four. The stars represent identity operations. The square and rectangle represent power-active gates (cNOT, single qubit rotations etc). Each qubit are being measured after the last gate on them have been applied. The blue "area" of the circuit represent the information-active part of the circuit. Because some qubits can be introduced later or measured earlier than at the very beginning or very end of the algorithm, this area is smaller than $Q_P D_P$. \textbf{b)}: An equivalent description of the algorithm when we averaged in time all the dynamic. This description is equivalent in the sense that the average power and metric will be the same as for the "real" algorithm: it is a simpler representation to consider in order to make energetic estimations. We see that $I^a_P$ can be computed by either calculating the ratio of the blue area over the area $Q_P D_P$, either by calculating the average number of information active qubits divided by $Q_P$.}
%\label{fig:power_information_activity}
%\end{center}
%\end{figure}
%\FloatBarrier

\subsubsection{Physical interpretations}
At this point the general models for both power and metric are defined. We now summarize and interpret physically what we introduced. First, the power consumption is composed of a passive cost which is here whatever the gates are implemented on the computer. In addition to that there is an active cost which will only be here if gates that require power (which usually exclude the identity gates) are being implemented. This is why knowing the number of qubits inside the algorithm is not enough, one has also to know the number of gates that are actually being implemented as they will \textit{actively} participate in term of power consumption. 

Also, each gate participating in the algorithm "brings in" noise. The more gates are implemented, and the longer it lasts, the more noise there might have. This is represented by the fact $\mathcal{M}_P$ increases if (for other parameter constant) any of the $N^{(i)}_{P,\parallel}$ increases, and by the fact $\mathcal{M}_P$ is proportional to $D_P$. We notice however that because the notion of activity can be different in term of information processing and power consumption, a different counting has to be done about the number of gates acting in parallel: some gates might not require power but will bring in noise. This is represented by the fact that the metric also involve a summation over $\mathcal{P}_{n.a}$.

Once those estimations have been done, the minimization under constraint can be performed as represented on the figure  \ref{fig:general_optimization_principle}.
% NE PAS SUPPRIMER: pour l'image
%\begin{align}
%P(\bm{\alpha},\bm{\beta})=\color{blue}Q_P\color{black}(\bm{\beta})\color{purple}a\color{black}(\bm{\alpha})+\sum_{i \in \color{purple}\mathcal{P}_a\color{black}}\color{blue}N^{(i)}_{P,\parallel}\color{black}(\bm{\beta})\color{purple}b^i\color{black}(\bm{\alpha})
%\end{align}
%\begin{align}
%\mathcal{M}_P(\bm{\alpha},\bm{\beta})=\color{blue}D_P\color{black}(\bm{\alpha}) \left(\sum_{i \in \color{purple}\mathcal{P}_a\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange} \mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha})\color{black}+\sum_{i \in \color{purple}\mathcal{P}_{n.a}\color{black}} \color{blue}N_{P,\parallel}^{(i)}\color{black}(\bm{\beta}) \color{orange}\mathcal{M}^{(i)}_{P}\color{black}(\bm{\alpha}) \color{black}\right)
%\end{align}
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.9\textwidth]{chapter4/images/general_optimization_principle2}
\caption{Overall principle of minimization of the power cost. The role of the different components participating to the energetic cost: the algorithm, the engineering part of the computer, the noise model (and the way it is quantified) are represented in blue, purple, orange respectively. They depend on two families of parameters $\bm{\alpha}$ and $\bm{\beta}$. The first one represents the tunable parameters in the physical architecture of the computer. It usually represents the tunable hardware parameters (qubit temperature, attenuation etc) but not only as the clock-speed could also be optimized and it would enter in this family. The second one represents the tunable parameters in how the algorithm is implemented, i.e how it is compiled, and how many qubits it requires.}
\label{fig:general_optimization_principle}
\end{center}
\end{figure}
\FloatBarrier
We see there that the algorithm, the quantity of noise and the engineering part of the model have clearly identified roles. The algorithm characteristics are described by the functions $Q_P(\bm{\beta}), N_{P,\parallel}^{(i)}(\bm{\beta}), D_P(\bm{\beta})$ and they will play a role both in the power and the metric. Indeed if we increase the number of qubits or the number of power-active gates, it will increase the power consumption of the computer. But it also play a role in the metric because longer algorithms, or algorithms that use a greater amount of gates active in parallel will be noisier. Then, the functions describing the power cost (per qubit or per power-active gate) are represented by the functions $a(\bm{\alpha})$ and $b^j(\bm{\alpha})$. Those functions will for instance represent the power efficiency of the cryogenic to remove the heat, how much heat the amplifiers are dissipating, what is the power of the pulse driving the quantum gates, etc. We can say that they represent the characteristics of the engineering aspect behind the computer and will thus only be involved in the expression of the power function. The quantity of noise introduced by the quantum gates will on the other hand only play a role in the metric as represented by the orange color. In summary, each expertise required to build a quantum computer have very well defined parameters to characterize, someone "at the end" has to regroup them and to solve the minimization under constraint which will provide all the experts the optimum tunable parameters they should choose in their respective field of expertise.

We finish by one important remark. We can notice here that despite the fact the gates in the family $\mathcal{P}_{n.a}$ do not require any active power, they will participate in an \textit{indirect} manner to the power consumption. Indeed, they will modify the expression of the metric and thus change the value of $P_{\min}$. As a concrete example, it is frequent to try to minimize the number of identity gates inside algorithms because the metric would then be lower \red{cite}. But with our approach of finding the minimum power, we will see that sometimes it can be helpful to introduce such elements because they could to reduce the amount of active gate in parallel. This will be a concrete example of the fact that despite they do not "directly" require power, identity operations "indirectly" influence the energetic cost required to run an algorithm, and we are going to illustrate it right now.
\subsection{A simple example of algorithm optimization}
Now, we can design an example in which we will optimize the shape of an algorithm that is running, in addition to the family of tunable parameters $\bm{\alpha}$ that play a role for the metric and the "engineering" part of the model. We will stay with the same model of power consumption we considered in the single qubit gate example (only the power dissipated into the attenuator will play a role). Thus, with the vocabulary we introduced, we will neglect any \textit{passive} cost involved in the computation. For the noise model, we will keep the assumption that only the thermal noise will affect the qubit and we will model it in the exact same manner as before. For the metric quantifying this noise, we will consider the worst-case infidelity of the gates as it verifies the property \ref{eq:sub_additivity} (the average infidelity wouldn't satisfy this property for instance \cite{carignan2019bounding}). Also as we are going to see we will only need two qubit and identity gates in the algorithm. The two qubit and identity gates will be assumed to last for a duration $\tau^{\text{timestep}}_P=25ns$. As we are going to keep the same noise model for each qubit as the one we introduced in the section \ref{sec:single_qubit_example}, the identity gates will be as noisy as a single qubit $\pi$-pulse (lasting $25ns$), and the two qubit gates twice as noisy as the identity gates (because two qubits are involved in their dynamic, and because they last for the same duration). Those two qubit gates will also require twice the power consumption of a $\pi$-pulse because they involve two qubits (identity gates will be "power free"). Of course there is nothing obvious behind this it is just a simple way to model the power consumption and noise behind the gates we used. This $\pi$-pulse will have the same properties than the one used in the previous section\footnote{It means that $\gamma_{\text{sp}}=1kHz, \tau=25 ns$}. Thus in this simple example we will have $\mathcal{P}_{a} = \{\text{2qb}\}$, $\mathcal{P}_{n.a} = \{\text{Id}\}$, $P=Q_P a +N^{(\text{2qb})}_{P,\parallel} b^{\text{2qb}}$ with:
\begin{align}
&a=0\\
&b^{\text{2qb}}=\frac{300-T_{\text{Q}}}{T_{\text{Q}}} A (2 \times P_g),
\label{eq:power_nisq}
\end{align}
and $\mathcal{M}_P=D_P \left(N_{P,\parallel}^{(\text{2qb})} \mathcal{M}^{(\text{2qb})}_{P}+N_{P,\parallel}^{(\text{Id})} \mathcal{M}^{(Id)}_{P}\right) $, with:
\begin{align}
 \mathcal{M}^{(\text{Id})}_{P}=\mathcal{M}^{(\text{2qb})}_{P}/2=(1+\overline{n}_{\text{BE}}(T_{\text{Q}})+\frac{\overline{n}_{\text{BE}}(300)}{A}) \gamma_{\text{sp}} \tau_P^{\text{timestep}}.
\end{align}
We recognize $\overline{n}_{\text{tot}}=\overline{n}_{\text{BE}}(T_{\text{Q}})+\overline{n}_{\text{BE}}(300)/A$ in this expression. We also see that we assumed $A \gg 1$ (as it will anyway be necessary to reach $\mathcal{M}_P=\mathcal{M}_{\text{target}}$ in what follows). We will ask an accuracy being $\mathcal{M}_{\text{target}}=1/3$ which implies that the fidelity of the algorithm output will be better than $2/3$ (because the metric is a pessimistic estimation: the "real" output fidelity will be better than the worst case one\footnote{And also because as explained before, the expression of $\mathcal{M}_P$ is only a bound on the exact value of the worst-case fidelity of the algorithm.}). 

Now, we need to describe the algorithm which will give us access to the average number of gate acting in parallel and $D_P$. For this example, we will consider running the quantum Fourier transform that we already introduced in the previous chapter. It will be directly implemented on physical qubits (not error correction yet). Of course, such algorithm is unlikely to be applied in the next few years on NISQ platforms as qubits are way too noisy: the task it would solve would be easily solved by a classical computer. But we take this as a simple example of the principle which could then be applied to more relevant NISQ (and also fault tolerant) algorithms. In order to simplify the discussion we will remove all the Hadamard gates that are required in this algorithm (they wouldn't change the general behavior we are going to show). The algorithm is represented for $5$ qubits on the figure \ref{fig:qft_5qubits}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/qft_5qubits}
\caption{\textbf{a)}: The QFT (where Hadamard gates have been removed for simplicity) performed on $5$ qubits with no compression. The vertical dotted lines represent the different timesteps of the circuits. On some of those timesteps, some qubits are waiting as represented by the stars indicating the associated "identity gates". Some other qubits are participating in a two qubit controlled-phase gate (which we described in the previous chapter). To reduce the level of noise, we can compress the circuit. It can be done by moving toward the left the different subcomponents represented by the colors (black, gred, yellow and blue). The red arrow represents how to do the first level of compression represented on \textbf{b)}. The red, yellow and blue subcomponents are pushed toward the left for two timesteps to put the first red two qubit gate inside the red dotted rectangle (removing the identity gates that were there). \textbf{b)}: First level of compression. The red, yellow and blue circuits have been pushed toward the left such that the first red two-qubit gate is done during the third timestep in parallel of the two qubit gate performed between the first and fourth qubit. \textbf{c)}: Second level of compression. The yellow subcomponent has also be pushed on the left (inside the yellow dotted rectangle) to reduce even more the algorithm duration and thus the noise. No further compression are possible. We can thus define a compression level for any size of QFT: $\epsilon=N_{\text{comp}}/N^{\max}_{\text{comp}}$ where $N_{\text{comp}}$ is the number of compression done and $N^{\max}_{\text{comp}}$ the maximum one (which is equal to $2$ in this example).}
\label{fig:qft_5qubits}
\end{center}
\end{figure}
As we see there are different way to actually implement it. Either we run the algorithm in an "uncompressed" manner as on the figure \ref{fig:qft_5qubits} \textbf{a)}, either we try to compress its length in such a way that the moments where qubits are waiting is minimized (on \textbf{c)}). The standard vision to implement algorithms is to make them the shortest possible. Indeed doing things this way the quantity of noise that is introduced is then minimal. But it might not be the best way to do things in order to minimize power consumption \textit{under the constraint} of aiming a targetted fidelity. Indeed, if the algorithm is highly compressed then a lot of gates are running in parallel which induces a big amount of active power consumption. More precisely, in this regime, the noise might be low (which implies that the qubits can be at higher temperature), but the heat dissipated in the attenuators will be high. Thus on one hand the power cost is minimized because the Carnot efficiency is higher, but we have more heat to evacuate. In the other limit it is the opposite. If the algorithm is minimally compressed (i.e more qubits are waiting), the noise will be higher (the qubits have to be colder) but the heat dissipated will be lower. In the end, the optimal way to compress the algorithm is not obvious if one wants to minimize the power consumption. To choose the optimal way we should compress the algorithm, we then introduce the parameter $\epsilon \in [0,1]$. It is defined as the number of compression it is possible to do over the maximum number of compression we can do: $\epsilon=N_{\text{comp}}/N_{\text{comp}}^{\max}$. The exact definition of a compression is given in the caption of the figure \ref{fig:qft_5qubits}. The other parameters we will optimize will be as previously $T_{\text{Q}}$ and $A$.
 
%It brings us to the last point: we explained which noise model, metric and resource to minimize (the expression of the power). The last thing to provide is the set of parameters on which the optimization can be performed. We are interested in the minimum power to implement this algorithm assuming that we can tune $T_{\text{Q}},A$ and $\beta \in [0,1]$, where $\beta \in [0,1]$ is the compression level which is defined in the caption of figure \ref{fig:qft_5qubits}. They are thus the parameters on which the optimization should be performed. But to get intuition behind the role of the compression factor, we will calculate the minimum power, minimized on the set $\bm{\alpha}=\{T_{\text{Q}},A\}$ for different values of $\beta$, and we will see for which value of $\beta$ the curve reaches a minimum. 

We now represent the minimum power consumption (minimized on $T_{\text{Q}},A$) as a function of $\epsilon$ in order to visualize the influence of the compression. It is represented on the figure \ref{fig:min_power_fct_compression}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/min_power_fct_compression}
\caption{Minimum power for a QFT implemented on $30$ qubits (minimized on $T_{\text{Q}},A$) as a function of the compression factor $\epsilon$. Bottom left inset: zoom around the minimum. Upper right inset: optimal temperature $T_{\text{Q}}^{\text{opt}}$ as a function of the compression factor. On this curve, we see that the algorithm should be implemented with a compression factor about $\epsilon^{\text{opt}} \approx 0.75$. The bigger the compression is, the higher the temperature can be which improves the Carnot efficiency. But at the same time, more power-active gates are implemented in parallel which dissipates more heat into the attenuators. The optimal compression factor results from this competition.}
\label{fig:min_power_fct_compression}
\end{center}
\end{figure}
\FloatBarrier
In this curve, we see that as expected there is an optimal compression factor on which the algorithm should be implemented in order to minimize the power consumption. It results from the competition we just described. This curve has been represented for a QFT implemented on $30$ qubits but when we increased the size of the QFT, the same kind of behavior remained: there were an optimal compression factor to choose resulting from the competition between noise and power. We also see that the optimization can be quantitative: the curve varies on more than one order of magnitude on the range of compression factor we considered. We could however consider that the conclusion of this curve is that the algorithm should anyway be close to a maximum compression (the power for a maximal compression would not be much higher than the minimum). But in practice we can expect the conclusion to be very system dependant: it highly depends on the characteristics of the algorithm implemented, the engineering aspect behind the computer, the noise model behind the quantum gates and the metric used to quantify it. We mainly took this specific example of the QFT because we already introduced the algorithm (and we will reuse it later on). 

The message we want to give here is simply that it is possible to optimize algorithms to make them minimize the power of the computer, and this minimization should at the same time involve the physical "hardware" parameters describing the computer. Here we took the simplest possible example which consisted in adding or removing identity operations, but the overall principle would remain if a given algorithm can be implemented in various manner. For instance, if different kind of gates can be used: some consume low power but introduce a high noise (and reciprocally), the optimal way to compile the algorithm could be deduced allowing to introduce energetic considerations in algorithm compilation problems.
\section{Adapting the framework for fault tolerance}

Now, that the concepts have been provided for a computer not using quantum error correction, we would like to adapt them to fault tolerant quantum computing. This is the role of this section. Ideally, we would like to keep the same interpretation of those quantities and replace all the physical quantities such as physical depth, number of qubits, power and number of active parallel gates by their logical equivalent. Under some approximations, we will see that it is possible to do so, at least for concatenated codes. However we will also see that some differences will remain: the notion of power and information activity will be a little bit different here.
\subsection{Metrics on the logical level}
Let us talk about the metric first. For that, we will use the tools that we already introduced: the probability of error of a logical gate\footnote{We remind that in general $p_L$ has not necessarily the interpretation of a probability, in more general case it is a mathematical norm (which can usually be related to a probabilistic interpretation). It will be the case if the noise model behind the physical gate is probabilistic. To keep the explanations simple we nonetheless assume the probabilistic interpretation to be appropriate.}. Calling it $p_L$, the probability that any of the gate in a computation composed of $N_L$ logical gates fails is simply $N_L p_L$. The implicit assumption here is that all gates have the same failure probability. This is not true but fault tolerance very frequently reason on worst-case scenario (because more accurate estimations are complicated). Thus, here, $p_L$ actually corresponds to the probability of failure of the "worst" logical gate: $N_L p_L$ is an over estimation of the probability of error that will be our estimation of the quantity of noise introduced in the algorithm. In some sense, considering the algorithm as a big logical gate, $p_L$ will play the role of what measures the quantity of noise in a (logical) gate, and will verify the sub-additivity property \eqref{eq:sub_additivity}. Because of that the general description we did is still valid on the logical level, and we have a particular case of \eqref{eq:physical_metric_gen}:
\begin{align}
&\mathcal{M}_L=D_L \left(\sum_{i \in \mathcal{P}_a \cup \mathcal{P}_{n.a}} N_{L,\parallel}^{(i)} \right) \mathcal{M}^{(0)}_{L}\\
&\mathcal{M}^{(0)}_{L} = p_L
\end{align}
With that, we notice that the metric we used before is simply switched on the logical level. Everything behave in the exact same manner.
\subsection{Power on the logical level}
Now, we can talk about the power part of the problem. One question is to wonder if it is possible to define it in an "effective manner" on the logical level. Can we just replace all the physical quantities entering in this expression by their logical counterpart and keep the same interpretation ? To answer this question, we need to find the expression of the power (thus breaking down the fault-tolerant algorithm into its physical components) to try to then "recognize" the logical components with the hope that it can lead to a nice expression, analog to \eqref{eq:physical_power_gen}. The first step will thus be to estimate the number of physical components (qubits and gates) that are required in a fault-tolerant algorithm. This is the role of this section. 

\subsubsection{The general construction behind FT logical gates}
To begin, we need to remind the how a level-1 logical gate is constructed from physical elements, more precisely, a 1-Rec as defined in the chapter 2. It is represented for a single qubit logical gate on the figure \ref{fig:steane_method_full_ch4}. The construction of a two qubit logical gate such as a cNOT follows the same structure excepted that error correction will be performed on the two logical data qubits (thus, we would need all the structure involving the ancilla "twice", one per logical qubit).
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/steane_method_full}
\caption{Fault-tolerant implementation of a single qubit logical gate for one concatenation, based on Steane method. Each horizontal line represents a logical qubit for one concatenation level, composed of seven physical qubits (because we use Steane code). The first line represents the logical data qubit: i.e the logical qubit participating in the calculation. The four bottom line are the four \textit{ancilla} logical qubits that are required to implement fault-tolerantly the error correction. We need at least (further details in the text) two syndrome ancilla (which are interacting with the logical data qubit to measure the syndrome), and two verifier logical ancilla (which are here to check that the syndrome ancilla do not contain error that could damage the data qubits). The preparation procedure for the ancilla qubits is represented on the figure \ref{fig:preparation_0logical_ch4}.}
\label{fig:steane_method_full_ch4}
\end{center}
\end{figure}
\FloatBarrier
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.7\textwidth]{chapter4/images/preparation_0logical}
\caption{Preparation of the $\ket{0_L}$ logical state. The preparation of the $\ket{+_L}$ logical state can be done via a similar procedure where (i) the direction of all the cNOT is being reversed (ii) four hadamard are added on the four qubits not affected by Hadamard here, right after their initialization in $\ket{0}$, (iii) the three Hadamard of this figure are being removed.}
\label{fig:preparation_0logical_ch4}
\end{center}
\end{figure}
\FloatBarrier
The role of each of those components has already been explained in the second chapter of this thesis, but we briefly remind them. The unprotected 1-Ga logical gate is implemented right before the purple box. It is implemented by a transversal implementation of the gate (i.e if the logical gate is Hadamard, the 1-Ga is implemented by applying a Hadamard on each physical qubit). It is then followed by quantum error correction which requires two "syndrome" logical ancilla corresponding to the second and third black lines. Their role is to detect $X$ and $Z$ errors occuring on the data qubits to know which appropriate correction should be implemented. The correction can then be applied. However, it is not strictly a requirement in practice: indeed it is enough to "keep track" of the errors with a classical computer, more precisely to keep in memory the result of the syndrome\footnote{In principle the correction only must be applied only before the non-transversal gates which are done through a different procedure as the one shown on figure \ref{fig:steane_method_full_ch4}. We come back on that point later.}. This is why in the calculations we will not include the cost of the correction following the syndrome\footnote{\red{Comment about magic gate for this}}. Now, for the construction to be fault-tolerant, verifier logical ancilla are required and represented by the third and last black line. They are interacting with the syndrome logical ancilla before being measured. This measurement is here to ensure that the potential faults that might have occured during the preparation of the syndrome ancilla will not corrupt the logical data qubit. Given the value of this measurement, the syndrome ancilla will either be accepted (and interact with the data qubit to detect the potential errors), or will be rejected. In the scenario it is rejected, new verifiers and syndromes ancilla have to be generated until the moment the verification succeeds. In principle, "many" syndromes and verifiers ancilla have to be prepared in parallel so that one will always be accepted when needed. In practice, the extra amount of those ancilla required will be negligible. Indeed based on the fact that it is more probable for an ancilla to be accepted, the extra amount of ancilla one would need to prepare in the case of failure will much smaller than the number of ancilla we would need in case the acceptation always succeeds. It will then be possible to neglect them in our energetic estimation. We show this property more rigorously in the appendix \red{to write down}. In the end, this circuit, drawed for each logical gate we want to implement, and the principle behind the concatenation is all what we need conceptually to deduce the number of physical qubits and gates that are required in a 1-Ec after $k$ level of concatenations. The exact counting of the number of physical element will differ for each logical gate one want to implement but the principle will be the same.

We show the principle of the calculation for a single qubit logical gate and single qubit identity gate. What we refer as single qubit physical gate will either be Pauli or Hadamard (in our energetic estimation we will identify those gates as if they were the same). We assume that we want to implement a 1-Rec for such single qubit logical gate. Assuming that the syndrome ancilla are always accepted, we need $7 \times 5 = 35$ physical qubits: $7$ for the logical data qubit, $7 \times 2$ for the syndrome ancilla qubits and $7 \times 2$ for the verifier ancilla qubits. We can also find the number of physical gates required. In order to make this counting, we assume that we can only do measurement in the computational basis ($Z$-measurement): measuring in the $X$ basis requires to apply Hadamard gates before a $Z$-measurement. We also assume that qubits can only be available in their ground state $\ket{0}$ (preparing $\ket{+}$ requires to apply an Hadamard on $\ket{0}$). With those assumptions we find that we need $7 \times 4+9 \times 4=64$ cNOT: $7 \times 4$ for the transversal implementation of the cNOT represented on the figure \ref{fig:steane_method_full_ch4}, and $9 \times 4$ for the preparation of the $\ket{+_L}$ and $\ket{0_L}$ states for the ancilla (see figure \ref{fig:preparation_0logical_ch4}). For the measurement gates, we need $7 \times 4$ of them to measure all the ancilla. We also need single qubit gates: $7$ for the transversal implementation of the gate on the logical data qubit, $7 \times 2$ Hadamard to apply before the $X$-measurement (because we can only to $Z$-measurements), and $3 \times 2 + 4 \times 2 = 14$ Hadamard for the preparation of the ancilla states as explained in the caption of figure \ref{fig:preparation_0logical_ch4}. It gives us $35$ single qubit gates to apply. We also need to make some qubits necessarily wait at some point. For instance, the syndrome logical qubit has to wait for the measurement outcome of the verifier to know if they can be injected or not: they are then doing a noisy physical identity. We won't go in the detail of this counting but in the end, we would find $36$ physical identity gates by looking at all the places the physical qubits composing the logical ones necessarily have to wait. In the end, doing an appropriate counting for each type of logical gate that has to be implemented, we have access to the table \ref{table:FT_gate_breakdown} which represents for each level-1 gate (on the line), the number of physical elements (on the column) its 1-Rec is composed of \footnote{To be very precise, the 1-Rec of a measurement is defined as 1-Ec followed by 1-measurement (the 1-Ec is "before" the 1-Ga measurement gate). This is defined this way for theoretical reason to prove the threshold \cite{aliferis2005quantum}. As we are interested to find the number of physical elements when concatenating, the elements in this 1-Ec would already have been counted by the gate before the measurement: taking them into account "again" would lead to an overcounting of the number of physical elements. This is why we remove the elements that would be in the 1-Ec before the measurement gates which explains why the last line of table \ref{table:FT_gate_breakdown} is composed of three zeros.}. We see from this table that as we could expect, a logical identity is the same as a logical single qubit gate excepted that the transversal operation is composed of identity gates. This is why it contains $7$ less single qubit gate but $7$ more identity gates than a logical single qubit gate.
\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
	\hline
	& lvl-0 cNOT & lvl-0 Single & lvl-0 Identity & lvl-0 Measurement\\
	\hline
   lvl-1 cNOT & $135$ & $56$ & $72$ & $56$ \\
   \hline
   lvl-1 Single & $64$ & $35$ & $36$ & $28$ \\
   \hline
   lvl-1 Identity & $64$ & $28$ & $43$ & $28$\\
   \hline
   lvl-1 Measurement & $0$ & $0$ & $0$ & $7$\\
   \hline
\end{tabular}
\caption{Each row lists a FT logical gate and tabulates the lower level components required for the listed gate as columns. Those level-0 components are thus physical gates. The single qubit gates here are either Hadamard or Pauli gates.}
\label{table:FT_gate_breakdown}
\end{center}
\end{table*}
\FloatBarrier
\subsubsection{Estimation of the number of physical gates acting in parallel}
This table allows us to deduce, based on a recursive reasoning the number of physical qubits and gates of each type that are required for a level-k logical gate. Let us start with the number of physical gates. We assume that we have $N_L^{\text{cNOT}}$, $N_L^{\text{1qb}}$, $N_L^{\text{Id}}$,$N_L^{\text{Meas}}$ logical cNOT, single qubit, identity gates and measurement gates in the algorithm. We put the number of logical gates required by the algorithm in a three dimensional vector $X_0=(N_L^{\text{cNOT}},N_L^{\text{1qb}},N_L^{\text{Id}},N_L^{\text{Meas}} )^T$. We can deduce the number of physical gates of each type after $k$ level of concatenations via the recursive formula $X_k=A^k X_0$, where:
\begin{align}
& A=\begin{pmatrix} 135 & 64 & 64 & 56\\ 56 & 35 & 28 & 28\\ 72 & 36 & 43 & 28 \\ 0 & 0 & 0 & 7\end{pmatrix},
\end{align}
and where the first line of $X_k$ will represent the number of physical cNOT, the second line, the number of physical single qubit (either Hadamard or Pauli), the third line the number of physical identity gates where the qubits have to wait for one physical timestep, and the last one the number of physical measurement gates. The formula for $k=1$ is just applying the table \ref{table:FT_gate_breakdown} to the number of gates implemented in the algorithm (removing the measurement from the counting for reason explained above). It gives us the number of physical gates after the first concatenation level. Each of them are then "promoted" into 1-Rec for the second concatenation level: we just have to "reuse" this table another time on the vector $X_1=A X_0$. The same principle applies recursively for further concatenation levels which explains why $X_k=A^k X_0$. In the end, from the knowledge of the number of gates required by the algorithm, we can access the number of physical gates required in the algorithm for an arbitrary concatenation level. We deduce that we have the following \textit{total} number of physical gates required in the algorithm:
\begin{align}
X_k = \left(
\begin{array}{c}
 \frac{1}{3} 199^k (2 N_L^{\text{cNOT}}+N_L^{\text{Id}}+N_L^{\text{1qb}})+\frac{7^k}{3} \left(N_L^{\text{cNOT}} -N_L^{\text{Id}} - N_L^{\text{1qb}}\right) \\
 \frac{7}{48} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{48} \left(-14 N_L^{\text{cNOT}} -7 N_L^{\text{Id}} +41\  N_L^{\text{1qb}}\right) \\
 \frac{3}{16} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{16} \left(-6 N_L^{\text{cNOT}} +13 N_L^{\text{Id}} -3\ N_L^{\text{1qb}}\right) \\
 \frac{7}{48} 199^k (2 N_L^{\text{cNOT}}+ N_L^{\text{Id}}+ N_L^{\text{1qb}})+\frac{7^k}{48}\left(-14 N_L^{\text{cNOT}} -7 N_L^{\text{Id}}+48N_L^{\text{Meas}}-7N_L^{\text{1qb}}\right)\\
\end{array}
\right)
\label{eq:number_physical_gate_k_concat}
\end{align}
We notice from this expression that two numbers seems to have a particular importance in this formula: $199$ and $7$ (they are the only two numbers elevated to a power $k$). They correspond to the two eigenvalues of the matrix $A$. In order to interpret their signification, let us first neglect the term proportional to $7^k$. Doing this, we realize that $X_k \propto (2 N_L^{\text{cNOT}}+N_L^{\text{Id}}+N_L^{\text{1qb}})$. It means that whatever the physical gate we are looking at, the exact type of gates implemented by the algorithm does not really matter, what matters is the \textit{total number} of logical gates involved (counting twice the cNOT, and removing the measurement gates on the logical level for a reason given in a few lines). For instance, if we had implemented $1$ logical identity, or $1$ single qubit logical gate (and no other gates), the number of physical components of each type wouldn't change. It symbolises the fact that the fault tolerant construction of the gates contains a dominant part that does not really depend on the gate that is being implemented, and we can understand that from the figure \ref{fig:steane_method_full_ch4}: whatever the 1-Ga has to be protected, the error correction structure is the same for any of the logical gate to implement. But this has two exceptions: first we need two implementation of error correction for a cNOT because it involves two logical qubits, it explains the $\times 2$ in front of $N_L^{\text{cNOT}}$. Then, the measurement gates will not be followed by error correction (because the information becomes classical when qubits are being measured). It explains why $N_L^{\text{Meas}}$ does not appear in the term proportional to $199^k$: the number of logical measurement gates does not play a significant role in the number of physical elements when concatenations are being performed. But the error correction is not everything, there is also the transversal implementation of the gate (the 1-Ga). And this part will differ depending on the exact logical gate we want to implement. For instance a logical identity gate would require $7$ less single qubit gate and $7$ more identity gates to be implemented. Those little differences are expressed by the much smaller eigenvalue $7$. And we see that the terms proportional to this eigenvalue are not the same for each physical gates (because the physical gates do vary depending on the logical one). 

Now, we are here interested in the \text{average} number of physical gate that are acting in parallel. In order to access it, we need to know the average number of gate acting in parallel for the ideal algorithm (for each type: single qubit, identity and two qubit gates). Putting those number in a vector $X_0=(\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}},\overline{N}_{L,\parallel}^{\text{Meas}})^T$, we can deduce the total number of physical gate inside an average algorithm logical timestep (one algorithm timestep correspond to the time it takes to execute any logical gate\footnote{Some logical gates can in principle be implemented faster than others. For instance a logical identity could only last for two timestep as the transversal implementation of the gate could be done instantaneously (as an identity operation can be performed instantaneously). But as we need to keep all the qubits "synchronized" the longest logical gate to execute should give the duration of a logical timestep of the algorithm (even though "smart" optimizations could be performed for specific algorithms in order to reduce slightly the algorithm duration).}). It naturally corresponds to \eqref{eq:number_physical_gate_k_concat} where we replace the number of logical gates by the number of logical gates acting in parallel ($N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb},\text{Meas}\}$). Now, this is not exactly the average number of physical gates that are acting in parallel. Indeed, a logical timestep is composed of a given number of physical timesteps. More precisely, calling $\tau_P^{\text{timestep}}$ the duration of a physical timestep (which corresponds to the duration of the longest physical gate used in the FT construction: we will assume it corresponds to both the duration of a cNOT and measurement gates in what follows), we have after $k$ concatenations a logical gate that lasts for $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. Indeed, we can see from figure \ref{fig:steane_method_full_ch4} that for one level of concatenation, the logical data qubit are going through three timesteps: the first one corresponds to the transversal implementation of the gate, followed by two timesteps used to perform the syndrome measurement\footnote{We remind that we assume the correction is not physically performed with out assumptions of "keeping track" of the syndrome with a classical processing.}. Increasing the concatenation level, each of those timestep will again be multiplied by three. This is how we deduce $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$. We notice here that the ancilla must however be prepared in advance: including their preparation and the moment they can be "plugged out", the duration of this gate would be longer. But as explained on the figure \ref{fig:timestep_logical_gate}, the good timescale to consider to estimate the average number of gates would still be $\tau_{L}^{\text{timestep}}=3^k \tau_P^{\text{timestep}}$.
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/timestep_logical_gate}
\caption{Determination of the average number of physical gates acting on an average logical timestep. On the first line of this figure are represented a sequence of three logical gates that are composed of three physical timesteps as indicated by the three red rectangles (the transversal implementation, and the measurement of the $X$ and $Z$ syndromes). Those logical gates require ancilla which are represented on the line below by the matching colors. Between the moment the ancilla are prepared and measured, there is more than three timesteps (we represented $6$ here for simplicity, but the exact number would be different and would actually depend on the ancilla we are looking at). However, in order to compute the average number of physical gates acting in one logical gate, everything will behave \textit{as if} those gates were actually implemented in parallel of the $3$ timesteps. Indeed, if we focus on the red logical gate, the ancilla might have gates applied on them before ($1$ and $2$ red boxes) and after the logical gate ($6$ red box), but the preceding and following logical gates would exactly compensate those missing gates. Rigorously speaking, this is true if we neglect the boundary of the algorithm and if we are interested into the average number of gates acting in parallel (which is the case).}
\label{fig:timestep_logical_gate}
\end{center}
\end{figure}
\FloatBarrier
%Finally, calling $\tau_P^{\text{1qb}}$ and $\tau_P^{\text{cNOT}}$ the duration of the physical single and cNOT gates respectively, the average number of single and two physical qubit gates acting in parallel in the algorithm can be expressed as:
Finally, the average number of $x \in \{\text{cNOT}, \text{Id}, \text{1qb},\text{Meas}\}$ physical gates in this logical timestep is:
\begin{align}
&\overline{N}_{L,\parallel}^{x}(k)=N_{\text{during } \tau_L}^{x}(k) /3^k
\label{eq:average_number_physical_gate_timestep}
\end{align}
Where $N_{\text{during } \tau_L}^{x}(k)$ is the number of $x$ type physical gates that are inside an average logical timestep, i.e the number of $x$ physical gates there are assuming that $\overline{N}_{L,\parallel}^{\text{cNOT}},\overline{N}_{L,\parallel}^{\text{1qb}},\overline{N}_{L,\parallel}^{\text{Id}},\overline{N}_{L,\parallel}^{\text{Meas}}$ logical gates are acting in parallel in the algorithm. We find (those numbers are simply obtained by replacing $N_{L}^{x} \to N_{L,\parallel}^{x}$ for $x \in \{\text{cNOT}, \text{Id}, \text{1qb}\}$ in \eqref{eq:number_physical_gate_k_concat}):
\begin{align}
&N_{\text{during } \tau_L}^{\text{cNOT}}(k)= \frac{1}{3} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{3} \left(\overline{N}_{L,\parallel}^{\text{cNOT}} -\overline{N}_{L,\parallel}^{\text{Id}} - \overline{N}_{L,\parallel}^{\text{1qb}}\right)
\label{eq:tot_number_physical_gate_timestep1}\\
&N_{\text{during } \tau_L}^{\text{1qb}}(k)=\frac{7}{48} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{48} \left(-14 \overline{N}_{L,\parallel}^{\text{cNOT}} -7 \overline{N}_{L,\parallel}^{\text{Id}} +41\  \overline{N}_{L,\parallel}^{\text{1qb}}\right)
\label{eq:tot_number_physical_gate_timestep2}\\
&N_{\text{during } \tau_L}^{\text{Id}}(k)= \frac{3}{16} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{16} \left(-6\overline{N}_{L,\parallel}^{\text{cNOT}} +13\overline{N}_{L,\parallel}^{\text{Id}} - 3 \overline{N}_{L,\parallel}^{\text{1qb}}\right) 
\label{eq:tot_number_physical_gate_timestep3}\\
&N_{\text{during } \tau_L}^{\text{Meas}}(k)= \frac{7}{48} 199^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})+\frac{7^k}{48} \left(-14 \overline{N}_{L,\parallel}^{\text{cNOT}} -7 \overline{N}_{L,\parallel}^{\text{Id}}+48 \overline{N}_{L,\parallel}^{\text{Meas}} - 7 \overline{N}_{L,\parallel}^{\text{1qb}}\right) 
\label{eq:tot_number_physical_gate_timestep4}
\end{align}
The second parenthesis of those expressions becoming negligible\footnote{We are only interested in order of magnitude estimations. So for us a quantity will be negligible with respect to another one as soon as it is smaller (or equal) to it which is clearly the case here.} to the first one as soon as $k=1$, and because we won't need to find the average number of physical identity gates (because they are not consuming any power), we will approximate the average number of physical single, cNOT and measurement gates by:
\begin{align}
&\overline{N}_{L,\parallel}^{\text{cNOT}}(k) \approx \frac{1}{3} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep1}\\
&\overline{N}_{L,\parallel}^{\text{1qb}}(k) \approx \frac{7}{48} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+ \overline{N}_{L,\parallel}^{\text{Id}}+ \overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep2}\\
&\overline{N}_{L,\parallel}^{\text{Meas}}(k) \approx \frac{7}{48} \left(\frac{199}{3}\right)^k (2 \overline{N}_{L,\parallel}^{\text{cNOT}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{1qb}})
\label{eq:average_number_physical_gate_timestep3}
\end{align}
This is all what we need in order to access the active-power part of the power function.
%The ratios $\frac{\tau_P^{\text{1qb}}}{\tau_L^{\text{timestep}}}$ and $\frac{\tau_P^{\text{cNOT}}}{\tau_L^{\text{timestep}}}$ in \eqref{eq:average_number_physical_single_cNOT_timestep1} and \eqref{eq:average_number_physical_single_cNOT_timestep2} represent the  fact that the associated gate might be faster than the duration of the physical timestep (we have to take in account the fact that for a given physical timestep the gate will not always be activated, it will be important for power estimations). Now, as we will assume that the cNOT is the longest physical gate we will have $\tau_P^{\text{cNOT}}=\tau_P^{\text{timestep}} \Rightarrow \frac{\tau_P^{\text{cNOT}}}{\tau_P^{\text{timestep}}}=1$ in practice. The precise explanations for this are given in the caption of the figure \ref{fig:estimation_average_number_gates}.
%\begin{figure}[h!]
%\begin{center}
%\includegraphics[width=0.7\textwidth]{chapter4/images/estimation_average_number_gates}
%\caption{How to estimate the average number of physical gates acknowleding the fact they can be faster than $\tau_P^{\text{timestep}}$. This image also represents the difference between physical and logical timestep (for $k=1$ because $\tau_L^{\text{timestep}}=3 \tau_P^{\text{timestep}}$ here). The duration of the physical timestep is given by the longest physical gate acting in the computer (which is not represented on this image). Each of the two "lines" on this figure represent a physical qubit on which single qubit gates represented by the black rectangles are being applied. There are $N^{\text{1qb}}=6$ of them. As the gates are faster than a physical timestep, the average number of single qubit gate acting in parallel is not given by $N^{\text{1qb}}/N_{\text{timestep}}=6/3=2$. Instead, we have to calculate the black area: $N^{\text{1qb}} \tau_P^{\text{1qb}}$ and divide it by the grey are \textit{covered by one physical qubit} (thus half the total grey area in this example). It gives: $\overline{N}^{\text{1qb}}_{\parallel}=N^{\text{1qb}} \tau^{\text{1qb}}_P/\tau_P^{\text{timestep}}$. To illustrate, we can consider the case in which the single qubit gate are lasting for the entire timestep (the black area would entirely cover the grey one). In this case we would find $\overline{N}^{\text{1qb}}_{\parallel}=2$ as expected.}
%\label{fig:estimation_average_number_gates}
%\end{center}
%\end{figure}
%\FloatBarrier 
\subsubsection{Estimation of the number of physical qubits used in the computer}
The number of physical gates being estimated for a given concatenation level $k$, it remains to estimate the number of physical qubits to be able to finally write down the expression of the power. For the physical gates, we were interested in finding their average number because the associated power consumption was an active type. For the physical qubits, we need to find the bottleneck of the algorithm. Indeed physical qubits cannot be removed from the computer when they are not being used, so we need to find the moment when the maximum number of physical qubits will be required to estimate their number. 

In order to do the estimation, we notice that the number of ancilla qubits dominates the total number of physical qubits required. Indeed, for $k=1$ for instance we would need $28$ (resp $28 \times 2$) ancilla qubits for a single or identity (resp cNOT) logical qubit gate. Compared to the $7$ to $14$ physical data qubits, as we are only interested in order of magnitude this is a fair approximation to make. Furthermore, increasing the concatenation level would only make the number of physical ancilla qubits dominate even more. For this reason, we will only try to estimate the number of ancilla qubits. Then, we remind that the $k$'th concatenation level is obtained from the $k-1$ level in which each physical gate has been promoted into a 1-Rec. Thus, we can estimate the number of physical qubits. We first assume that the algorithm requires a unique logical timestep composed of $(N_{L,\parallel}^{\text{cNOT}},N_{L,\parallel}^{\text{1qb}},N_{L,\parallel}^{\text{Id}},N_{L,\parallel}^{\text{Meas}})$ cNOT, single, identity and measurement logical gates acting in parallel. From this knowledge, we can find the the total number of physical gates required on the $k-1$ level. Multiplying this number by $28$ for the single qubit and identity gates, and $28 \times 2$ for the cNOT, we deduce the total number of ancilla qubits required. We notice that we don't multiply measurement gates by $28$ because they do not require ancilla (because they are not followed by a quantum error correction procedure). It would give us access to the total number of ancilla qubit after $k$ concatenation, and thus roughly the total number of physical qubits. We notice that this calculation assumes that no ancilla qubits can be recycled after $k$ concatenation (i.e each gate on the $k-1$ level needs "fresh" ancilla). The $X$-syndrome ancilla are participating to $9$ physical timesteps. Thus, in principle, we can reuse them once they have done those $9$ timesteps. In a similar way, the verifier ancilla can be reused (even earlier because they are used for a smaller amount of timesteps). Properly counting the number of ancilla that could be reused would however be a complicated task for an arbitrary concatenation level. Furthermore, in practice we will mainly be interested in the first $3$ concatenations levels in the next chapter (more concatenation level would imply an unrealistic power demands for all practical purposes, with the models we will consider in the following chapter). Because of that, the number of timesteps for the logical gates on the $k-1$ level is also equal to $9$: $\tau^{\text{timestep}}_L/\tau^{\text{timestep}}_P=3^{k-1}=9$ which means that anyway the level of recycling of the syndrome ancilla qubit would be "poor" (but we might be able to recycle roughly half of the verifier ancilla qubits). We assumed in the end that the ancilla qubits are not recycled within this logical gate which gives a slight overestimation of the total number of physical qubits that would really be required. In summary, using \eqref{eq:tot_number_physical_gate_timestep1},\eqref{eq:tot_number_physical_gate_timestep2} and \eqref{eq:tot_number_physical_gate_timestep3}, we can estimate that the total number of physical qubits required in an algorithm composed of a unique logical timestep having $(N_{L,\parallel}^{\text{cNOT}},N_{L,\parallel}^{\text{1qb}},N_{L,\parallel}^{\text{Id}},N_{L,\parallel}^{\text{Meas}})$ cNOT, single, identity and measurement logical gates acting in parallel is $Q_P(k) \approx \frac{28}{199} 199^k (2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}})$. Now, an algorithm is composed of many logical timesteps. With our assumption where the ancilla qubits are not being recycled within a logical gate, the number of physical qubits required is given by the moment in the algorithm where $2 N_{L,\parallel}^{\text{cNOT}} + N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}$ will be \textit{maximum} (which is in some way the "bottleneck" in term of physical resources required). Thus, the number of physical qubits can be written as:
\begin{align}
Q_P(k) \approx \frac{28}{199} 199^k \max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]
\label{eq:number_physical_qubits_k_concat}
\end{align}
where $i$ denotes the logical timestep on which there are $N_{L,\parallel,i}^{\text{cNOT}}$, $N_{L,\parallel,i}^{\text{1qb}}$, $N_{L,\parallel,i}^{\text{Id}}$ logical cNOT, single qubit and identity gates acting in parallel. In principle, for the same reason that consecutive gates on the $k-1$ level had to use fresh ancilla, we cannot use the same ancilla for consecutive logical gates because the ancilla preparation takes longer than the duration of the logical gate. Fortunately, as shown in the appendix \red{to write and double check}, the most pessimistic estimation of that would lead to only multiply our previous es $Q_P$ by $4$ in \eqref{eq:number_physical_qubits_k_concat}: it wouldn't change its order of magnitude such that we won't take this coefficient into account. At this point we can then consider that \eqref{eq:number_physical_gate_k_concat} is the number of physical qubits used after $k$ concatenations.

However, to define the power on the logical level, we would like to "make appear" the number of logical qubits $Q_L$. In order to do it, we can notice that we have\footnote{It assumes that the algorithm uses the minimal number of logical qubits it conceptually need. Indeed, this equation means that the moment the maximum number of logical qubits are doing something "together" is equal to the number of logical qubits. But we could imagine inefficient implementation where this wouldn't be true.} $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}+N_{L,\parallel,i}^{\text{Meas}} \right]=Q_L$, where $N_{L,\parallel,i}^{\text{Meas}}$ is the number of logical measurement gates at the timestep $i$. The reason behind this equation can intuitively be understood from the figure \ref{fig:bottleneck_algo_physical_qubits}. We remind that $N_{L,\parallel,i}^{\text{Meas}}$ did not appear in \eqref{eq:number_physical_qubits_k_concat} because measurement gates do not require ancilla, and our estimation of the number of physical qubits was given by the number of ancilla (as they dominate). Calling $i_0$ the associated logical timestep, we deduce that an estimation for the total number of physical qubits required by the computer is, for $k>0$:
\begin{align}
Q_{P}(k) \approx \frac{28}{199} 199^k (Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx \frac{28}{199} 199^k Q_L,
\label{eq:number_physical_qubits_from_logical}
\end{align}
where $N_{L,\parallel,i_0}^{\text{Meas}}$ corresponds to the number of logical measurement gates active in parallel at this "bottleneck timestep" $i_0$. We explain why $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ in a few lines. This formula does not apply for $k=0$ as it is based on estimating the total number of physical qubits from the number of ancilla qubits. And there are no ancilla qubits when no concatenations are performed. For all practical purpose, we can comment that it will frequently be true for algorithm to have $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ (where $\approx$ means same order of magnitude). Indeed, if this equation is not true, it means that on the timestep $i_0$, the dominant number of logical gates are measurement gates. On the logical timestep right before, all those measurement gates were either logical identity, single qubit or cNOT gates. It implies that $2 N_{L,\parallel,i_0-1}^{\text{cNOT}} + N_{L,\parallel,i_0-1}^{\text{1qb}}+N_{L,\parallel,i_0-1}^{\text{Id}} > N_{L,\parallel,i_0}^{\text{Meas}}$ (this is a strict inequality because on the timestep $i_0-1$, the measurements are replaced by other logical gates, but qubits that were not measured in $i_0$ might be affected by some other logical gates). Thus, $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]>N_{L,\parallel,i_0}^{\text{Meas}}$. And as $N_{L,\parallel,i_0}^{\text{Meas}}$ was the dominant number of gates on timestep $i_0$, it shows that $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]$ gives a good estimation to $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}+N_{L,\parallel,i}^{\text{Meas}}\right]$, and thus that $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$. In what follows, we will always assume $(Q_L-N_{L,\parallel,i_0}^{\text{Meas}}) \approx Q_L$ as we only care about order of magnitudes estimations. We illustrate this on figure \ref{fig:bottleneck_algo_physical_qubits} b).
\begin{figure}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{chapter4/images/bottleneck_algo_physical_qubits}
\caption{\textbf{a)} How the number of qubits is related to the maximum number of gates acting in parallel. On this figure, we illustrate an algorithm composed of two and identity gates. We notice that the number of qubits required by the algorithm (here they appear to be logical ones) is equal to $\max[2 \overline{N}_{L,\parallel}^{\text{cNOT}} + \overline{N}_{L,\parallel}^{\text{1qb}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{Meas}}]=5$, it happens on the red rectangle (but also on the following timestep). \textbf{b)} Intuitive understanding of why we can expect that $Q_L \approx \max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}} \right]$. The red box rectangle verifies $2 \overline{N}_{L,\parallel}^{\text{cNOT}} + \overline{N}_{L,\parallel}^{\text{1qb}}+\overline{N}_{L,\parallel}^{\text{Id}}+\overline{N}_{L,\parallel}^{\text{Meas}}=Q_L$ exactly. But because the measurement gates dominate on this timestep, and that they are identity, single or two qubit gates on the timestep before (we assume that a qubit will never directly be measured as it would be useless for an algorithm), the result is close to $\max_i \left[2 N_{L,\parallel,i}^{\text{cNOT}} + N_{L,\parallel,i}^{\text{1qb}}+N_{L,\parallel,i}^{\text{Id}}\right]$.}
\label{fig:bottleneck_algo_physical_qubits}
\end{center}
\end{figure}
\FloatBarrier
\subsubsection{Expression of the power}
Now, we can regroup the different thing we calculated to express the power on the logical level. On the physical level, it is a function: $P=Q_P a + \sum_{i \in \mathcal{P}_{a}} N^{(i)}_{P,\parallel} b^i$ where $\mathcal{P}_{a}$ correspond to the power-active gate (that we assume here to be $\mathcal{P}_a = \{\text{1qb},\text{cNOT},\text{Meas}\}$). Thus, from \eqref{eq:average_number_physical_gate_timestep1}, \eqref{eq:average_number_physical_gate_timestep2}, \eqref{eq:average_number_physical_gate_timestep3} and \eqref{eq:number_physical_qubits_from_logical}, we have here:
\begin{align}
&P=Q_L t(k) a + \left( b^{\text{1qb}} u(k) + b^{\text{cNOT}} v(k)+ b^{\text{Meas}} w(k)\right) (N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}}) \label{eq:logical_power}\\
& t(k) \equiv \frac{28}{199} 199^k\\
& u(k) \equiv \frac{7}{48}\left(\frac{199}{3}\right)^k\\
& v(k) \equiv \frac{1}{3} \left(\frac{199}{3}\right)^k\\
& w(k) \equiv \frac{7}{48} \left(\frac{199}{3}\right)^k
\end{align}
We remind that we only focused on the transversal logical gates. An algorithm would in principle required other gates than cNOT, what we called single qubit gates here (which were Hadamard or Pauli), identity or measurement gates. Those other gates such as the $T$-gate have to be implemented with a completely different protocole which goes beyond the scope of this thesis. Taking them into account would in principle add additional terms in this power function. That being said, we see that we were able to define the power on the logical level with some adaptations. We have to keep in mind that each term involved in this equation might vary from a coefficient $\epsilon$ roughly between $1$ and $10$ as we only estimated quantities in their order of magnitudes. Now, we can remind the most important hypothesis that lead us here. For the passive costs, we only took into account the ancilla qubits because they give the dominant contribution in the total number of physical qubits. We also assumed that no recycling is being performed for the all ancilla qubits that are inside a given logical gate, and we assumed that the number of physical qubits is proportional to $Q_L$. This will be true for some algorithms, and only an approximation for some others (it depends if the moment when the maximum number of logical qubits are involved at the same time corresponds to a moment some logical qubits are being measured). If this happen to not be true, this approximation should still be fair (see previous discussions). For the active costs, the main assumption that we did is to neglect the "variation" in the concatenated construction between the different kind of logical gates. It allowed us to have a number of physical gates proportional to $(N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}})$. Now, we believe that the most "critical" assumptions, the ones that would change by more than $100 \%$ some of the numbers in \eqref{eq:logical_power} are (i) the assumption that the number of physical qubits is proportional to $Q_L$, (ii) the assumptions behind the qubits recycling. The other considerations should not change our result quantitatively. 

Now, we comment the expressions we obtained. We notice here the functions $t$,$u$,$v$,$w$. They are representing the increasing power cost of the logical elements when more and more error correction is being performed (because more and more physical components are there). They are the "translation" of the energetic cost from the logical to the physical world (where the power is "really" taken in the laboratory). We notice that $u$, $v$ and $w$ are growing following the same law $(199/3)^k$ (with a different prefactor). This law comes from the recursive construction, as the 1-Ec is the same whatever the 1-Ga was, the scaling in the number of physical components will be identical for all the kind of physical gates \red{double check if that's really the reason}. But there is not exactly the same number of cNOT, single qubit gates and measurement gates inside a 1-Ec, this is what explains the different prefactors. In the section \ref{sec:formulation_problem_physical}, we said that we would neglect the active cost related to measurement. This was a fair assumption to do because physical measurements only occured on the boundary of the algorithm (and will thus have a negligible "weight" in term of parallel operation compared to all the other gates occupying the "volume" of the algorithm). Here, as we are doing quantum error correction, physical measurements are done "very frequently in time" (thus inside the "volume") to detect errors. In principle we can no longer neglect them\footnote{Actually as in practice measurement require much less active power than single qubit gate we will still be able to neglect them, but we wanted to emphasize on this difference anyway.}, this is why there is a cost per physical measurement gate represented by $b^{\text{Meas}}$ in \eqref{eq:logical_power}. We also notice that $t(k)/u(k)$, $t(k)/v(k)$ and $t(k)/w(k)$ diverge in the infinite concatenation level. This is based on our assumption that the ancilla qubits are not being recycled within a logical gate. Because of that, the passive cost will dominate in the $k \to \infty$ limit. In practice we can expect that with smart recycling scenarios, those ratios would actually converge toward some constant. We can also see that the passive costs are proportional to the total quantity $(N_{L,\parallel}^{\text{1qb}}+N_{L,\parallel}^{\text{Id}}+2 N_{L,\parallel}^{\text{cNOT}})$. It means that the exact logical gate that is being implemented in the algorithm doesn't matter, what matters is the average number of logical qubits that are actively participating on an information processing level. It also allows us to notice that in the opposite of what we saw without error correction, logical identity gates require an active power consumption. The reason is that it costs energy to protect the information: an error-protected quantum memory \textit{has} an \textit{active} energetic cost. More generally, in fault tolerant quantum computing, because error correction is being performed for any gate, all the logical gate are active in term of power consumption such that we can say $\mathcal{P}_{L,a}=\mathcal{P}_{L,n.a}$ (we remind that $\mathcal{P}_a$ and $\mathcal{P}_{n.a}$ represented the power-active and not active gates in the section \ref{sec:formulation_problem_physical}).
 
\section{Conclusion}
In this chapter, we proposed a formulation for the question of the energetic cost of quantum computing. This formulation is based on a minimization under constraint: we ask to minimize the power it costs to run an algorithm \textit{under the constraint} that the noise contained in its output is not higher than a given target. Formulating the question this way allows to optimize all the tunable parameters in order to reach this minimum. Then, we proposed some generic model for the expression of the power and the metric. We saw that some part of the power are associated to passive energetic cost, i.e they do not depend on what the algorithm is doing at a given instant of time while some other depends on what it is actually doing. It allowed us to see under which perspective energetic considerations can be considered in algorithm compilations problems. Finally, we adapted the generic model for power and metric to fault-tolerant quantum computing working with concatenated codes. The metric on the logical level is the natural generalization of the metric on the physical level. For the power consumption it is however less straightforward, and some approximations are required in order to be able to define it on the logical level. We also saw important differences between the physical and logical power. For instance, because error correction is being applied, all the logical gates will require power to be implemented which is not the case on the physical level: an active operation in term of information processing is also active in term of power consumption. We also saw that each logical gate requires the same amount of power to be implemented: difference in power consumption between different logical gates would be a first order correction to that.

\begin{appendices}
\end{appendices}

